A Piece-wise Polynomial Filtering Approach for Graph Neural Networks

Graph Neural Networks (GNNs) exploit signals from node features and the input graph topology to improve node classification task performance. However, these models tend to perform poorly on heterophilic graphs, where connected nodes have different labels. Recently proposed GNNs work across graphs having varying levels of homophily. Among these, models relying on polynomial graph filters have shown promise. We observe that solutions to these polynomial graph filter models are also solutions to an overdetermined system of equations. It suggests that in some instances, the model needs to learn a reasonably high order polynomial. On investigation, we find the proposed models ineffective at learning such polynomials due to their designs. To mitigate this issue, we perform an eigendecomposition of the graph and propose to learn multiple adaptive polynomial filters acting on different subsets of the spectrum. We theoretically and empirically show that our proposed model learns a better filter, thereby improving classification accuracy. We study various aspects of our proposed model including, dependency on the number of eigencomponents utilized, latent polynomial filters learned, and performance of the individual polynomials on the node classification task. We further show that our model is scalable by evaluating over large graphs. Our model achieves performance gains of up to 5% over the state-of-the-art models and outperforms existing polynomial filter-based approaches in general.

==> iclr2022/sections/approach_V1.tex <==
\section{Proposed Approach}
\label{sec:proposedapproach}

\subsection{Piece-wise Polynomial/Spline Graph Filter Function}
The goal of our proposed modeling approach is to get improved task specific performance by learning effective task-specific graph filters. We learn better graph filters by using a richer class of parameterized frequency filter functions and optimizing task-specific loss function over filter parameters. We model the filtering function $h(\lambda)$ as a piece-wise polynomial or spline function where each polynomial is lower degree (e.g., a cubic polynomial). We partition the eigen-spectrum in $[-1,1]$ (or $[0,2]$ as needed) into contiguous intervals and approximate the desired frequency response by fitting a low degree polynomial in each interval. This helps us to learn more complex shaped frequency response that is optimized for each task.  

Let $\sigma = \{\sigma_1,\sigma_2,\ldots,\sigma_m\}$ denote a partition set with $m$ contiguous intervals and  $h_{i,k_i}(\lambda;\gamma_i)$ denote a $k_i$-degree polynomial filter function of the interval $\sigma_i$ with polynomial coefficients $\gamma_i$. We define PP-GNN filter function as: 
\begin{equation}
    h(\lambda) = \sum_{i=1}^m h_{i,k_i}(\lambda;\gamma_i)
\label{eq:PPFF-GNN}
\end{equation}
and learn a smooth filter function by imposing additional constraints to maintain continuity between polynomials of contiguous intervals at different endpoints (\textit{aka} knots). This class of filter functions is rich, and its complexity is controlled by choosing intervals (i.e., endpoints and number of partitions) and polynomial degrees. Given the filter function, we compute the node embedding matrix as: 
\begin{equation}
    \mathbf{Z} = \sum_{i=1}^m \eigenU_i H_i(\mathbf{\gamma}) \eigenU^T_i {\mathbf Z}_0(\mathbf{X;\Theta})
\label{eq:nodeemb}    
\end{equation}
where $\eigenU_i$ is a matrix with eigenvectors corresponding to eigenvalues that lie in $\sigma_i$. 

\subsection{Practical and Implementation Considerations}
The filter function (\ref{eq:nodeemb}) requires computing eigendecomposition of $\hat{\mathbf{A}}$ and is expensive, therefore, not scalable for very large graphs. Thus, having finer control to learn complex frequency responses comes with a high computational cost. We address this problem by devising a graph filter function that enables trade-off between computational cost and frequency response control. First, we make the following observations: 
\begin{enumerate}
    \item Top-k and bottom-k eigenvalues represent $k$ low and high frequencies. There are efficient algorithms and off-the-shelf library packages available to get top-k and bottom-k eigenvalues and eigenvectors of sparse matrices. 
\item GPR-GNN method also learns a graph filter but operates on the entire eigen-spectrum by sharing the filter coefficients across the spectrum. Therefore, it can be seen as a special case of our proposed model (\ref{eq:nodeemb}). Since GPR-GNN learns a global polynomial by having shared coefficients across the spectrum (like learning a global polynomial to fit a function) it is not flexible enough to learn complex frequency responses, as needed in several practical applications. Note that increasing the degree of the global polynomial does not help beyond some high degree specific to tasks. We demonstrate this through extensive experiments on benchmark datasets in the experiment and appendix sections. One important advantage of GPR-GNN is that it does not require computation of eigendecomposition, therefore, efficient. 
  \item 
    Many recent works including GPR-GNN investigated the problem of designing robust graph neural networks that work well across homophilic and heterophilic graphs. They found that graph filters that amplify or attenuate low and high frequency components of signals (i.e., low-pass and high-pass filters) are critical to get improved performance on several benchmark datasets.
\end{enumerate}
\textbf{Efficient Variant.} Using the above observations, we propose an efficient variant of (\ref{eq:PPFF-GNN}) as: 
\begin{equation}
    {\tilde h}(\lambda) = \eta_l \sum_{i=1}^{m_l} h^{(l)}_{i}(\lambda;\gamma^{(l)}_i) + \eta_h \sum_{i=1}^{m_h} h^{(h)}_{i}(\lambda;\gamma^{(h)}_i) +  \eta_{gpr} h_{gpr}(\lambda;\gamma)
  \label{eq:PPFF-GNN-EFF}
\end{equation}
where the first and second terms fit piece-wise polynomials\footnote{For brevity, we dropped the polynomial degree dependency.} in low and high frequency regions, as indicated through superscripts. However, we do not want to lose any useful information from other frequencies in the central region yet maintain efficiency. We achieve this by adding the GPR-GNN filter function, $h_{gpr}(\lambda;\gamma)$, which is computationally efficient. Since $h_{gpr}(\lambda;\gamma)$ is a special case of (\ref{eq:PPFF-GNN}) and the terms in (\ref{eq:PPFF-GNN-EFF}) are additive, it is easy to see that (\ref{eq:PPFF-GNN-EFF}) is same as (\ref{eq:PPFF-GNN}) with a modified set of polynomial coefficients. In practice, the required low and high frequency components are computed based on affordable computational cost. Furthermore, contributions from each term could be controlled by setting or optimizing over hyperparameters, $\eta_l$, $\eta_h$ and $\eta_{gpr}$. Thus, the proposed model offers richer capability and flexibility in learning complex frequency response and balancing computation cost over GPR-GNN.       

\textbf{Model Training.} Like GPR-GNN, we apply $\textsc{Softmax}$ activation function on (\ref{eq:nodeemb}) and use the standard cross-entropy loss function to learn the sets of polynomial coefficients ($\gamma$) and classifier model parameters ($\Theta$) using labeled data. To ensure smoothness of the learned filter functions, we add a regularization term that penalizes squared differences between the function values of polynomials of contiguous intervals at each other's interval end-points. More details are available in the experiment and appendix sections.  

\textbf{Computational Cost.} There is some pre-training cost of computing the eigendecomposition ($O(n^2k)$)[\sundar{Manan - can you please in Golub and VanLoan book and refer one of the best algorithms and write the cost. That should suffice!}]. Node embedding is computed fresh Whenever the model parameters are updated and this computation involves matrix multiplication with eigenmatrices incurring an additional cost (over GPR-GNN) of $O(nkL)$ where $k$ and $L$ denote the number of selected low/high eigenvalues and classes respectively. 

\subsection{Analysis}
We first give a simple theoretical justification for using multiple polynomials by upper-bounding the error that the optimal approximation such an approximation achieves by the error that the single polynomial parameterization achieves. We relegate the proofs of all the theorems of this section to appendix.

\begin{theorem}
\label{thm:better_approximation}
For any frequency response $h^*$, and an integer $K\in\mathbb{N}/{\infty}$, let $\Tilde{h}:=h+h_f$, with $h_f$ having any random eigenvalue support $\sigma_f$. Assuming $h$ and $h_f$ to be parameterized by $K$-order polynomials $p$ and $p_f$ respectively, then $\min\|\Tilde{h} - h^*\|_2\leq \min\|h-h^*\|_2$. Moreover, for multiple polynomial adaptive filters $h_{f_1},h_{f_2},...,h_{f_m}$ parameterized by independent K-degree polynomials but having disjoint, contiguous supports, the same inequality holds for $\Tilde{h} = h + \sum_{i=1}^m h_{f_i}$.
\end{theorem}

%The proof naturally arises from simple algebraic constructions. One can now think of the adaptive filters as providing better local control over the polynomial fit, adding more degrees of freedom on its support, and hence resulting in a better fit. But since the spectrum of the reference matrix is $[-1,1]$, controlling the lower order terms is more important that fitting the higher order terms, which can be achieved by using adaptive filters parameterized by a lower degree polynomial. One can show by a simple construction that the optimal approximation error by using such filters is still lower than the one achievable by a globally defined polynomial.

\begin{corollary}
\label{thm:lower_than_k}
If the adaptive filters $h_{f_1},h_{f_2},...,h_{f_m}$ are parameterized by independent polynomials having degree $K'\leq K$, and let $h$ be parameterized by a K-degree polynomial, then $\|\Tilde{h} - h^*\|_2\leq \min\|h-h^*\|_2$.
\end{corollary}

We constructed wave-forms of arbitrary complexity, which were then approximated by first fitting a single globally-defined polynomial and then by adding locally defined polynomials on top of it.  We assess the performance by varying the degrees of the local polynomials. The corresponding plots are present in [\ms{Refer to Appendix}] Figure~\ref{fig:fictitious}~which indicate that use of lower-order filters achieves a fit comparable to one by a relatively higher-degree polynomial. Since a real waveform isn't observed in practice and is estimated by optimizing over the observed labels via learning a graph filter, we theoretically show that the family of filters that we learn is a strict superset of the polynomial filter family. The same result is shown to hold true for the families of the resulting adapted graphs.



\begin{theorem}
\label{thm:space_of_filters}
Define $\mathbb{H}:=\{h(\mathbf{\Lambda})\;|\;\forall\text{ possible K-degree polynomial parameterizations of }h\}$ to be the set of all K-degree polynomial filters with diagonal evaluation. Similarly $\mathbb{H}':=\{ \Tilde{h}(\mathbf{\Lambda})\;|\;\forall\text{ possible polynomial parameterizations of }\Tilde{h}\}$ is set of all filters learn-able via \ourmodel~, with $\Tilde{h} = h + h_{f_1} + h_{f_2}$, where $h$ is parameterized by a K-degree polynomial supported over entire spectrum, $h_{f_1}$ and $h_{f_2}$ are adaptive filters parameterized by independent K'-degree polynomials supported over top and bottom $t$ eigenvalues respectively, with $t<n/2$ and $K'\leq K$; then $\mathbb{H}$ and $\mathbb{H}'$ form a vector space, with $\mathbb{H}\subset \mathbb{H}'$. Also, $\frac{\text{dim}(\mathbb{H}')}{\text{dim}(\mathbb{H})} = \frac{K+2K'+3}{K+1}$.
\end{theorem}

\begin{corollary}
\label{thm:space_of_graphs}
The corresponding adapted graph families $\mathbb{G}:=\{\mathbf{U}^T h(\mathbf{\Lambda})\mathbf{U}^T\;|\;\forall h(\mathbf{\Lambda})\in\mathbb{H}\}$ and $\mathbb{G'}:=\{\mathbf{U}^T \Tilde{h}(\mathbf{\Lambda})\mathbf{U}^T\;|\;\forall \Tilde{h}(\mathbf{\Lambda})\in\mathbb{H}'\}$ for any unitary matrix $\mathbf{U}$ form a vector space, with $\mathbb{G}\subset \mathbb{G}'$ and $\frac{\text{dim}(\mathbb{G}')}{\text{dim}(\mathbb{G})} = \frac{K+2K'+3}{K+1}$.
\end{corollary}

This implies that our model is learning from a more diverse space of adapted graphs. Moreover, the dimension of this became three-fold by using just two adaptive filters. To justify that learning from such diverse region is feasible, we first note from the proofs of Theorem 4.2 and Corollary 4.2.1, that using the adaptive filters without any filter with entire spectrum as support, results in learning a set of adapted graphs, $\hat{\mathbb{G}}$, that is disjoint from $\mathbb{G}$, with $\mathbb{G'}=\mathbb{G}\oplus\hat{\mathbb{G}}$. We conduct various ablative studies where we demonstrate the effectiveness of learning from $\hat{\mathbb{G}}$ and $\mathbb{G'}$.

%We set up an experiment, where we learn an adapted graph from the disjoint family, $\hat{\mathbb{G}}$, and compare our results with \gprgnn, which learns from $\mathbb{G}$. Our experiments on multiple datasets result in a significant lift in performance on the graphs with lower homophily score, and a competitive performance on the graphs with higher homophily score. \ms{This section can be moved to answer RQ3 in Experiments}. 

%\begin{enumerate}
%    \item Relate to theoretical/analytical results of the %previous section to contrast GPR-GNN with our model. 
%\end{enumerate}


==> iclr2022/sections/approach_old.tex <==
\section{Proposed Approach}

In this section, we present an alternate interpretation of the \gprgnn~and present our proposed approach that utilizes multiple adaptive filters, each acting on different subsets of the eigen spectrum. 

% . Talk about how we account for left over eigen values by adding in the GPR term. Also, formally describe the model.

\subsection{Untitled Model}

We start by observing closely the GPR component output given by: 
\begin{equation}
    {\mathbf G} = \eigenU h_K(\adjS) \eigenU^T {\mathbf Z}^{(0)}.
\label{eqn:GPRGNN2}    
\end{equation}
Our first observation is that learning filter coefficients is equivalent to learning a \textit{new} graph, ${\tilde \adj(\eigenU, \adjS;\alpha})$ which is dependent on the fixed set of eigenvectors and eigenvalues, but, parameterised using $\alpha$. Therefore, the \gprgnn~model may be interpreted as adapting the original adjacency matrix $\adj$. Next, as noted in the previous section, using the structures present in eigendecomposition and polynomial function, we can expand (\ref{eqn:GPRGNN2}) by unrolling over eigenvalues and interchanging the summation as:
\begin{equation}
    {\mathbf G} = \sum_{j=1}^n \eigenUc_j h_K(\lambda_j;\alpha) \eigenUc^T_j {\mathbf Z}^{(0)}.
\label{eqn:GPRGNN3}    
\end{equation}
% Basis our analysis in Section (Motivation section), we replace the single polynomial filter $h_K(.)$ in equation~(\ref{eqn:GPRGNN3}) with multiple polynomials as defined below:

% \begin{equation}
%     {\mathbf G_{m}} = \sum_{j=1}^n  \eigenUc_i h_K(\lambda_j;\alpha_{(j)}) \eigenUc^T_j {\mathbf Z}^{(0)},
% \label{eqn:multiPolyGPRGNN}    
% \end{equation}

% Equation~(\ref{eqn:multiPolyGPRGNN}) requires explicit decomposition of all eigenvalues. This would be intractable for large graphs. However, it would be feasible to compute and adapt a few eigen components.~\cite{gprgnn} and \cite{fagcn} have shown the importance of high frequency and low frequency components for the node classification task. Taking this into account, we could reformulate equation~(\ref{eqn:multiPolyGPRGNN}) as follows:

% \begin{equation}
%     {\mathbf GL} = \sum_{l=1}^L h_K(\lambda_l; \alpha_{(l)}) u_l u_l^T {\mathbf Z}^{(0)} + \sum_h^H h_K(\lambda_h; \alpha_{(h)}) u_h u_h^T {\mathbf Z}^{(0)}
% \label{eqn:GL}    
% \end{equation}

% where L refers to bottom-L eigen components and H refers to top-H eigen components. Equation~(\ref{eqn:GL}) can be interpreted as multiple polynomial filters acting on L-bottom and H-top eigen components. We can observe that depending on the number of top/bottom eigen components being adapted, several eigen components would be missed out. A simple fix to account for these lost signals would be to add ${\mathbf G}$ to the ${\mathbf GL}$ term, leading to our proposed approach as depicted below:

% \begin{equation}
%     {\mathbf G} + {\mathbf GL} = (1 - \beta)(\eigenU h_K(\adjS) \eigenU^T {\mathbf Z}^{(0)}) + \beta (\sum_{l=1}^L h(\lambda_l; \alpha_{(l)}) u_l u_l^T {\mathbf Z}^{(0)} + \sum_h^H h(\lambda_h; \alpha_{(h)}) u_h u_h^T {\mathbf Z}^{(0)})
% \label{eqn:GGL}    
% \end{equation}

% Since polynomial filters are used across the terms in the above equation, the above polynomials can be added together. The last two terms in equation~(\ref{eqn:GGL}) can be interpreted as correction terms that are working to reduce the residual error discussed in Section~(MOTIVATION). By appropriately setting the value of $\beta$, we can recover the original~\gprgnn~from equation~(\ref{eqn:GGL}). Since all the signals in the eigenspectrum are accounted for in this formulation, one can reduce the computation burden by limiting the explicit adaptation of eigen values (last two terms) depending on the compute available.

% In the following sections, we comprehensively compare our proposed approach against several baselines on benchmark datasets. We also provide several ablative studies and empirical analysis to show the usefulness of our approach.


The output graph of \gprgnn~can be written as:
\begin{equation}
    {\mathbf G} = \sum_k a_k A^k 
\label{eqn:G}    
\end{equation}
where $a_k$ are the learned polynomial coefficients. 

Basis our analysis in Section~\ref{motivation}, we replace the single polynomial filter $h_K(.)$ in equation~(\ref{eqn:GPRGNN3}) with multiple polynomial filters. The new output graph can be written as follows:

\begin{equation}
\mathbf{G_m} = \sum_{j=1}^n {h_K}^{(j)}(\lambda_j) u_j u_j^T
\end{equation}

However, we can observe that this computation would require an explicit decomposition, which would be intractable for large graphs. Let m be the feasible number of eigen components that can be adapted. We write this output graph with explicit adaptation, but missing signals as follows:

\begin{equation}
{\mathbf{GL}} = \sum_m g(\lambda_m) u_m u_m^T
\label{eqn:GL}
\end{equation}

We do the following to compensate for the missing signals in equation~\ref{eqn:GL}. We breakdown the eigenvalues into three disjoint partitions as follows:

\begin{equation}
\mathbf{G} = \eigenU (h_K(\adjS_{E - (E_l + Eh)}) + h_{K_1}(\adjS_{E_l}) + h_{K_2}(\adjS_{E_h}) ) \eigenU^T
\end{equation}

Let ${E_l}$ and ${E_h}$ denote l low-end eigenvalues and h high-end eigenvalues. These components can be captured and adapted by the $\mathbf{GL}$ term. We can see that the first partition term can be viewed as the $\mathbf{G}$ term.

Therefore, the final output graph with multiple polynomial adaptive filters acted on can be written as:

\begin{equation}
\mathbf{G_{eff}} = \sum_k \sum_m a_k \lambda^k u_m u_m^T  + \sum_m g(\lambda_m) u_m u_m^T
\end{equation}





==> iclr2022/sections/experiments_old.tex <==
\section{Experiments}
\renewcommand{\arraystretch}{1.3}

\label{sec:experiments}
We design several experiments to investigate the effectiveness of our proposed approach. Through these experiments, we would like to answer the following questions: \\
\textbf{[RQ1]} In Theorem~\ref{thm:better_approximation}, we claim that using multiple polynomial filters can approximate the latent frequency response better than using a single polynomial filter. How does this translate to classification performance? \textbf{[RQ2]} How does the proposed approach compare against existing state-of-the-art models? 
% \textbf{[RQ3]} We expect our model to work better when the latent optimal filter is of a higher order. How does the learnt filter look in practice? 
\textbf{[RQ3]} Theorem~\ref{thm:space_of_filters} shows that \ourmodel~can learn from a larger set of filters. Does the learnt filter response differ from that of \gprgnn? \textbf{[RQ4]} In Section~\ref{sec:proposedapproach}, we based our model on the observation that low-pass and high-pass frequency components are critical for performance. Do they really contain useful information? \textbf{[RQ5]} Does increasing the number of components and the number of polynomials improve our approximation of latent filter and give better performance? Or are there trade-offs involved? \textbf{[RQ6]} How expensive is it to compute top and bottom eigenpairs in practice?

%In the following subsections, we briefly describe the datasets used in our experiments, and provide responses to the above questions.\\

\textbf{Datasets.} We evaluate our model on several real-world Heterophilic and Homophilic datasets including a few large graphs for the node classification task. Detailed statistics of the benchmark datasets are provided in the Appendix. Our Heterophilic graphs include \textbf{Texas}\footnote{\label{fn:webkb}http://www.cs.cmu.edu/afs/cs.cmu.edu/project/theo-11/www/wwkb}, \textbf{Cornell}\footnotemark[\value{footnote}], \textbf{Wisconsin}\footnotemark[\value{footnote}], \textbf{Chameleon}, \textbf{Squirrel}, \citep{chameleondataset} and \textbf{Flickr}. We evaluate on 8 Homophilic graphs: \textbf{Cora-Full}, \textbf{Obgn-Arxiv}, \textbf{Wiki-CS}, \textbf{Citeseer}, \textbf{Pubmed}, \textbf{Cora}, \textbf{Computer}, and \textbf{Photos} borrowed from \cite{supergat}. We follow the experimental setup described in~\cite{supergat}. For Heterophilic datasets, we use the 10 random splits (48\%/32\%/20\% of nodes for train/validation/test set) from~\cite{geomgcn}. For \textbf{Flickr}, \textbf{Ogbn-Arxiv}, and \textbf{Wiki-CS}, we use the data splits from~\cite{supergat}. For the remaining Homophilic datasets, we create 10 random splits for each dataset following~\cite{supergat}. \textbf{Note:} for \textbf{Chameleon} and \textbf{Cora-Full} datasets, we resort to PCA node features as described in~\cite{supergat}.

% For datasets in \{Texas, Wisconsin, Cornell, Chameleon, Squirrel, Actor\}, we use 10 random splits (48\%/32\%/20\% of nodes for train/validation/test set) from~\cite{geomgcn}. For Crocodile, we create 10 random splits following~\cite{supergat}. We borrowed \textbf{Cora}, \textbf{Citeseer}, and \textbf{Pubmed} datasets and the corresponding train/val/test set splits from \cite{geomgcn}. The remaining datasets were borrowed from \cite{supergat}. We follow the same dataset setup mentioned in \cite{supergat} to create 10 random splits for each of these datasets.


\begin{table}[H]
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccc}
\hline
\multicolumn{1}{c|}{\textbf{Test Acc}}                      & \textbf{Texas}         & \textbf{Wisconsin}     & \textbf{Squirrel}     & \textbf{Chameleon}    & \textbf{Cornell}      & \cellcolor[HTML]{FFFFFF}\textbf{Flickr} \\ \hline
\multicolumn{1}{c|}{\textbf{LR}}                            & 81.35 (6.33)           & 84.12 (4.25)           & 34.73 (1.39)          & 45.68 (2.52)          & \textbf{83.24 (5.64)} & 46.51                                   \\
\multicolumn{1}{c|}{\textbf{MLP}}                           & 81.24 (6.35)           & 84.43 (5.36)           & 35.38 (1.38)          & 51.64 (1.89)          & \textbf{83.78 (5.80)} & 46.93                                   \\
\multicolumn{1}{c|}{\textbf{SGCN}}                          & 62.43 (4.43)           & 55.69 (3.53)           & 45.72 (1.55)          & 60.77 (2.11)          & 62.43 (4.90)          & 50.75                                   \\
\multicolumn{1}{c|}{\textbf{GCN}}                           & 61.62 (6.14)           & 53.53 (4.73)           & 46.04 (1.61)          & 61.43 (2.70)          & 62.97 (5.41)          & 53.4                                    \\
\multicolumn{1}{c|}{\textbf{SuperGAT}}                      & 61.08 (4.97)           & 56.47 (3.90)           & 31.84 (1.26)          & 43.22 (1.71)          & 57.30 (8.53)          & \textbf{53.47}                          \\
\multicolumn{1}{c|}{\textbf{Geom-GCN}}                      & 67.57*                 & 64.12*                 & 38.14*                & 60.90*                & 60.81*                & NA                                      \\
\multicolumn{1}{c|}{\textbf{H2GCN}}                         & \textbf{84.86 (6.77)*} & \textbf{86.67 (4.69)*} & 37.90 (2.02)*         & 58.40 (2.77)          & 82.16 (4.80)*         & OOM                                     \\
\multicolumn{1}{c|}{\textbf{FAGCN}}                         & 82.43 (6.89)           & 82.94 (7.95)           & 42.59 (0.79)          & 55.22 (3.19)          & 79.19 (9.79)          & OOM                                     \\
\multicolumn{1}{c|}{\textbf{APPNP}}                         & 81.89 (5.85)           & 85.49 (4.45)           & 39.15 (1.88)          & 47.79 (2.35)          & 81.89 (6.25)          & 50.33                                   \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{LGC}}   & 80.20 (4.28)           & 81.89 (5.98)           & 44.26 (1.49)          & 61.14 (2.07)          & 74.59 (3.42)          & 51.67                                   \\
\multicolumn{1}{c|}{\textbf{GPR-GNN}}                       & 81.35 (5.32)           & 82.55 (6.23)           & \textbf{46.31 (2.46)} & \textbf{62.59 (2.04)} & 78.11 (6.55)          & 52.74                                   \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{TDGNN}} & 83.00 (4.50)*          & 85.57 (3.78)*          & 43.84 (2.16)          & 55.20 (2.30)          & 82.92 (6.61)*         & OOM                                     \\\hline
% \multicolumn{1}{c|}{\textbf{UFG}}                           & 66.22 (7.46)           & 68.63 (4.98)           & 42.09 (1.70)          & 55.78 (1.29)          & 69.19 (6.40)          & OOM                                     \\ \hline
\multicolumn{7}{c}{\textbf{Our Model}}                                                                                                                                                                                          \\ \hline
\multicolumn{1}{c|}{\textbf{\ourmodel}}                  & \textbf{89.73 (4.90)}  & \textbf{88.24 (3.33)}  & \textbf{56.86 (1.20)} & \textbf{67.74 (2.31)} & \textbf{82.43 (4.27)} & \textbf{54.44}                          \\ \hline
\end{tabular}
}
\caption{Results on Heterophilic Datasets. We bold the results of the models that come close to achieving the performance of our proposed model, as well as the results of the models that perform better than our proposed approach. `*' indicates that the results were borrowed from corresponding papers. For computing the final average rank, we ignore the entries that contain `OOM' or `NA'.}
\label{tab:result_table_heterophily}
\end{table}


\begin{table}[H]
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccc}
\hline
\multicolumn{1}{c|}{\textbf{Test Acc}}                    & \textbf{Cora-Full}    & \cellcolor[HTML]{FFFFFF}\textbf{OGBN-ArXiv} & \textbf{Wiki-CS}      & \textbf{Citeseer}      & \textbf{Pubmed}       & \textbf{Cora}         & \textbf{Computer}                   & \textbf{Photos}       \\ \hline
\multicolumn{1}{c|}{\textbf{LR}}                          & 39.10 (0.43)          & 52.53                                       & 72.28 (0.59)          & 72.22 (1.54)           & 87.00 (0.40)          & 73.94 (2.47)          & 64.92 (2.59)                        & 77.57 (2.29)          \\
\multicolumn{1}{c|}{\textbf{MLP}}                         & 43.03 (0.82)          & 54.96                                       & 73.74 (0.71)          & 73.83 (1.73)           & 87.77 (0.27)          & 77.06 (2.16)          & 64.96 (3.57)                        & 76.96 (2.46)          \\
\multicolumn{1}{c|}{\textbf{SGCN}}                        & 61.31 (0.78)          & 68.51                                       & 78.30 (0.75           & 76.77 (1.52)           & 88.48 (0.45)          & 86.96 (0.78)          & 80.65 (2.78)                        & 89.99 (0.69)          \\
\multicolumn{1}{c|}{\textbf{GCN}}                         & 45.44 (1.01)          & 63.48                                       & 77.64 (0.49)          & 76.47 (1.33)           & 87.86 (0.47)          & 86.27 (1.34)          & 78.16 (1.85)                        & 86.38 (1.71)          \\
\multicolumn{1}{c|}{\textbf{SuperGAT}}                    & 57.75 (0.97)          & 55.1*                                       & 77.92 (0.82)          & 76.58 (1.59)           & 87.19 (0.50)          & 86.75 (1.24)          & 83.04 (1.02)                        & 90.31 (1.22)          \\
\multicolumn{1}{c|}{\textbf{Geom-GCN}}                    & NA                    & NA                                          & NA                    & 77.99*                 & \textbf{90.05*}       & 85.27*                & NA                                  & NA                    \\
\multicolumn{1}{c|}{\textbf{H2GCN}}                       & 57.83 (1.47)          & OOM                                         & OOM                   & \textbf{77.07 (1.64)*} & 89.59 (0.33)*         & 87.81 (1.35)*         & OOM                                 & 91.17 (0.89)          \\
\multicolumn{1}{c|}{\textbf{FAGCN}}                       & 60.07 (1.43)          & OOM                                         & 79.23 (0.66)          & 76.80 (1.63)           & 89.04 (0.50)          & \textbf{88.21 (1.37)} & 82.16 (1.48)                        & 90.91 (1.11)          \\
\multicolumn{1}{c|}{\textbf{APPNP}}                       & 60.83 (0.55)          & \textbf{69.2}                               & 79.13 (0.50)          & 76.86 (1.51)           & 89.57 (0.53)          & 88.13 (1.53)          & 82.03 (2.04)                        & 91.68 (0.62)          \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{LGC}} & \textbf{61.84 (0.90)} & 69.64                                       & \textbf{79.82 (0.49)} & 76.96 (1.73)           & 88.78 (0.51)          & 88.02 (1.44)          & 83.44 (1.77)                        & 91.56 (0.74)          \\
\multicolumn{1}{c|}{\textbf{GPR-GNN}}                     & 61.37 (0.96)          & 68.44                                       & 79.68 (0.50)          & 76.84 (1.69)           & 89.08 (0.39)          & 87.77 (1.31)          & 82.38 (1.60)                        & 91.43 (0.89)          \\
\multicolumn{1}{c|}{\textbf{TDGNN}}                       & OOM                   & OOM                                         & 79.58 (0.51)          & 76.64 (1.54)*          & 89.22 (0.41)*         & 88.26 (1.32)*         & 84.52 (0.92)                        & 92.54 (0.28)          \\ \hline
% \multicolumn{1}{c|}{\textbf{UFG}}                         & 60.98 (0.82)          & OOM                                         & \textbf{78.56 (0.43)} & 76.74 (1.33)           & 85.68 (0.62)          & 87.97 (1.61)          & {\color[HTML]{000000} 80.01 (1.78)} & 90.03 (1.41)          \\ \hline
\multicolumn{9}{c}{\textbf{Our Model}}                                                                                                                                                                                                                                                         \\ \hline
\multicolumn{1}{c|}{\textbf{\ourmodel}}                & \textbf{61.42 (0.79)} & \textbf{69.28}                              & \textbf{80.04 (0.43)} & \textbf{78.25 (1.76)}  & \textbf{89.71 (0.32)} & \textbf{89.52 (0.85)} & \textbf{85.23 (1.36)}               & \textbf{92.89 (0.37)} \\ \hline
\end{tabular}
}
\caption{Results on Homophilic Datasets.}
\label{tab:result_table_homophily}
\end{table}

% \textbf{Importance of ${\mathbf GL}$ Term:} We perform an ablative study in Table~\ref{tab:ablative_table} to understand the importance of GL term. We observe that using  ${\mathbf GL}$ Term alone gives improvements in performance of up to $\sim 10\%$ compared to \gprgnn. However, there is a drop in performance on a Homophilic datasets including Pubmed and Photos. We believe this gap in performance is because of the missing signals that the  ${\mathbf GL}$ Term is not compensating for. By combining \gprgnn with the ${\mathbf GL}$ Term, we can observe performance gains across datasets.


% \begin{table}[h]
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
%                      & \multicolumn{1}{c|}{Texas} & \multicolumn{1}{c|}{Wisconsin} & \multicolumn{1}{c|}{Squirrel} & \multicolumn{1}{c|}{Chameleon} & \multicolumn{1}{c|}{Cornell} & \multicolumn{1}{c|}{Flickr} & \multicolumn{1}{c|}{Cora-Full} & \multicolumn{1}{c|}{Ogbn-arxiv} & \multicolumn{1}{c|}{Wiki-CS} & \multicolumn{1}{c|}{Citeseer} & \multicolumn{1}{c|}{Pubmed} & \multicolumn{1}{c|}{Cora} & \multicolumn{1}{c|}{Computer} & \multicolumn{1}{c|}{Photos} \\ \hline
% \textbf{GPR-GNN}     & 81.35 (5.32)               & 82.55 (6.23)                   & 46.31 (2.46)                  & 62.59 (2.04)                   & 78.11 (6.55)                 & 52.74                       & 61.37 (0.96)                   & 68.44                           & 79.68 (0.50)                 & 76.84 (1.69)                  & 89.08 (0.39)                & 87.77 (1.31)              & 82.38 (1.60)                  & 91.43 (0.89)                \\ \hline
% \textbf{GL Term}     & 85.68 (3.83)               & 85.10 (3.09)                   & 55.63 (1.44)                  & 68.51 (1.64)                   & 82.70 (5.13)                 &                             & 55.93 (0.77)                   &                                 &                              & \textbf{78.41 (1.58)}         & 83.65 (0.53)                & 89.50 (0.78)              & 82.55 (1.93)                  & 89.87 (0.49)                \\ \hline
% \textbf{G + GL Term} & \textbf{89.73 (4.90)}      & \textbf{88.24 (3.33)}          & \textbf{56.86 (1.20)}         & 67.74 (2.31)                   & 82.43 (4.27)                 &                             & \textbf{61.42 (0.79)}          &                                 &                              & 78.25 (1.76)                  & \textbf{89.71 (0.32)}       & \textbf{89.52 (0.85)}     & \textbf{85.23 (1.36)}         & \textbf{92.89 (0.37)}       \\ \hline
% \end{tabular}
% }
% \caption{Importance of GL Term.}
% \label{tab:ablative_table}
% \end{table}


% \textbf{Effect of Varying number of adapted EVD components in ${\mathbf GL}$ Term:} We vary the number of adapted eigenvalues in our proposed approach for four benchmark datasets and plot them in Figure~\ref{fig:EVDablative}. We observe that as we keep increasing the number of adapted eigen components until a certain point, the test accuracy increases in general for graphs with low homophily scores. This phenomenon can be observed in the Chameleon and Squirrel dataset as shown in Figures XXXChameleon, XXXSquirrel. On the contrary, adapting a few eigen components in graphs with higher homophily levels seems sufficient as can be seen in Figures XXXCora, XXXCiteseer. The test accuracy stabilizes even though more eigen components are adapted. We conjecture that a smooth polynomial filter is sufficient for homophilic graphs, while a complicated polynomial might be required for graphs with lower homophilic scores. 

% \begin{figure}[t!]
%     \centering
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.95\textwidth]{images/G_GL_EVDPlots/chameleon_pca.jpg}
%         \caption{Chameleon}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.95\textwidth]{images/G_GL_EVDPlots/squirrel.jpg}
%         \caption{Squirrel}
%     \end{subfigure} 
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.95\textwidth]{images/G_GL_EVDPlots/cora.jpg}
%         \caption{Cora}
%     \end{subfigure}%
%     ~
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.95\textwidth]{images/G_GL_EVDPlots/citeseer.jpg}
%         \caption{Citeseer}
%     \end{subfigure}
%     \caption{Effect of Varying EVD components}
%     \label{fig:EVDablative}
% \end{figure}


% \textbf{Comparing Polynomials learned by our model against that of \gprgnn's:} To pictorially analyse the effect of adaptation in \gprgnn and our model, we plot the learned polynomials in Figure~\ref{fig:polyPlots}. We observe that the polynomials learned by our model starkly differs from \gprgnn's polynomial on Heterophilic datasets like Texas and Squirrel. Also, these are the datasets, where our approach outperforms \gprgnn's classification performance by a significant margin. Conversely, the polynomials learned by both these approaches are very similar in Homophilic datasets like Cora and Citeseer. We believe that adapting the eigen spectrum using multiple filters has more significant effect in terms on performance on Heterophilic datasets than on Homophilic datasets. 


% \begin{figure}[H]
%     \centering
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.95\textwidth]{images/G_GL_polyPlots/texas_split5.png}
%         \caption{Texas}
%         \label{fig:texas}
%     \end{subfigure}%
%     ~
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.95\textwidth]{images/G_GL_polyPlots/squirrel_split3.png}
%         \caption{Squirrel}
%         \label{fig:squirrel}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.95\textwidth]{images/G_GL_polyPlots/cora_split2.png}
%         \caption{Cora}
%         \label{fig:Cora}
%     \end{subfigure}%
%     ~
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.95\textwidth]{images/G_GL_polyPlots/citeseer_split8.png}
%         \caption{Citeseer}
%         \label{fig:citeseer}
%     \end{subfigure}
%     \caption{Learned Polynomial Plots. Red curves correspond to the learned polynomial from our model. Blue curve corresponds to \gprgnn's learned polynomial.}
%     \label{fig:polyPlots}
% \end{figure}


% \textbf{RQ1.} How does adapting low and high frequency components simultaneously affect task performance? \textit{GL Term is important, Varying EVD comps in G+GL} \todo{\textbf{Add Ablative Table, Discuss which plots to add}}

\textbf{[RQ1] \ourmodel~vs. \gprgnn~\ms{Need to fix the title}}

% We conduct an extensive set of experiments that compare~\ourmodel~against \gprgnn~and report the results in Tables~(\ref{tab:result_table_heterophily},~\ref{tab:result_table_homophily}). \ourmodel~outperforms \gprgnn~on all our benchmark datasets with significant gains of up to~10\% on heterophilic datasets and considerable gains of up to~2\% on homophilic datasets. Our studies at an individual split level for benchmark datasets show performance gains ranging from 0.15\% to 18.92\%. \ms{Refer to Appendix} \ms{T-SNE plots for qualitative analysis}

\textbf{Points to convey:} \\
1) Using multiple polynomial filters over single filter can give superior performance. This is evident in Tables~(\ref{tab:result_table_heterophily},~\ref{tab:result_table_homophily}). \\
2)On performing an individual split level analysis, we observe gains with our model over \gprgnn~on almost all of the splits [on 93.6\% splits, we have better results]. \\
3) t-SNE plots of learned embedding



\textbf{[RQ2] Comparison against other state-of-the-art models?}

% \textbf{Baselines.} We compare our model against filtering based approaches, which includes~\gprgnn, ~\fagcn, ~\ufg, and~\lingcn. Other state-of-the-art baseline models include~\tdgnn,~\mixhop,~\hhgcn, and~\geomgcn. In addition, we compare against standard baselines namely, \textsc{LR} (Logistic Regression), \textsc{MLP} (Multi Layer Perceptron), ~\gcn, and~\sgcn. Detailed baselines descriptions, hardware and software specifications including hyper-parameter tuning are provided in the Appendix.

% \textbf{Performance on Benchmark Datasets:} The test performance of the various baselines and our approach is reported in Table~\ref{tab:result_table_heterophily} and~\ref{tab:result_table_homophily}. We observe that on both homophilic and heterophilic datasets, \ourmodel~outperforms or performs competitively to the baselines in comparison. We compute the average rank for all the models in comparison across datasets and observe that \ourmodel~ achieves a rank of XXX.

\textbf{Points to Convey:} [Can combine with (RQ1)] \\ 
1) We observe that our model outperforms all the baselines in comparison on majority on the datasest. On the remaining datasets, we perform competitively. We observe significant lifts of up to 10\% over previous SOTA models.
2) Average rank of our model.

% \textbf{[RQ3]} We expect our model to work better when the latent optimal filter is of a higher order. How does the learnt filter look in practice? What about the optimal filter?


\textbf{[RQ3] \ourmodel's learnt frequency response.}
\textbf{Use Figure ~\ref{fig:PPGNN_learned_poly} for this RQ. The important points are conveyed in the below para. Additional point: Significant improvement in classification performance on heterophilic graphs, where we also observe a stark difference in learnt frequency responses of models in comparison.} 
Figure ~\ref{fig:PPGNN_learned_poly} indicates that \ourmodel~learns a more complicated frequency response compared to \gprgnn~for heterophilic datasets, while both the models learn a simple and similar frequency response for homophilic datasets. This indicates that the latter possibly requires a simple frequency response to achieve a better task performance with a single polynomial filter. This is in stark contrast to heterophilic datasets, where multiple polynomial filters significantly improve the task performance. Even though the learned frequency response is marginally different from \gprgnn's response, we observe considerable gains in homophilic datasets. For instance, we observe gains of up to 1.18\% in Citeseer and up to 2.19\% on Computers dataset. Our observations align with Theorem~\ref{thm:space_of_filters}, which shows that \gprgnn~is incapable of constructing the complicated frequency response that \ourmodel~ is learning. 

\begin{figure}[H]
    % \centering
    % \begin{subfigure}[t]{0.5\textwidth}
    %     \centering
    %     \includegraphics[height=1.5in, width=0.85\textwidth]{iclr2022/images/G_GL_polyPlots/chameleon_pca_boundaryReg.png}
    %     \caption{Chameleon}
    %     \label{RQ3_chameleon}
    % \end{subfigure}%
    % ~ 
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[height=1.5in, width=0.85\textwidth]{iclr2022/images/G_GL_polyPlots/squirrel_boundaryReg.png}
        \caption{Squirrel}
        \label{RQ3_squirrel}
    \end{subfigure}
    % \\
    % \vspace{2mm}
    % \begin{subfigure}[t]{0.5\textwidth}
    %     \centering
    %     \includegraphics[height=1.5in, width=0.85\textwidth]{iclr2022/images/G_GL_polyPlots/amazon_electronics_computers_boundaryReg.png}
    %     \caption{Computers}
    %     \label{RQ3_computers}
    % \end{subfigure}%
    % ~ 
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[height=1.5in, width=0.85\textwidth]{iclr2022/images/G_GL_polyPlots/citeseer_boundaryReg.png}
        \caption{Citeseer}
        \label{RQ3_citeseer}
    \end{subfigure}
    
    \caption{Visualization of adapted eigenspectrum by our proposed model and~\gprgnn}
    \label{fig:PPGNN_learned_poly}
\end{figure}

% The next question that we would like to address is that does such a complicated polynomial exist in practice? 

% Since we don't have access to this underlying optimal frequency response, we try to construct this `optimal' frequency response by solving a regression task. The details of this regression are left to the appendix. On plotting the moving average of this constructed frequency response, we observe that our learned polynomial filters are structurally similar to this constructed frequency response, thereby learning. \textbf{I am not sure whether we should include this question/points at all. This is like opening a can of worms as these are the questions a reviewer can ask: 1. Does a complicated polynomial exist in practise? If we use the constructed optimal polynomial, now all the claims about not needed a complicated polynomial for homophilic datasets don't work anymore. If we do decide to add this, lets just remove the question on the optimal polynomial. Lets take a call on this.} 

\textbf{[RQ4] In Section~\ref{sec:proposedapproach}, we based our model on the observation that low-pass and high-pass frequency components are critical for task performance. Do they really contain useful information?}

\textbf{Using Table~\ref{tab:result_ppgnnVSgprgnn}, Figure~\ref{fig:AdaptingEVDTopBottom}}

\textbf{Points to convey:}

1) Adapting the lower and higher ends of the spectrum for heterophilic datasets can already lead to a graph that performs well for the node classification task. However, adapting the entire spectrum for homophilic datasets leads to a better node classification performance, as compared to adapting only the ends of the spectrum. This seems to show that the lower and higher ends of the spectrum contain lot more information about the graph for heterophilic datasets, while the information seems to be more diffused throughout the entire spectrum for homophilic datasets. On adapting both the lower and higher ends of the spectrum in conjunction with adapting the entire spectrum does lead to better classification performance for homophilic datasets, further strengthening the argument that adapting the entire spectrum is indeed required for homophilic graphs.   
From this analysis, we conjecture that for heterophilic datasets, the lower and higher ends of the spectrum contain a lot more information about the graph (for the task at hand). We also conjecture that for homophilic datasets, the information regarding the graph is diffused throughout the spectrum thereby needing adaption on the entire spectrum. Evidence from Table~\ref{tab:result_ppgnnVSgprgnn}. For instance, GL Term outperforms GPR-GNN on all heterophilic datasets. However, GL term is lacking in performance on Homophilic datasets. In PP-GNN, where the missing middle eigen spectrum is also accounted for, we see it performing well across the datasets. This reiterates it is important to account for the entire spectrum in homophilic graphs. 

We plot the results for the described studies in Figure~\ref{fig:AdaptingEVDTopBottom} and make the following observations: 1) For Homophilic datasets, adapting an increasing number of components in the lower ends of the spectrum exhibits better classification accuracy compared to adapting the higher end counterparts. Also, adapting only the lower or higher frequencies in conjunction with a global filter shows similar performance. Basis these observations, we extrapolate that important signals in the input graph are diffused throughout the spectrum, thereby requiring an adaption on the entire spectrum. 2) On the contrary, Heterophilic datasets display significant improvements in performance by adapting the higher ends of the spectrum. We also observe that adapting the lower ends of the spectrum in conjunction with adapting the entire spectrum performs worse than adapting only higher ends of the spectrum. This seems to show that for Heterophilic datasets, useful signals for the task at hand are concentrated in the higher end of the spectrum. 




\begin{table}[H]
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|ccccccccccc}
\hline
{\color[HTML]{000000} \textbf{Test Acc}} & \textbf{Texas}                                 & \textbf{Wisconsin}                             & \textbf{Squirrel}                              & \textbf{Chameleon}                    & \textbf{Cornell}                      & \textbf{Cora-Full}                             & \textbf{Citeseer}                              & \textbf{Pubmed}                                & \textbf{Cora}                                  & \textbf{Computer}                              & \textbf{Photos}                                \\ \hline
\textbf{GPR-GNN}                & 81.35   (5.32)                                 & 82.55   (6.23)                                 & 46.31   (2.46)                                 & 62.59   (2.04)                        & 78.11   (6.55)                        & 61.37   (0.96)                                 & 76.84   (1.69)                                 & 89.08   (0.39)                                 & 87.77   (1.31)                                 & 82.38   (1.60)                                 & 91.43   (0.89)                                 \\
\textbf{GL Term}                & 85.68   (3.83)                                 & 85.10   (3.09)                                 & 55.63   (1.44)                                 & \textbf{68.51 (1.64)}                 & \textbf{82.70 (5.13)}                 & 55.93   (0.77)                                 & {\color[HTML]{330001} \textbf{78.41   (1.58)}} & 83.65   (0.53)                                 & 89.50   (0.78)                                 & 82.55   (1.93)                                 & 89.87   (0.49)                                 \\
\textbf{\ourmodel}            & {\color[HTML]{000000} \textbf{89.73   (4.90)}} & {\color[HTML]{000000} \textbf{88.24   (3.33)}} & {\color[HTML]{000000} \textbf{56.86   (1.20)}} & {\color[HTML]{000000} 67.74   (2.31)} & {\color[HTML]{000000} 82.43   (4.27)} & {\color[HTML]{000000} \textbf{61.42   (0.79)}} & {\color[HTML]{000000} 78.25   (1.76)}          & {\color[HTML]{000000} \textbf{89.71   (0.32)}} & {\color[HTML]{000000} \textbf{89.52   (0.85)}} & {\color[HTML]{000000} \textbf{85.23   (1.36)}} & {\color[HTML]{000000} \textbf{92.89   (0.37)}} \\ \hline
\end{tabular}
}
\caption{\ourmodel~v/s \gprgnn}
\label{tab:result_ppgnnVSgprgnn}
\end{table}

\begin{figure}[H]
    \centering
        \includegraphics[height=1.2in, width=\textwidth]{iclr2022/images/G_GL_tuning_lowHigh_comps/TuningEVDcollage_GPRGNN_tuningLowHighEVD.png}
    \label{fig:AdaptingEVDTopBottom}
    \caption{Adapting increasing number of top or bottom EVD components}
\end{figure}


% \textbf{[RQ4] Importance of low/high frequency components.}
%The improvement over the classification performance can be explained from two perspectives: (a) from the filter response, and (b) the adapted graph being learnt. All the experiments done till now indicate that we need more control over the frequency response towards the extremal subsets of the spectrum for the graphs having lower homophily score as compared to ones having a higher score, which work upon a shared polynomial response. 
% Theorem`\ref{thm:space_of_filters} showed that the basis corresponding to the adaptive filters (with supports on spectrum's extrema) spans a different space, a point of which represents the corresponding low/high frequency response. We term these points to be having a 'locally focused response'. Following \textbf{[RQ3]}, we know that homophilic graphs are relatively apathetic towards the locally-focused responses. To understand the role of adapting low and high frequency components in \ourmodel~for homophilic datasets, we perform the following ablative studies. \textbf{1)} We assess the test performance for our \ourmodel~with only the $G_L$ term. This forces to learn from a locally-focused family. The results are present in Figure~\ref{fig:AdaptingEVD}, where learning with only the GL term (plot corresponding to 'GL EVD') results in a marginal drop of performance as comapred to the global model. \textbf{2)} To study this lack of sensitivity, we conduct another experiment, where we vary the parameters of the adaptive filters, namely support-size and the number of polynomials. We plot these results as  Figure~\ref{RQ4_cora}. We can observe that the homophilic graphs' performance is seemingly unaffected by these parameters. \textbf{3)} To compare the relative importance of top and bottom ends of the spectrum, we conduct experiments, where we adapt only one of these ends at a time, on two models: a model with global polynomial present (we call it '\ourmodel-Top/Bottom EVD') and a model without it (referred to as 'GL-Top/Bottom EVD'). The corresponding results are plotted in Figure~\ref{fig:AdaptingEVD}. As expected, the first model is insensitive to the adaptation of any of the ends, whereas in the second model, we observe that adapting the bottom end of the spectrum gives significant performance lifts as compared to adapting the top end. This seems to suggest that a lot more information that is present at the lower ends of the spectrum as compared to the top ends. It also seems to show that information is diffused throughout the spectrum, for homophilic graphs.

% We perform similar sets of experiments for heterophilic datasets: \textbf{1)} When we force the model to learn from a global family, which is what \gprgnn~does, there's a significant drop in the performance, as evident in Table 1, which is in line with our claims. \textbf{2)} We modify this experiment, where now we run two models: \ourmodel~which adapts to both ends of spectrum (referred to as '\ourmodel~EVD') and the same model without the global polynomial (referrred to as 'GL EVD'), with results plotted in Figure~\ref{fig:AdaptingEVD}. We observe that the presence of a global polynomial doesn't affects the performance much. We then plot the learnt frequency response of only the GL term \ms{we also comment on beta here. If these look favourable, we add a line here}. \textbf{3)} For experiments where we adapt only one of these ends at a time, the results are plotted in Figure~\ref{fig:AdaptingEVD}. In contrast to our observations for homophilic datasets, adapting only the top ends of the spectrum gave significant performance gains compared to adapting only the lower end. We can observe that adapting the bottom ends of the spectrum in conjunction with adapting the entire spectrum still performs worse than adapting only the higher ends of the spectrum, on increasing the number of adapted eigenpairs. This seems indicate that useful signals, for the task at hand, are concentrated at the higher ends of the spectrum.   
%Experiment description%
% \ms{We plan an experiment where we run one $G_L$ only model in parallel with $G+G_L$ model of \gprgnn~for the heterophilic datasets and then observe the waveform learnt by the $G_L$ filters of both the $G_L$ only model and $G+G_L$ only model. If they seem to coincide/be very similar, we can make a strong statement: heterophilic Graphs are apathetic to the global polynomial family in presence of a locally-focused family, whereas homophilic datasets are apathetic to any locally focused family in presence of a global family. We have evidence for latter half, but we would need the $G_L$ responses for the first}.

\textbf{[RQ5] Does increasing the number of components and the number of polynomials improve our approximation of the underlying latent filter and give better performance?}\\

\textbf{Using Figure~\ref{fig:AdaptingSupportSize}}

\textbf{Points to convey:} \\
1) The variation in performance when increasing the number of polynomial filters is minimal. This same trend is observed across both homophilic and heterophilic graphs. 
[For fixed polynomial order]
2) For heterophilic graphs, varying the support size (number of evd components adapted) has a significant effect on the task performance. For instance, in Chameleon dataset (Figure~\ref{fig:AdaptingSupportSize} a) the task performance reaches it's peak when the support size increases to 256 and then we observe a dip in performance as we increase the support size. However, in Squirrel dataset, the task performance sharply increases as we increase the support size. As emphasized before, important signals for task are concentrated in extremes of the eigenspectrum for heterophilic graphs. This phenomenon is reflected in our plots.
3) For homophilic graphs, the task performance is agnostic to any increment in the support size. [Not sure why this is happening. Analysing the beta values might give us some insights.]
4) We also repeat the same analysis for a different polynomial order and observe similar behavior. This also suggests we can get good performance using our model with even a lower order polynomial.


\begin{figure}[H]
    \centering
        \includegraphics[height=1.2in, width=\textwidth]{iclr2022/images/2D_Plots/2D_plot_all_5_degree.png}
    \label{fig:AdaptingSupportSize5}
    \caption{Effect of varying the number of polynomial filters and the support size for a 5textsuperscript{th} polynomial}
\end{figure}


\begin{figure}[H]
    \centering
        \includegraphics[height=1.2in, width=\textwidth]{iclr2022/images/2D_Plots/2D_plot_all_10_degree.png}
    \label{fig:AdaptingSupportSize10}
    \caption{Effect of varying the number of polynomial filters and the support size for a 5textsuperscript{th} polynomial}
\end{figure}


\begin{table}[H]
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|llll}
\hline
\textbf{Test Acc}      & \multicolumn{1}{c}{\textbf{Squirrel}} & \multicolumn{1}{c}{\textbf{Chameleon}} & \multicolumn{1}{c}{\textbf{Citeseer}}                     & \multicolumn{1}{c}{\textbf{Cora}}   \\ \hline
\textbf{GL (Low)}      & 45.75 (1.69)                          & 56.73 (4.03)                           & 76.23 (1.54)                                              & 88.03 (0.79)                        \\
\textbf{GL (High)}     & 58.70 (1.60)                          & 69.19 (1.88)                           & 55.50 (6.38)                                              & 73.76 (2.03)                        \\
\textbf{G + GL (Low)}  & 50.96 (1.26)                          & 63.71 (2.69)                           & 78.07 (1.71)                                              & 89.56 (0.93)                        \\
\textbf{G + GL (High)} & 60.39 (0.91)                          & 67.83 (2.30)                           & 78.30 (1.60)                                              & 89.42 (0.97)                        \\ \hline
\textbf{PP-GNN}        & 56.21 (1.79)                          & 68.93 (1.95)                           & \multicolumn{1}{c}{{\color[HTML]{000000} 78.25   (1.76)}} & {\color[HTML]{000000} 89.52 (0.85)}
\end{tabular}
}
\caption{}
\label{tab:result_ppgnnVSgprgnn}
\end{table}

\begin{figure}[H]
    \centering
        \includegraphics[height=1.2in, width=\textwidth]{iclr2022/images/G_GL_tuning_lowHigh_comps/TuningEVDcollage_GPRGNN_tuningLowHighEVD.png}
    \label{fig:AdaptingEVDTopBottom}
    \caption{Adapting increasing number of top or bottom EVD components}
\end{figure}


% For heterophilic datasets, increasing the number of filters with fixed supports at spectrum's extremes can give the desired local control and allows us to search for models in an even higher dimensional subspace. However, this control comes at a cost of increased model complexity, thus increasing the generalization error. Due to this bias-variance trade off, we do not expect to see any monotonous trend in performance while increasing the number of filters. This is also reflected in Table X. One possible way to mitigate this trade off is to increase the support size without changing the number of filters. This does not reduces the bias as the model complexity and the search space dimension remain the same. Thus, we can adapt to more regions of the spectrum's extremas without running into bias-variance pulls. But since we have observed that model is relatively apathetic to global adaptation for heterophilic datasets, this indicates that the central parts of the spectrum adds a diffused signal to the response. This is further indicated by experiments of table XXX, where we see a significant increase in performance for initial increase of the support, but the performance drops after increasing it more than a certain number, which we hypothesize is where the diffusive response starts accumulating.

%To understand the role of adapting low and high frequency components in our proposed model, we perform the following ablative study. Our model can be viewed as learning a global filter (G, refer to equation) that acts on the entire eigenspectrum, which is refined by multiple adaptive polynomial filters (GL) acting on a few disjoint subsets of this spectrum. We decouple G and GL and study them in isolation. We report the test performance for these individual components in Table XXX and make the following observations: % We first learn a graph filter (G / GPR-GNN) that acts on the entire spectrum. Next, we learn a graph filter (GL) that adapts only the lower and higher ends of the eigenspectrum. Finally, we combine both the filters (G + GL/ PP-GNN) to understand the effect of such a combination.1) The graph filter (GL) performs better than the graph filter (G) (\gprgnn) on Heterophilic datasets. However, on most Homophilic datasets, G performs better than GL. We conjecture that for Heterophilic graphs, adapting both lower and higher ends of the spectrum can already lead to a graph that performs well for the node classification task. However, reaching such a graph for Homophilic datasets might require adapting the entire spectrum as useful signals could be scattered throughout. 
%1) Adapting the lower and higher ends of the spectrum for heterophilic datasets can already lead to a graph that performs well for the node classification task. However, adapting the entire spectrum for homophilic datasets leads to a better node classification performance, as compared to adapting only the ends of the spectrum. This seems to show that the lower and higher ends of the spectrum contain lot more information about the graph for heterophilic datasets, while the information seems to be more diffused throughout the entire spectrum for homophilic datasets. On adapting both the lower and higher ends of the spectrum in conjunction with adapting the entire spectrum does lead to better classification performance for homophilic datasets, further strenthening the arguement that adapting the entire spectrum is indeed required for homophilic graphs.   
% From this analysis, we conjecture that for heterophilic datasets, the lower and higher ends of the spectrum contain a lot more information about the graph (for the task at hand). We also conjecture that for homophilic datasets, the information regarding the graph is diffused throughout the spectrum thereby needing adaption on the entire spectrum. 
% 2) Following the previous conjecture, we then combine both G and GL and observe a performance boost across all the homophilic datasets, while retaining or improving performance across heterophilic datasets as well. 
% 2) Combining G with GL adapts the eigenspectrum that is not accounted in the GL graph filter. This effect is also reflected in Table XXX. G + GL model achieves significant improvements on Heterophilic datasets, while also giving considerable lifts on Homophilic datasets. This study reaffirms our conjecture that adapting the entire spectrum does indeed help increase the performance on Homophilic datasets.   


% \begin{figure}[H]
%     \centering
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.85\textwidth]{iclr2022/images/TA_Varying_EVD_Components/chameleon_pca_TA_Varying_EVD_Components.png}
%         \caption{Chameleon}
%         \label{RQ1_chameleon}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.85\textwidth]{iclr2022/images/TA_Varying_EVD_Components/citeseer_TA_Varying_EVD_Components.png}
%         \caption{Citeseer}
%         \label{RQ1_citeseer}
%     \end{subfigure}
%     ~
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.85\textwidth]{iclr2022/images/TA_Varying_EVD_Components/cora_TA_Varying_EVD_Components.png}
%         \caption{Cora}
%         \label{RQ1_cora}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.85\textwidth]{iclr2022/images/TA_Varying_EVD_Components/squirrel_TA_Varying_EVD_Components.png}
%         \caption{Squirrel}
%         \label{RQ1_squirrel}
%     \end{subfigure}
    
%     \label{fig:RQ1}
%     \caption{Impact of number of EVD components adapted on Test Accuracy in proposed model}
% \end{figure}


% Need to reformulate RQ2. THis is what we would have to add: How does adapting only low (GL-Low) and only high frequency (GL-High) components in conjunction with G affect task performance? Is it sufficient to create such a filter?
% \textbf{RQ2. How does adapting only low and high frequency components in isolation affect task performance? Is it sufficient to adapt only high or only low frequency components?} \textit{It is better to adapt both ends of the spectrum following experiments}

%\textbf{Our previous studies highlight the importance of adapting both low and high frequency components. How does adapting only low and high frequency components in isolation affect task performance? Is it sufficient to adapt only high or only low frequency components?}

%To understand this phenomenon, we perform two ablative studies: i) The first study adapts increasing number of eigenvalues in the lower ends of the frequency spectrum. ii) The second study explores a similar setting in the higher ends of the frequency spectrum. We further extend these studies by appending another filter in conjunction to adapt the entire frequency spectrum. We finally compare these settings with our proposed approach, which adapts eigenvalues in both ends of the spectrum in conjunction with a global filter.
% We finally adapt both the higher and lower ends of the spectrum while having another filter in conjunction that adapts the entire spectrum. 
%We plot the results for the described studies in Figure XXX and make the following observations: 1) For Homophilic datasets (Figures X, Y), adapting increasing number of components in the lower ends of the spectrum exhibits better classification accuracy compared to adapting the higher end counterparts. Also, adapting only the lower or higher frequencies in conjunction with a global filter shows similar performance. Basis these observations, we extrapolate that important signals in the input graph are diffused throughout the spectrum, thereby requiring an adaption on the entire spectrum. 2) On the contrary, Heterophilic datasets display significant improvements in performance by adapting the higher ends of the spectrum. We also observe that adapting the lower ends of the spectrum in conjunction with adapting the entire spectrum performs worse than adapting only higher ends of the spectrum. This seems to show that for Heterophilic datasets, useful signals for the task at hand are concentrated in the higher end of the spectrum. 
% \todo{1. Add Performance Plots. 2. Finish and add the polynomial plots, refine RQ2 once we have the polynomial plots.}



% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.85\textwidth]{iclr2022/images/G_GL_tuning_lowHigh_comps/chameleon_pca_GPRGNN_tuningLowHighEVD.png}
%         \caption{Chameleon}
%         \label{RQ2_chameleon}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.85\textwidth]{iclr2022/images/G_GL_tuning_lowHigh_comps/citeseer_GPRGNN_tuningLowHighEVD.png}
%         \caption{Citeseer}
%         \label{RQ2_citeseer}
%     \end{subfigure}

    % \begin{subfigure}[t]{0.5\textwidth}
    %     \centering
    %     \includegraphics[height=1.5in, width=0.85\textwidth]{iclr2022/images/G_GL_tuning_lowHigh_comps/cora_GPRGNN_tuningLowHighEVD.png}
    %     \caption{Cora}
    %     \label{RQ2_cora}
    % \end{subfigure}%
    % ~ 
    % \begin{subfigure}[t]{0.5\textwidth}
    %     \centering
    %     \includegraphics[height=1.5in, width=0.85\textwidth]{iclr2022/images/G_GL_tuning_lowHigh_comps/squirrel_GPRGNN_tuningLowHighEVD.png}
    %     \caption{Squirrel}
    %     \label{RQ2_squirrel}
    % \end{subfigure}
    
%     \label{fig:AdaptingEVD}
%     \caption{Adapting increasing number of top or bottom EVD components}
% \end{figure}


\textbf{RQ6. [Manan] How expensive is it to compute top/bottom EVD components in practice? (Can move it to motivation section as well)}\\
Since we only deal with the extremal eigenpairs, we use \MATLAB implementation of the Arnoldi-Lanczos' Iterative Algorithm, provided via ARPACK, which proceeds by first tridiagonalizing the input matrix, and then performs a series of non-trivial steps to obtain the required eigenpairs. It benefits immensely from the sparsity and symmetry of the input matrix, making it a suitable choice for. Complexity analysis of Lanczos seems to be hard to find in the literature. Analysis of the probabilistic relative failure of the algorithm, by Kuczyński and Woźniakowski indicates that the bounds for the Lanczos algorithm depend on the ratio between the difference of the two largest eigenvalues and the difference of the largest and the smallest eigenvalues.



%\textbf{RQ3 [Manan]  What is the effect of using multiple adaptive filters on classification performance? How \ourmodel's filter response varies from GPRGNN's. Can we connect this difference to improvements in accuracy? \ms{A possible reframe: "How can we attribute use of high/low pass filters to the performance gains, and when are they useful? Also what effects does the number of polynomials and the support sizes have on the performance?"; the difference in response then serves to answer the second question}}\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.85\textwidth]{images/2D_Plots/chameleon_pca_2D_plot_10_order}
%         \caption{Chameleon}
%         \label{RQ4_chameleon}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.85\textwidth]{images/2D_Plots/cora_2D_plot_10_order}
%         \caption{Cora}
%         \label{RQ4_cora}
%     \end{subfigure}
%     % \\
%     % \vspace{2mm}
%     % \begin{subfigure}[t]{0.5\textwidth}
%     %     \centering
%     %     \includegraphics[height=1.5in, width=0.85\textwidth]{images/2D_Plots/squirrel_2D_plot_10_order}
%     %     \caption{Squirrel}
%     %     \label{RQ4_squirrel}
%     % \end{subfigure}%
%     % ~ 
%     % \begin{subfigure}[t]{0.5\textwidth}
%     %     \centering
%     %     \includegraphics[height=1.5in,width=0.85\textwidth]{images/2D_Plots/computers_2D_plot_10_order}
%     %     \caption{Computers}
%     %     \label{RQ4_computers}
%     % \end{subfigure}
    
%     \caption{Effect of varying the number of polynomial filters and the support size}
%     \label{fig:RQ4}
% \end{figure}

%\textbf{RQ4.} In Theorem X, we claimed that multiple polynomial adaptive filters can give lesser classification error compared to using a single polynomial filter. Does this actually happen in practice? What happens to the task performance as we vary the degree of the polynomial, the number of eigenvalues adapted and the number of adaptive filters?
% vary the number of adaptive filters
%5To understand 

%\todo{1. Update plot for all the intermediate values [2, 4, 8, 16,.., 1024], 2. Add plots. 3. Refine RQ4. once thats done}







%\textbf{RQ5.} Theorem Y shows that our proposed model can explore a larger space of graphs than~\gprgnn, thereby possibly leading to obtain a better graph for the task at hand. Can we quantify the quality of these graphs? \textbf{TBD: Experiment has to be done}


==> iclr2022/sections/preliminaries_V1.tex <==
\section{Problem Setup and Motivation}
\label{sec:preliminaries}
We focus on the problem of semi-supervised node classification on a simple graph $\graph = (\verts, \edges)$, where $\verts$ is the set of vertices and $\edges$ is the set of edges. Let $\adj \in \{0, 1\}^{n \times n}$ be the adjacency matrix associated with $\graph$, where $n = |\verts|$ is the number of nodes. Let $\mathcal{Y}$ be the set of all possible class labels. Let $\feat \in \real^{n \times d}$ be the $d$-dimensional feature matrix for all the nodes in the graph. Given a training set of nodes $\train \subset \verts$ whose labels are known, along with $\adj$ and $\feat$, our goal is to predict the labels of the remaining nodes. Let $\adji = \adj + \eye$ where $\eye$ is the identity matrix. Let $\dadji$ be the degree matrix of $\adji$ and $\tadj = \dadji^{-1/2}\adji\dadji^{-1/2}$. 

Let $\tadj = \boldsymbol{E}\adjS\boldsymbol{E}$ be the eigendecomposition of $\tadj$. Then, the spectral convolution of $\feat$ on the graph $\adj$ can be defined via the reference operator $\tadj$ and a filter function $h$ operating on the eigenvalues, in the Fourier domain~\citep{tremblay2017design} as,
\begin{gather}
    \label{eq:spec_conv}
    Z = \boldsymbol{E}H(\adjS)\boldsymbol{E}X
\end{gather}
where $H(\adjS) = \textrm{diag}(h(\adjS))$. This process can be seen as the filter function adapting the graph for the desired task at hand. To tackle the problem of heterophily,~\citet{gprgnn} proposed a polynomial filter design, $H(\adjSv) = \sum_{i=1}^k \alpha_i \adjSv^i$ where $\alpha_i$'s are coefficients of the polynomial, $k$ is the order of the polynomial and $\adjSv$ is any eigenvalue from $\adjS$. Thus, $H(\adjS) = \textrm{diag}(V\boldsymbol{\alpha})$ where $V \in \real^{n \times k}$ is a Vandermonde matrix constructed using eigenvalues from $\adjS$ and $\boldsymbol{\alpha} \in \real^{k \times 1}$ is the vector consisting of $\alpha_j$'s. Thereby, we can write Equation~\ref{eq:spec_conv} as,
\begin{gather}
    \label{eq:spec_conv_poly_direct}
    Z = \boldsymbol{E}\textrm{diag}(V\boldsymbol{\alpha})\boldsymbol{E}X
\end{gather}
To avoid full eigendecomposition, Equation~\ref{eq:spec_conv_poly_direct} with the polynomial filter can be written as,
\begin{gather}
    \label{eq:spec_conv_poly}
    Z = \sum_{j=1}^k \alpha_j \tadj^j X
\end{gather}

 It is well-known that polynomial filters can approximate any graph filter \citep{shumangsp, tremblay2017design}. However, the inherent design of this model makes it less effective at learning a good polynomial filter. Let $h^*$ be the optimal filter for some given task, then comparing Equation~\ref{eq:spec_conv} and~\ref{eq:spec_conv_poly_direct}, we can see that for a fixed polynomial order $k$, the solutions for $\boldsymbol{\alpha}$ in Equation~\ref{eq:spec_conv_poly_direct} will be a superset of the solutions for the following linear system of equations,
\begin{gather}
    \label{eq:overdeterminedsystem}
    h^* = V\boldsymbol{\alpha}
\end{gather}
 Notice that, Equation~\ref{eq:overdeterminedsystem} is an overdetermined system of equations since the number of unknowns ($k$, the size of $\boldsymbol{\alpha}$) is less than the number of equations ($n$, the number of nodes). To obtain a consistent solution, we may have to work with higher-order polynomials. At higher powers, node features computed via $\tadj^jX$ becomes indistinguishable (see Figure~\ref{fig:indistinguishable}). Since the node features are indistinguishable, the importance of the coefficient associated with $\tadj^jX$ for the task at hand reduces significantly. We performed experiments by increasing the order of the polynomial. In Figure~\ref{fig:vary_order_cora} and~\ref{fig:vary_order_chameleon}, we plot the final task's accuracy for various polynomial orders. We observe that test accuracies do not improve significantly with an increase in the order of the polynomial. These observations are inline with Theorem 4.2 in~\citet{gprgnn}. It is noted in that Theorem that as the node features become indistinguishable (or over-smoothing happens), the corresponding coefficients of the polynomial go to zero. Now, one can avoid this issue with $\tadj^jX$ by directly working with Equation~\ref{eq:spec_conv_poly_direct}. However, this will incur the cost of doing full eigendecomposition, prohibitively expensive for large graphs. Even if we were to do this, $\adjSv_i$'s are in the range of $[-1, 1]$ and thus $\adjSv_i^j$ will diminish with higher powers. Thus, it will continue to be less effective in learning coefficients of a higher power. 
 
 To address the above problem, we propose to learn the polynomial filter as a sum of polynomials operating on different eigenvalue intervals. The next section is organized in the following way: 1] We gives detailed information about the model and the filter design, taking into account practical considerations of such an implementation. 2] We go ahead and show some of the properties of this filter design. We first show that our proposed filter design can approximate the latent optimal graph filter better than a single polynomial. As discussed earlier, the filter function adapts the graph for the desired task. We show that the possible learnable graphs via a single polynomial filter are a smaller subset of the learnable graphs via our proposed filter design. 3] Finally, we discuss the training and computational complexity of the proposed model.
 \begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[height=1.5in, width=0.95\textwidth]{iclr2022/images/Oversmoothening/cora_oversmoothening.png}
        \caption{}
        \label{fig:indistinguishable}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[height=1.5in, width=0.95\textwidth]{iclr2022/images/TA_Varying_K_GPRGNN/cora_TA_Varying_K_GPRGNN.png}
        \caption{}
        \label{fig:vary_order_cora}
    \end{subfigure}
    %\label{fig:fictitious}
    ~ 
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[height=1.5in, width=0.95\textwidth]{iclr2022/images/TA_Varying_K_GPRGNN/chameleon_pca_TA_Varying_K_GPRGNN.png}
        \caption{}
        \label{fig:vary_order_chameleon}
    \end{subfigure}
    \caption{In (a), we plot the average of pairwise distances between node features for the Cora dataset, after computing $\tadj^jX$ for increasing $j$ values. X-axis represents the various powers $j$ and the Y-axis represents the average of pairwise distances between node features. In (b) and (c), we plot the test accuracies of the model in \citet{gprgnn} for increasing order of polynomials for Cora and Chameleon dataset respectively. X-axis represents the order of the polynomial and Y-axis represents the test accuracy achieved for that order.}
\end{figure}


==> iclr2022/sections/preliminaries_old.tex <==
\section{Problem Setup and Motivation}

We focus on the problem of semi-supervised node classification on a simple graph $\graph = (\verts, \edges)$, where $\verts$ is the set of vertices and $\edges$ is the set of edges. Let $\adj \in \{0, 1\}^{n \times n}$ be the adjacency matrix associated with $\graph$, where $n = |\verts|$ is the number of nodes. Let $\mathcal{Y}$ be the set of all possible class labels. Let $\feat \in \real^{n \times d}$ be the $d$-dimensional feature matrix for all the nodes in the graph. Given a training set of nodes $\train \subset \verts$ whose labels are known, along with $\adj$ and $\feat$, our goal is to predict the labels of the remaining nodes. The proportion of edges that connect two nodes with the same labels in a graph is called the homophily score of the graph. In our problem, we are particularly concerned with graphs that exhibit low homophily scores. In the next sub-section, we provide background material on the GPR-GNN modelling method and its approach to graph adaptation.

\subsection{\gprgnn~Model}  
The \gprgnn~\citep{gprgnn} model consists of two core components: (a) a non-linear network that transforms raw feature input $\feat$: ${\bf Z}^{(0)} = f(\feat;{\mathbf W})$ and (b) a generalized page ranking (GPR) component, ${\mathbf G}$, that essentially aggregates  the transformed output ${\mathbf Z}$ recursively as: ${\bf Z}^{(k)} = \adj{\bf Z}^{(k-1)}, k = 1, \ldots, K$. Notice that there is no nonlinear operation involved after each aggregation step over $k$. Therefore, the functionality of the GPR component can be written using an operator ${\mathbf G}$ defined as: ${\mathbf G} = \sum_{k=0}^K \alpha_k {\mathbf A}^k$
and we obtain aggregated node embedding by applying ${\mathbf G}$ on the nonlinear network output:  ${\mathbf S} = {\mathbf G} {\mathbf Z}^{(0)}$. 
Using eigendecomposition, ${\adj} = \eigenU \adjS \eigenU^T$, \citet{gprgnn} presented an interpretation that the GPR component essentially performs a graph filtering operation: ${\mathbf G} = \eigenU h_K(\adjS) \eigenU^T$ where $h_K(\adjS)$ is a polynomial graph filter applied element-wise and $h_K(\adjSv_i) = \sum_{k=0}^K \alpha_k \adjSv^k_i$ where $\adjSv_i$ is the $i^{th}$ eigen value. As explained in~\citet{gprgnn}, learning filter coefficients (i.e.,$\alpha$) help to get improved performance. Since the coefficients can take negative values the \gprgnn~model is able to capture high-frequency components of the graph signals, enabling the model to achieve improved performance on heterophilic graphs. In the following subsection, we identify the inadequacies of \gprgnn.

\subsection{Motivation}  
\label{motivation}

\noindent\fbox{%
    \parbox{\textwidth}{%
    We plan to add the inadequacies of \gprgnn~in this section itself.
        \begin{enumerate}
            \item Now, for a fixed output $\bf Z_0$, \gprgnn~ tries to obtain the optimal value of the parameters of the filter $h_K$, which try to approximate the underlying waveform $h^*$ corresponding to the graph $\bf{A}$ and transformed features $\bf Z_0$. If we assume that the noise-less $h^*$ is fully observed on the interval [-1,1] and assuming it can be arbitrarily complex, then it can approximated it with using a very high degree polynomial, so it fits almost perfectly in [-1,1] (since this interval of interest is fully observed, any polynomial with appropriately high order can be made to fit the waveform with arbitrary accuracy (that depends on the choice of degree of the polynomial).
            \item But we observe that increasing the degree of polynomial in \gprgnn~does not generally leads to an increase in its performance. The reason behind this is the phenomenon of oversmoothing, that is observed for orders greater than some $K'$, such that for $K>K'$, the rows of matrix $\mathbf{A}^K\mathbf{X}$ approach a single vector with arbitrary proximity governed by $K$.
            \item We take a different way to approximate the waveform. (Need to cite those spline interpolation literature here), where it can be shown that, error bound in fitting a single spline to the waveform is more that the error achieved in fitting multiple independent splines defined on disjoint, mutually exclusive domains. The plots in Figure 1 demonstrate the idea where a single 10-degree polynomial fails to fit a fictitious waveform as compared to multiple 10-degree polynomials. We observe that even using multiple 5-degree polynomials performs much better than a single 1-degree polynomial as evident in figure 1(c).
            \item After this we define \textbf{Polynomial Adaptive Filters} like in Definition 3.1 whose definition naturally arises from the last point.
            \item We prove that least achievable approximation error by using one polynomial is higher than the least achievable approximation error obtained by using multiple adaptive filters. This is Theorem 3.1
            \item We theoretically show that a model with adaptive filters learns a more diverse set of graphs than \gprgnn, which includes \gprgnn's graphs as well. This is Theorem 3.2 and increasing the hypothesis space is reducing bias. To show that the extra graphs reachable by our model perform well, we add the plots/numbers of those experiments where only the $GL$ term is present. The graph family learnt by only $GL$ model is disjoint with the family learnt by \gprgnn, and yet the numbers/performance is competitive with our model and superior with \gprgnn~on heterophilic datasets and comparable on homophilic ones.
            \item $\left[\text{IN PROGRESS}\right]$ We show that our model's generalization error bound that grows slowly when we increase adaptive filters, as compared to when we increase $K$.

        \end{enumerate}
    }%
}

\cite{fagcn} and \cite{gprgnn} have shown the importance of low/high frequency components for the node classification task on graphs with varying levels of homophily. The polynomial graph filter described in \gprgnn~can, in theory, approximate any function given a high degree polynomial, but computing higher order terms is computationally intensive. Instead, we show that having polynomial adaptive filters on top of \gprgnn~help us to get a reduced error bound for the same degree polynomial as compared with \gprgnn.

\begin{definition}[Polynomial Adaptive Filter] A \textbf{polynomial adaptive filter}, denoted by $h_f(\adjS)$, is a polynomial filter (parameterized by polynomial $p$) whose frequency response acts only on a subset of the spectrum of the reference matrix. Given a support, $\mathbf\sigma_f\subset\mathbf\sigma(\mathbf A)$; $h_f(\adjSv) = \mathbbm{1}_{\adjSv\in\sigma_f}p(\adjSv)$.
\end{definition}

The following theorem shows that having an polynomial adaptive filter with a polynomial filter approximate any frequency response over the graph better than just the polynomial filter.

\begin{theorem}
For any frequency response $h^*$, and an integer $K\in\mathbb{N}/{\infty}$, let $\Tilde{h}:=h+h_f$, with $h_f$ having any random eigenvalue support $\sigma_f$, and let $\Hat{h}:=h$. Assuming $h$ and $h_f$ to be parameterized by $K$-order polynomials $p$ and $p_f$ respectively, then $\min\left\Vert\Tilde{h} - h^*\right\Vert_2\leq\min\norm{\Hat{h}-h^*}_2$. Moreover, for multiple polynomial adaptive filters $h_{f_1},h_{f_2},...,h_{f_m}$ with disjoint supports, the same inequality holds for $\Tilde{h} = h + \sum_{i=1}^m h_{f_i}$. The inequality can be made tighter by appropriate selection of support sizes.
\end{theorem}
\begin{proof}
For simplicity, we show the above bound for the case where the size of supports of all $h_{f_i}$ are equal, though following can be easily extended to unequal supports as well. We make the following assumptions:
\begin{enumerate}
    \item $\abs{\sigma_{f_i}}>K,\;\; \forall i\in[m]$
    \item All eigenvalues of the reference matrix are distinct
\end{enumerate}

For methods that use a single polynomial filter, the polynomial graph filter, $h_K(\adjS) = diag(\mathbf V\mathbf \gamma)$ where $\mathbf{\gamma}$ is a vector of coefficients, with sorted in descending order in components, and $\mathbf V$ is a Vandermonde matrix:
\begin{equation*}
\begin{aligned}
    \mathbf V = 
    \begin{bmatrix} 
    1&\lambda_1&\lambda_1^2&\cdots&\lambda_1^K\\ 
    1&\lambda_2&\lambda_2^2&\cdots&\lambda_2^K\\
    \vdots&\vdots&\vdots&\ddots&\vdots\\
    1&\lambda_n&\lambda_n^2&\cdots&\lambda_n^K\\\end{bmatrix}\\
\end{aligned}
\end{equation*}

And to approximate a frequency response $h^*$, we have the following objective:
\[
\min_{\gamma}\norm{diag(h^*) - diag(\mathbf V\gamma)}^2_F = \min_{\gamma}\norm{h^* - \mathbf V\gamma}^2_2
 \]
Where $\norm{}_F$ and $\norm{}_2$ are the Frobenius and $L_2$ norms respectively. Due to assumption 2, the system of equations $h^* = \mathbf V\gamma$ is well-defined and has a unique minimizer, say $\gamma^*$. Next we break the error vector as:
\begin{equation*}
\begin{aligned}
    \mathbf e_p &:= h^* - \mathbf V\gamma^* \\ 
    &= \sum_{i=1}^m (h^*_i - \mathbf V_i\gamma^*) + (h^*_L - \mathbf V_L\gamma^*)\\ 
    &= \sum_{i=1}^m \mathbf e_{p_i} + \mathbf e_{p_L}
\end{aligned}
\end{equation*}
Where $h^*_i$ is a vector whose value at components corresponding to the set $\sigma(h_{f_i})$ is same as that of $h^*$ and rest are zero. Similarly, $\mathbf V^*_i$ is a matrix whose rows corresponding to the set $\sigma(h_{f_i})$ are same as that of $\mathbf V$ with other rows being zero. Also, $\mathbf V_L = \mathbf V - \sum_{i=0}^m \mathbf V_i$ and $h^*_L = h^* - \sum_{i=0}^m h^*_i$. Note that by this construction, the vectors $\mathbf e_i$ form a linearly independent set.
Now, we analyze the case where we have polynomial adaptive filters added, where the objective is:
\[
\min_{\gamma,[\gamma_i]}\norm{diag(h^*) - diag\left(\mathbf V\gamma + \sum_{i=0}^m \mathbf V_i\gamma_i\right)}^2_F = \min_{\gamma, [\gamma_i]}\norm{h^* - \mathbf V\gamma - \sum_{i=0}^m \mathbf V_i\gamma_i}^2_2
\]
Before characterizing the above system, we break a general error vector as:
\begin{equation*}
\begin{aligned}
    \mathbf e_g &:= h^* - \mathbf V\gamma - \sum_{i=0}^m \mathbf V_i\gamma_i\\ 
    &= \sum_{i=1}^m (h^*_i - \mathbf V_i(\gamma + \gamma_i)) - (h^*_L - \mathbf V_L\gamma) \\ 
    &= \sum_{i=1}^m \mathbf e_{g_i} + \mathbf e_{g_L}
\end{aligned}
\end{equation*}
Clearly, the systems of equations, $\mathbf e_{g_i} = 0,\;\;\forall i$ and $\mathbf e_{g_L} = 0$ are well-defined. Since all the systems of equations have independent argument, unlike in the polynomial filter case where the optimization is constrained over a single variable; one can now resort to individual minimization of squared norms of $\mathbf e_{g_i}$ which results in a minimum squared norm of $\mathbf e_g$. Thus, we can set:
\[
\gamma = \mathbf V_L^{\dagger}h^*_L;\;\;\;\;\;\gamma_i = \mathbf V_i^{\dagger}h^*_i - \mathbf V_L^{\dagger}h^*_L,\;\;\forall i\in[m] 
\]
to minimize squared norms of $\mathbf e_{g_i}$ and $\mathbf e_{g_L}$. Since these form an orthogonal set, we have $\norm{\mathbf e_{g}}^2 = \sum_{i=1}^m\norm{\mathbf e_{g_i}}^2 + \norm{\mathbf e_{g_L}}^2$, and hence the above assignment leads to minimizing $\mathbf e_g$.

Clearly, $\norm{\mathbf e_{p_i}}^2\leq \norm{\mathbf e_{g_i}}^2$ and $\norm{\mathbf e_{p_L}}^2\leq \norm{\mathbf e_{g_L}}^2$ since the LHS in these inequalities is a solution of a constrained minimization problem, whereas the RHS comes from an unconstrained one.
Hence,
\[
\begin{aligned}
\sum_{i=1}^m\norm{\mathbf e_{p_i}}^2 + \norm{\mathbf e_{p_L}}^2 &\leq \sum_{i=1}^m\norm{\mathbf e_{g_i}}^2 + \norm{\mathbf e_{p_L}}^2 \\
\min\left\Vert\Tilde{h} - h^*\right\Vert &\leq \min\norm{\Hat{h}-h^*}
\end{aligned}
\]
\end{proof}

\begin{theorem}
Let $\mathbb{G}$ be the family of graphs learned by \gprgnn~, such that $\mathbb{G}:=\{\mathbf{U}^T h(\mathbf{\Lambda})\mathbf{U}\;|\;\forall\text{ possible K-degree polynomial parameterizations of }h\}$ for any unitary matrix $\mathbf{U}$. If $\mathbb{G}':=\{\mathbf{U}^T \Tilde{h}(\mathbf{\Lambda})\mathbf{U}\;|\;\forall\text{ possible K-degree polynomial parameterizations of }\Tilde{h}\}$ is the family of graphs learned by \ourmodel~, with $\Tilde{h} = h + h_{f_1} + h_{f_2}$, where $h$ is parameterized by a K-degree polynomial supported over entire spectrum, $h_{f_1}$ and $h_{f_2}$ are adaptive filters parameterized by independent K-degree polynomials supported over top and bottom $t$ eigenvalues respectively, with $t<n/2$; then $\mathbb{G}$ and $\mathbb{G}'$ form a subspace in $\mathbb{M}_{n\times n}[\mathbb{R}]$, with $\mathbb{G}\subset \mathbb{G}'$. Also, $\frac{\text{dim}(\mathbb{G}')}{\text{dim}(\mathbb{G})} = 3$.
\end{theorem}
\begin{proof}
Consider the set of all the univariate polynomials having degree at most $K$ in the vector space over the ring $\mathbb{K}[x_1,\ldots,x_n]$ where $\mathbb{K}$ is the field of real numbers. Partition this set into $n$ subsets, say $V_1,\ldots,V_n$, such that for $i\in[n]$,  $V_i$ contains all polynomials of degree up to $K$ in $x_i$. It is easy to see that $V_1,\ldots,V_n$ are subspaces of $\mathbb{K}[x_1,\ldots,x_n]$. Define $V = V_1 \oplus V_2 \oplus \cdots \oplus V_n$. Define the matrix $D_{i}[c]$ whose $(i,i)^{\text{th}}$ entry is $c$ and all the other entries are zero. For $i\in[n]$, define a linear map $\phi_i:V_i \rightarrow \mathbb{M}_{n\times n}\left(\mathbb{R}\right)$ by $f(x_i)\mapsto D_{i}[f(\lambda_i)]$. Im($\phi_i$) forms a vector space of all diagonal matrices, whose $(i,i)$ entry is the evaluation of an element of $V_i$ at $\lambda_i$.
Generate a linear map $\phi:V\rightarrow \mathbb{M}_{n\times n}(\mathbb{R})$ by mapping $\phi(f(x_i))$ to $ \phi_i(f(x_i))$ for all $i\in[n]$. Note that $\phi_i$ for $i\in[n]$ are injective maps, making $\phi$ an injective map. Observe that $h(\mathbf{\Lambda})\subset \text{Im}(\phi)$ is a subspace with basis $\mathcal{B}_h:=$ $\{\phi(1+\cdots+1), \phi(x_1+\cdots+x_n), \ldots, \phi(x_1^K+\cdots+x_n^K)\}$, making $\text{dim}(h(\mathbf{\Lambda})) = K+1$. Similarly we have, $h'(\mathbf{\Lambda})\subset \text{Im}(\phi)$, a subspace with basis $\mathcal{B}_{h'}:=\mathcal{B}_h \bigcup\;\{\phi(1+\cdots+1+0+\cdots+0), \phi(x_1+\cdots+x_t+0+\cdots+0), \ldots, \phi(x_1^K+\cdots+x_t^K+0+\cdots+0)\}\bigcup\;\{\phi(0+\cdots+0+1+\cdots+1), \phi(0+\cdots+0+x_{n-t+1}+\cdots+x_n), \ldots, \phi(0+\cdots+0+x_{n-t+1}^K+\cdots+x_n^K)\}$, implying $h(\mathbf{\Lambda})\subset h'(\mathbf{\Lambda})$ and $\text{dim}(h'(\mathbf{\Lambda})) = 3(K+1)$. Consider the injective linear maps $f_1,f_2:\mathbb{M}_{n\times n}(\mathbb{R})\rightarrow \mathbb{M}_{n\times n}(\mathbb{R})$ as $f_1(\mathbf{A})=\mathbf{U}^T\mathbf{A}$ and $f_2(\mathbf{A})=\mathbf{AU}$. Define $f_3: \text{Im}(\phi) \rightarrow \mathbb{M}_{n\times n}(\mathbb{R})$ as $f_3(\mathbf A) = (f_1\circ f_2)(\mathbf A)$. Since $f_3$ is a monomorphism, we have $\mathbb{G}\subset \mathbb{G}'$.
\end{proof}

\begin{corollary}
For a frequency response $h^*$ belonging to a set of absolute minimizers of the downstream task objective corresponding to the optimal error corresponding to any $\Theta$, use of polynomial adaptive filters achieve a lower error in approximating $h^*$ than \gprgnn~and Linear Graph Convolution (LGC) methods. Specificially for node classification, $\Tilde{h}\in \argmin_h[\min_{\Theta} \norm{\mathbf{Y} - softmax(\eigenU h(\adjS)\eigenU^Tf_{\Theta}(\mathbf X)}_F^2]$, where $f_{\Theta}$ is a (non) linear down-scaling function. Minimizing the cross-entropy error is approximately equivalent to approximating the response $\Tilde{h}$ above.
\end{corollary}
\begin{proof}
We start by bounding the cross-entropy loss similar to \cite{errorcomp}. Let $q(\cdot|x_i):=softmax(\eigenU h(\adjS)\eigenU^Tf_{\Theta}(\mathbf X)$ where the softmax is applied along the rows of its argument. Denote the true label of node $i$ as $y_i$ We define the cross-entropy and MSE loss as:
\[
\begin{aligned}
\mathcal{L}_{xent} &= -\sum_{i=1}^n [\ln q(y_i|x_i)]\\
\mathcal{L}_{MSE} &= \sum_{i=1}^n\sum_{y=1}^c [\delta(y,y_i) - q(y|x_i)]^2
\end{aligned}
\]
While cross-entropy is only defined over the model's score for the correct label, MSE is defined over model's score for all the labels, making it difficult to directly compare it with the cross-entropy. We instead try to get the upper and lower bounds for the MSE. For any node $i$, the cost term for MSE is 
\[
\mathcal{L}_{MSE,i} = \sum_{y=1}^c [\delta(y,y_i) - q(y|x_i)]^2 = (1-q(y_i|x_i))^2 + \sum_{y\neq y_i} q(y|x_i)^2
\]
Now by definition, every component of $q(\cdot|x_i)$ is positive. Hence, we have: 
\[
\sum_{y\neq y_i} q(y|x_i)^2 \leq \left(\sum_{y\neq y_i} q(y|x_i)\right)^2 = \left(1-q(y_i|x_i)\right)^2
\]
Thus,
\[
\mathcal{L}_{MSE,i} \leq 2\left(1-q(y_i|x_i)\right)^2 < -\ln q(y_i|x_i) = \mathcal{L}_{xent, i} \\
\]
The second inequality holds since $q(y_i|x_i) \in (0,1)$. Above result implies that the upper bound of MSE is strictly bounded above by the cross-entropy loss. Thus by minimizing the cross-entropy, one also minimizes the MSE, and it is easy to see that:

\begin{equation*}
\begin{split}
\mathcal{L}_{MSE} & = \norm{\mathbf{Y} - softmax(\eigenU h(\adjS)\eigenU^Tf_{\Theta}(\mathbf X))}_F^2 \\
&= \norm{\mathbf{Y} - softmax(\eigenU h^*(\adjS)\eigenU^Tf_{\Theta}(\mathbf X) + softmax(\eigenU h^*(\adjS)\eigenU^Tf_{\Theta}(\mathbf X) - softmax(\eigenU h(\adjS)\eigenU^Tf_{\Theta}(\mathbf X)}_F^2 \\
&\leq \norm{\mathbf{Y} - softmax(\eigenU h^*(\adjS)\eigenU^Tf_{\Theta}(\mathbf X)}_F^2  + \norm{softmax(\eigenU h^*(\adjS)\eigenU^Tf_{\Theta}(\mathbf X) - softmax(\eigenU h(\adjS)\eigenU^Tf_{\Theta}(\mathbf X)}_F^2 \\
&\leq \norm{softmax(\eigenU h^*(\adjS)\eigenU^Tf_{\Theta}(\mathbf X) - softmax(\eigenU h(\adjS)\eigenU^Tf_{\Theta}(\mathbf X)}_F^2 \\
&\leq \norm{\eigenU h^*(\adjS)\eigenU^Tf_{\Theta}(\mathbf X - \eigenU h(\adjS)\eigenU^Tf_{\Theta}(\mathbf X}_F^2\\
&=\norm{\eigenU (h^*(\adjS) - h(\adjS))\eigenU^Tf_{\Theta}(\mathbf X)}
\end{split}
\end{equation*}

The second inequality results from the term $\norm{\mathbf{Y} - softmax(\eigenU h^*(\adjS)\eigenU^Tf_{\Theta}(\mathbf X)}_F^2$ being independent of $h$. The third inequality results from the standard softmax being an 1-Lipschitz function. Thus, when we minimize the classification objective, we also end up minimizing the MSE. Since $\Tilde{h},\Tilde{\Theta}=\argmin_{h.\Theta}\mathcal{L}_{MSE}$ define the best performing model for the observed graph data in the \ourmodel~family, this defines the lower bound on the achievable MSE across all models in the \ourmodel~family. Now, it follows from Theorem 3.1 that the frequency response corresponding to this lower bound achievable by any model in \ourmodel~family is closer to the observed frequency response than the family of models relying on a polynomial filter.
\end{proof}

Theorem 3.1 implies that polynomial adaptive filters better approximate the frequency response, since they provide flexibility to adapt to specific regions of the spectrum providing a local control over it, without any dependence on the other regions, unlike their single polynomial counterparts which try to adapt to all eigenvalues at once thereby limiting the model flexibility. Thus adaptive filters eliminate the need of increasing the polynomial order while simultaneously achieving the better approximation. Since we do not have access to $h^*$ in order to correctly approximate $\Tilde{h}$, we do so approximately via minimizing a downstream objective like the cross-entropy objective for the node classification. This comes from the intuition that the observed labels are the function of the optimal frequency response.

% To support the argument that GPR-GNN as well our proposed approach reduces to solving a system of equations as shown in theorem 3.1, given a fixed input functional transformation, we can construct the following thought experiment.\\
% ----------------------------------------------------------------------

% \textbf{Possible argument for adding MLP} (Appendix):

% The questions that we still have to answer are the following:

% 1. How do we connect solving a system of equations to GPR-GNN\\
% 2. We then have to show how our approach ends up performing better. I think this is well known. 1 is not very well understood. I will try to use some intuition to connect 1 with GPR-GNN and then we can discuss that.

% Lets consider that we have a fixed functional transformation (instead of a learnable one) given by $f$. Then solution that GPR-GNN is trying to find out reduces to the following:

% \begin{equation}
%     \gamma^* = min_{\gamma} \sum_{i=1}^{N}H(y_i, softmax(\hat{y}_i))
% \end{equation}

% Where $H$ is the cross entropy, $N$ is the number of nodes, and $\hat{y}$ is defined as follows:

% %\begin{equation}
% %    \hat{y} = \sum_{k=1}^{M}\gamma_{k} A^{k} f(X)
% %\end{equation}

% %\begin{equation}
% %    \hat{y} = \sum_{k=1}^{M} \gamma_{k}U  \Lambda^k U^T f(X)
% %\end{equation}

% \begin{equation}
%     \hat{y} =  U  diag(V \gamma) U^T f(X)
% \end{equation}

% Let $y^*$ be the $\hat{y}$ that corresponds to the optimal solution. Let the filter response that corresponds to $y^*$ be h. Therefore:

% \begin{equation}
%     y^* =  U  diag(h) U^T f(X)
% \end{equation}

% Now from equation 2 and 3 we can observe that for GPR-GNN to approach the optimal solution, we need $\hat{y} \approx y^*$ when then implies $diag(V\gamma) \approx diag(h) \implies V\gamma \approx h$. Hence we can conjecture that given a fixed functional transformation, all GPR-GNN is learning is an optimal $\gamma$ that satisfies $V \gamma \approx h$ which can be obtained by solving a system of linear equations: $h = V\gamma$. Hence we can reduce the entire GPR-GNN model to solving a linear system of equations. \\
% ----------------------------------------------------------------------

% End to end error analysis:

% Let the output filtered graph signal that gives the best classification accuracy be defined as follows:

% \begin{equation*}
%     x^* = Udiag(h)U^Tf_{*}(X)    
% \end{equation*}

% Note that $h$ and $f_*$ are the ideal filter response and the ideal functional transformation of the input graph signal respectively. There can be multiple such $h$ and $f_*$ that would give a good classification accuracy. We pick one amongst the solution set.

% Let the output of the GPR-GNN model be defined as follows:

% \begin{equation*}
%     \tilde{x} = Udiag(V\gamma)U^Tf_{\theta}(X)    
% \end{equation*}

% The error due to GPR-GNN not being an exact solution can be seen as follows:

% \begin{equation*}
% \begin{aligned}
%     e = Udiag(h)U^Tf_{*}(X) - Udiag(V\gamma)U^Tf_{\theta}(X) \\
    
% \end{aligned}
% \end{equation*}


--------------------------------

Next, to empirically validate the results, we performed experiments on a complex, fictitious waveform where we demonstrate that a single polynomial performs poorly in approximating the waveform as compared to polynomial with polynomial adaptive filters applied. The corresponding plots are shown in Figure 1. Clearly, due to local flexibility of the adaptive filters, we can better approximate for the waveform without increasing the polynomial degree. We refer the reader to Appendix X, where we demonstrate that fits of comparable approximation error can be achieved by even a much lower degree polynomial, an observation that we exploit to achieve comparable performance on the downstream task using a scaled-down model.

\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[height=1.5in, width=0.95\textwidth]{figs/gprgnn_order10.png}
        \caption{Fitting single 10-degree polynomial}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[height=1.5in, width=0.95\textwidth]{figs/adafilt_order10.png}
        \caption{Fitting 10-degree polynomial with adaptive filters}
    \end{subfigure}
    %\label{fig:fictitious}
    \caption{To demonstrate the adaptability of adaptive polynomial filter, we try to approximate a complex waveform (blue dashed line) via (a) a single 10 degree polynomial, and (b) a 10-degree polynomial with 10 adaptive filters. The waveform learnt via the filter is shown in a solid dashed line. The corresponding RMSE are: (a) 3.9011, (b) 0.1824}
\end{figure}

\todo{For the proof:\\
    i) [\textbf{DONE}] From DSP, how frequency response of graph filter leads to solving system of equations: \\
    ii) [\textbf{DONE}] How h($\Lambda$), in \gprgnn, can be written as Vandermonde matrix \\
    iii) [\textbf{DONE}] Overdetermined/Underdetermined system based on how we partition these system of equations and solve the coefficients \\
    iv) [\textbf{DONE}] Talk about residual error for each case: 1) using single polynomial, 2) using multiple polynomials, and 3) a polynomial for every eigen component\\
    v) [\textbf{DONE}] Empirically show what happens to residual error as we increase number of polynomials (Fictitious waveform experiment)\\
    vi) [\textbf{DONE}] We also need to consider the effect of $f(X)$. We can probably write the alternative interpretation as a loose theorem or at the worst case a conjecture. However such a similar process would have to be done for our G+GL model as well.\\
    vii) Reframe theorem 3.1 and Corollary 3.1.1 into a) Lemma 1: Cross entropy minimization leads to MSE minimization; b) Solving h=V$\gamma$ leads to MSE minimization c) Theorem: multiple polynomials approximate $h^*$ better than single polynomial and d) a corollary that connects end-to-end: cross-entropy minimization gives better results for \ourmodel~than \gprgnn. Now to cover up the loose connection b/w lemma 1 and 2, we'll use the word 'approximately' in corollary.

\vspace{0.12in}

For the writing part for the motivation: \\   
1) [\textbf{DONE}] Introduce what having multiple adaptive filters upon GPRGNN mean \\
2) [\textbf{DONE}] State the theorem that having different adaptive filters can approximate any frequency response better than GPRGNN\\
3) [\textbf{DONE}] Then we can show empirical results on fictitious waveforms.\\
4) [\textbf{DONE}] Talk about scalability issues as well\\
5) Talk about oversmoothing as another possible drawback when increasing the polynomial order.
}
%Previous Motivation%
% We conduct the following empirical experiment to infer if a higher order polynomial is required for heterophilic datasets. We consider the eigendecomposition of given graph as ${\adj} = \eigenU \adjS \eigenU^T$ and we assign the node features as $\eigenU \adjS^{\frac{1}{2}}$. The columns in this feature matrix are essentially the eigenvectors. We construct new training data with these features using the known labels from training set~$\train$. We train a Logistic Regression model with this data. We perform max pooling on the per-class weights learned by the model and depict this in Figure~\ref{fig:polyAnalysis}. Max pooling reveals the highest weight required by the corresponding class for a given node. We also plot a closest fit polynomial on these weighted eigenvalues. We observe that in both Chameleon and Squirrel datasets, a polynomial with order as high as 70 is required to capture finer subtleties. 

% We conjecture that a sophisticated  adaptation function, or a high degree polynomial might be required for further improvement in performance. A simple fix to achieve this would be to increase the order of polynomial learned in \gprgnn. However, as reflected in Table XXX, we observe that increasing the polynomial order does not translate to improvement in performance and in some cases leads to degradation. Computing higher powers of the input graph leads to the oversmoothing problem (CITE XXX). Also, from a practical view, it is infeasible to compute powers of a large graph. Computationally this can also lead to numerical instabilities. In the next section, we present our proposed approach that addresses these inadequacies. 

==> sections/abstract.tex <==
\begin{abstract}
Graph Neural Networks (GNNs) exploit signals from node features and the input graph topology to improve node classification task performance. However, these models tend to perform poorly on heterophilic graphs, where connected nodes have different labels. Recently proposed GNNs work across graphs having varying levels of homophily. Among these, models relying on polynomial graph filters have shown promise. We observe that solutions to these polynomial graph filter models are also solutions to an overdetermined system of equations. It suggests that in some instances, the model needs to learn a reasonably high order polynomial. On investigation, we find the proposed models ineffective at learning such polynomials due to their designs. To mitigate this issue, we perform an eigendecomposition of the graph and propose to learn multiple adaptive polynomial filters acting on different subsets of the spectrum. We theoretically and empirically show that our proposed model learns a better filter, thereby improving classification accuracy. We study various aspects of our proposed model including, dependency on the number of eigencomponents utilized, latent polynomial filters learned, and performance of the individual polynomials on the node classification task. We further show that our model is scalable by evaluating over large graphs. Our model achieves performance gains of up to 10\% over the state-of-the-art models and outperforms existing polynomial filter-based approaches in general. 

% Our anonymized code is available at \url{https://tinyurl.com/PPGNN}.
\end{abstract}


% {Should we add Reddit numbers or mention it somewhere? We don't have all baseline numbers for Reddit though. Mentioning large graphs sets some expectation.}

==> sections/approach_V1.tex <==
\section{Proposed Approach}
\label{sec:proposedapproach}

\subsection{Piece-wise Polynomial/Spline Graph Filter Function}
The goal of our proposed modeling approach is to get improved task specific performance by learning effective task-specific graph filters. We learn better graph filters by using a richer class of parameterized frequency filter functions and optimizing task-specific loss function over filter parameters. We model the filtering function $h(\lambda)$ as a piece-wise polynomial or spline function where each polynomial is lower degree (e.g., a cubic polynomial). We partition the eigen-spectrum in $[-1,1]$ (or $[0,2]$ as needed) into contiguous intervals and approximate the desired frequency response by fitting a low degree polynomial in each interval. This helps us to learn more complex shaped frequency response that is optimized for each task.  

Let $\sigma = \{\sigma_1,\sigma_2,\ldots,\sigma_m\}$ denote a partition set with $m$ contiguous intervals and  $h_{i,k_i}(\lambda;\gamma_i)$ denote a $k_i$-degree polynomial filter function of the interval $\sigma_i$ with polynomial coefficients $\gamma_i$. We define PP-GNN filter function as: 
\begin{equation}
    h(\lambda) = \sum_{i=1}^m h_{i,k_i}(\lambda;\gamma_i)
\label{eq:PPFF-GNN}
\end{equation}
and learn a smooth filter function by imposing additional constraints to maintain continuity between polynomials of contiguous intervals at different endpoints (\textit{aka} knots). This class of filter functions is rich, and its complexity is controlled by choosing intervals (i.e., endpoints and number of partitions) and polynomial degrees. Given the filter function, we compute the node embedding matrix as: 
\begin{equation}
    \mathbf{Z} = \sum_{i=1}^m \eigenU_i H_i(\mathbf{\gamma}) \eigenU^T_i {\mathbf Z}_0(\mathbf{X;\Theta})
\label{eq:nodeemb}    
\end{equation}
where $\eigenU_i$ is a matrix with eigenvectors corresponding to eigenvalues that lie in $\sigma_i$. 

\subsection{Practical and Implementation Considerations}
The filter function (\ref{eq:nodeemb}) requires computing eigendecomposition of $\hat{\mathbf{A}}$ and is expensive, therefore, not scalable for very large graphs. Thus, having finer control to learn complex frequency responses comes with a high computational cost. We address this problem by devising a graph filter function that enables trade-off between computational cost and frequency response control. First, we make the following observations: 
\begin{enumerate}
    \item Top-k and bottom-k eigenvalues represent $k$ low and high frequencies. There are efficient algorithms and off-the-shelf library packages available to get top-k and bottom-k eigenvalues and eigenvectors of sparse matrices. 
\item GPR-GNN method also learns a graph filter but operates on the entire eigen-spectrum by sharing the filter coefficients across the spectrum. Therefore, it can be seen as a special case of our proposed model (\ref{eq:nodeemb}). Since GPR-GNN learns a global polynomial by having shared coefficients across the spectrum (like learning a global polynomial to fit a function) it is not flexible enough to learn complex frequency responses, as needed in several practical applications. Note that increasing the degree of the global polynomial does not help beyond some high degree specific to tasks. We demonstrate this through extensive experiments on benchmark datasets in the experiment and appendix sections. One important advantage of GPR-GNN is that it does not require computation of eigendecomposition, therefore, efficient. 
  \item 
    Many recent works including GPR-GNN investigated the problem of designing robust graph neural networks that work well across homophilic and heterophilic graphs. They found that graph filters that amplify or attenuate low and high frequency components of signals (i.e., low-pass and high-pass filters) are critical to get improved performance on several benchmark datasets.
\end{enumerate}
\textbf{Efficient Variant.} Using the above observations, we propose an efficient variant of (\ref{eq:PPFF-GNN}) as: 
\begin{equation}
    {\tilde h}(\lambda) = \eta_l \sum_{i=1}^{m_l} h^{(l)}_{i}(\lambda;\gamma^{(l)}_i) + \eta_h \sum_{i=1}^{m_h} h^{(h)}_{i}(\lambda;\gamma^{(h)}_i) +  \eta_{gpr} h_{gpr}(\lambda;\gamma)
  \label{eq:PPFF-GNN-EFF}
\end{equation}
where the first and second terms fit piece-wise polynomials\footnote{For brevity, we dropped the polynomial degree dependency.} in low and high frequency regions, as indicated through superscripts. However, we do not want to lose any useful information from other frequencies in the central region yet maintain efficiency. We achieve this by adding the GPR-GNN filter function, $h_{gpr}(\lambda;\gamma)$, which is computationally efficient. Since $h_{gpr}(\lambda;\gamma)$ is a special case of (\ref{eq:PPFF-GNN}) and the terms in (\ref{eq:PPFF-GNN-EFF}) are additive, it is easy to see that (\ref{eq:PPFF-GNN-EFF}) is same as (\ref{eq:PPFF-GNN}) with a modified set of polynomial coefficients. In practice, the required low and high frequency components are computed based on affordable computational cost. Furthermore, contributions from each term could be controlled by setting or optimizing over hyperparameters, $\eta_l$, $\eta_h$ and $\eta_{gpr}$. Thus, the proposed model offers richer capability and flexibility in learning complex frequency response and balancing computation cost over GPR-GNN.       

\textbf{Model Training.} Like GPR-GNN, we apply $\textsc{Softmax}$ activation function on (\ref{eq:nodeemb}) and use the standard cross-entropy loss function to learn the sets of polynomial coefficients ($\gamma$) and classifier model parameters ($\Theta$) using labeled data. To ensure smoothness of the learned filter functions, we add a regularization term that penalizes squared differences between the function values of polynomials of contiguous intervals at each other's interval end-points. More details are available in the experiment and appendix sections.  

\textbf{Computational Cost.} There is some pre-training cost of computing the eigendecomposition ($O(n^2k)$)[\sundar{Manan - can you please in Golub and VanLoan book and refer one of the best algorithms and write the cost. That should suffice!}]. Node embedding is computed fresh Whenever the model parameters are updated and this computation involves matrix multiplication with eigenmatrices incurring an additional cost (over GPR-GNN) of $O(nkL)$ where $k$ and $L$ denote the number of selected low/high eigenvalues and classes respectively. 

\subsection{Analysis}
We first give a simple theoretical justification for using multiple polynomials by upper-bounding the error that the optimal approximation such an approximation achieves by the error that the single polynomial parameterization achieves. We relegate the proofs of all the theorems of this section to appendix.

\begin{theorem}
\label{thm:better_approximation}
For any frequency response $h^*$, and an integer $K\in\mathbb{N}/{\infty}$, let $\Tilde{h}:=h+h_f$, with $h_f$ having any random eigenvalue support $\sigma_f$. Assuming $h$ and $h_f$ to be parameterized by $K$-order polynomials $p$ and $p_f$ respectively, then $\min\|\Tilde{h} - h^*\|_2\leq \min\|h-h^*\|_2$. Moreover, for multiple polynomial adaptive filters $h_{f_1},h_{f_2},...,h_{f_m}$ parameterized by independent K-degree polynomials but having disjoint, contiguous supports, the same inequality holds for $\Tilde{h} = h + \sum_{i=1}^m h_{f_i}$.
\end{theorem}

%The proof naturally arises from simple algebraic constructions. One can now think of the adaptive filters as providing better local control over the polynomial fit, adding more degrees of freedom on its support, and hence resulting in a better fit. But since the spectrum of the reference matrix is $[-1,1]$, controlling the lower order terms is more important that fitting the higher order terms, which can be achieved by using adaptive filters parameterized by a lower degree polynomial. One can show by a simple construction that the optimal approximation error by using such filters is still lower than the one achievable by a globally defined polynomial.

\begin{corollary}
\label{thm:lower_than_k}
If the adaptive filters $h_{f_1},h_{f_2},...,h_{f_m}$ are parameterized by independent polynomials having degree $K'\leq K$, and let $h$ be parameterized by a K-degree polynomial, then $\|\Tilde{h} - h^*\|_2\leq \min\|h-h^*\|_2$.
\end{corollary}

We constructed wave-forms of arbitrary complexity, which were then approximated by first fitting a single globally-defined polynomial and then by adding locally defined polynomials on top of it.  We assess the performance by varying the degrees of the local polynomials. The corresponding plots are present in [\ms{Refer to Appendix}] Figure~\ref{fig:fictitious}~which indicate that use of lower-order filters achieves a fit comparable to one by a relatively higher-degree polynomial. Since a real waveform isn't observed in practice and is estimated by optimizing over the observed labels via learning a graph filter, we theoretically show that the family of filters that we learn is a strict superset of the polynomial filter family. The same result is shown to hold true for the families of the resulting adapted graphs.



\begin{theorem}
\label{thm:space_of_filters}
Define $\mathbb{H}:=\{h(\mathbf{\Lambda})\;|\;\forall\text{ possible K-degree polynomial parameterizations of }h\}$ to be the set of all K-degree polynomial filters with diagonal evaluation. Similarly $\mathbb{H}':=\{ \Tilde{h}(\mathbf{\Lambda})\;|\;\forall\text{ possible polynomial parameterizations of }\Tilde{h}\}$ is set of all filters learn-able via \ourmodel~, with $\Tilde{h} = h + h_{f_1} + h_{f_2}$, where $h$ is parameterized by a K-degree polynomial supported over entire spectrum, $h_{f_1}$ and $h_{f_2}$ are adaptive filters parameterized by independent K'-degree polynomials supported over top and bottom $t$ eigenvalues respectively, with $t<n/2$ and $K'\leq K$; then $\mathbb{H}$ and $\mathbb{H}'$ form a vector space, with $\mathbb{H}\subset \mathbb{H}'$. Also, $\frac{\text{dim}(\mathbb{H}')}{\text{dim}(\mathbb{H})} = \frac{K+2K'+3}{K+1}$.
\end{theorem}

\begin{corollary}
\label{thm:space_of_graphs}
The corresponding adapted graph families $\mathbb{G}:=\{\mathbf{U}^T h(\mathbf{\Lambda})\mathbf{U}^T\;|\;\forall h(\mathbf{\Lambda})\in\mathbb{H}\}$ and $\mathbb{G'}:=\{\mathbf{U}^T \Tilde{h}(\mathbf{\Lambda})\mathbf{U}^T\;|\;\forall \Tilde{h}(\mathbf{\Lambda})\in\mathbb{H}'\}$ for any unitary matrix $\mathbf{U}$ form a vector space, with $\mathbb{G}\subset \mathbb{G}'$ and $\frac{\text{dim}(\mathbb{G}')}{\text{dim}(\mathbb{G})} = \frac{K+2K'+3}{K+1}$.
\end{corollary}

This implies that our model is learning from a more diverse space of adapted graphs. Moreover, the dimension of this became three-fold by using just two adaptive filters. To justify that learning from such diverse region is feasible, we first note from the proofs of Theorem 4.2 and Corollary 4.2.1, that using the adaptive filters without any filter with entire spectrum as support, results in learning a set of adapted graphs, $\hat{\mathbb{G}}$, that is disjoint from $\mathbb{G}$, with $\mathbb{G'}=\mathbb{G}\oplus\hat{\mathbb{G}}$. We conduct various ablative studies where we demonstrate the effectiveness of learning from $\hat{\mathbb{G}}$ and $\mathbb{G'}$.

%We set up an experiment, where we learn an adapted graph from the disjoint family, $\hat{\mathbb{G}}$, and compare our results with \gprgnn, which learns from $\mathbb{G}$. Our experiments on multiple datasets result in a significant lift in performance on the graphs with lower homophily score, and a competitive performance on the graphs with higher homophily score. \ms{This section can be moved to answer RQ3 in Experiments}. 

%\begin{enumerate}
%    \item Relate to theoretical/analytical results of the %previous section to contrast GPR-GNN with our model. 
%\end{enumerate}


==> sections/approach_V2.tex <==
\section{Proposed Approach}
\label{sec:proposedapproach}
The central goal of our approach is to get improved task-specific performance by learning effective task-specific graph filters. We propose to learn the polynomial filter as a sum of polynomials operating on different eigenvalue intervals, taking task-specific requirements and practical considerations into account. We show that our proposed filter design can approximate the latent optimal graph filter better than a single polynomial, and the resultant class of learnable filters/graphs is richer. We briefly discuss the training and computational complexity of the proposed model.
\subsection{Piece-wise Polynomial/Spline Graph Filter Function}
 We model the filtering function $h(\lambda)$ as a piece-wise polynomial or spline function where each polynomial is of a lower degree (e.g., a cubic polynomial). We partition the eigen spectrum in $[-1,1]$ (or $[0,2]$ as needed) into contiguous intervals and approximate the desired frequency response by fitting a low degree polynomial in each interval. This process helps us to learn a more complex shaped frequency response as needed for the task.  
Let $\mathcal{S} = \{\sigma_1,\sigma_2,\ldots,\sigma_m\}$ denote a partition set with $m$ contiguous intervals and  $h_{i,k_i}(\lambda;\gamma_i)$ denote a $k_i$-degree polynomial filter function of the interval $\sigma_i$ with polynomial coefficients $\gamma_i$. We define PP-GNN filter function as: 
\begin{equation}
    h(\lambda) = \sum_{\sigma_i \in \mathcal{S}} h_{i,k_i}(\lambda;\gamma_i)
\label{eq:PPFF-GNN}
\end{equation}
and learn a smooth filter function by imposing additional constraints to maintain continuity between polynomials of contiguous intervals at different endpoints (\textit{aka} knots). This class of filter functions is rich, and its complexity is controlled by choosing intervals (i.e., endpoints and number of partitions) and polynomial degrees. Given the filter function, we compute the node embedding matrix as: 
\begin{equation}
    \mathbf{Z} = \sum_{i=1}^m \eigenU_i H_i(\mathbf{\gamma_i}) \eigenU^T_i {\mathbf Z}_0(\mathbf{X;\Theta})
\label{eq:nodeemb}    
\end{equation}
where $\eigenU_i$ is a matrix with eigenvectors corresponding to eigenvalues that lie in $\sigma_i$, $H_i(\gamma_i)$ is the diagonal matrix with diagonals containing the $h_i$ evaluated at the eigenvalues and ${\mathbf Z}_0(\mathbf{X;\Theta})$ is an MLP network with parameters $\mathbf{\Theta}$.

\subsection{Practical and Implementation Considerations}
The filter function (\ref{eq:nodeemb}) requires computing eigendecomposition of $\tadj$ and is expensive, therefore, not scalable for very large graphs. Thus, having finer control to learn complex frequency responses comes with a high computational cost. We address this problem by devising a graph filter function that enables a trade-off between computational cost and frequency response control. First, we make the following observations: 
\begin{enumerate}
    \item Top-k and bottom-k eigenvalues represent $k$ low and high frequencies. There are efficient algorithms and off-the-shelf library packages available to get top-k and bottom-k eigenvalues and eigenvectors of sparse matrices. 
    \item GPR-GNN method also learns a graph filter but operates on the entire eigen spectrum by sharing the filter coefficients across the spectrum. Therefore, it is a special case of our proposed model (\ref{eq:nodeemb}). Since GPR-GNN learns a global polynomial by having shared coefficients across the spectrum (like learning a global polynomial to fit a function), it is not flexible enough to learn complex frequency responses, as needed in several practical applications. Note that increasing the degree of the global polynomial does not help beyond some high degree specific to tasks. We demonstrate this through extensive experiments on benchmark datasets in the experiment and appendix sections. One important advantage of GPR-GNN is that it does not require computation of eigendecomposition; therefore, efficient. 
    \item Many recent works, including GPR-GNN, investigated the problem of designing robust graph neural networks that work well across homophilic and heterophilic graphs. They found that graph filters that amplify or attenuate low and high-frequency components of signals (i.e., low-pass and high-pass filters) are critical to improving performance on several benchmark datasets.
\end{enumerate}
\textbf{Efficient Variant.} Using the above observations, we propose an efficient variant of (\ref{eq:PPFF-GNN}) as: 
\begin{equation}
    {\tilde h}(\lambda) = \eta_l \sum_{\sigma_i \in \mathcal{S}^l} h^{(l)}_{i}(\lambda;\gamma^{(l)}_i) + \eta_h \sum_{\sigma_i \in \mathcal{S}^h} h^{(h)}_{i}(\lambda;\gamma^{(h)}_i) +  \eta_{gpr} h_{gpr}(\lambda;\gamma)
  \label{eq:PPFF-GNN-EFF}
\end{equation}
where $\mathcal{S}^l$ consists of partitions over low frequency components, $\mathcal{S}^h$ consists of partitions over high frequency components, the first and second terms fit piece-wise polynomials\footnote{For brevity, we dropped the polynomial degree dependency.} in low and high frequency regions, as indicated through superscripts. However, we do not want to lose any useful information from other frequencies in the central region, yet maintain efficiency. We achieve this by adding the GPR-GNN filter function, $h_{gpr}(\lambda;\gamma)$, which is computationally efficient. Since $h_{gpr}(\lambda;\gamma)$ is a special case of (\ref{eq:PPFF-GNN}) and the terms in (\ref{eq:PPFF-GNN-EFF}) are additive, it is easy to see that (\ref{eq:PPFF-GNN-EFF}) is same as (\ref{eq:PPFF-GNN}) with a modified set of polynomial coefficients. In practice, the required low and high-frequency components are computed based on affordable computational cost. Furthermore, we can also control the contributions from each term by setting or optimizing over hyperparameters, $\eta_l$, $\eta_h$ and $\eta_{gpr}$. Thus, the proposed model offers richer capability and flexibility to learn complex frequency response and balance computation costs over GPR-GNN.       

\textbf{Model Training.} Like GPR-GNN, we apply $\textsc{Softmax}$ activation function on (\ref{eq:nodeemb}) and use the standard cross-entropy loss function to learn the sets of polynomial coefficients ($\gamma$) and classifier model parameters ($\Theta$) using labeled data. To ensure smoothness of the learned filter functions, we add a regularization term that penalizes squared differences between the function values of polynomials of contiguous intervals at each other's interval end-points. More details can be found in the appendix (\ref{subsec:app_boundary_reg}).

\textbf{Computational Cost.} There is some pre-training cost of computing the eigendecomposition for top and bottom k eigenvalues. Most algorithms for this task utilize Lanczos' iteration, convergence bounds of which depends on the input matrix' spectrum \citep{eigbound1,eigbound2}, which although have superlinear convergence, but are observed to be efficient in practice. We compute node embeddings afresh whenever the model parameters are updated. This computation involves matrix multiplication with eigenmatrices incurring an additional cost (over GPR-GNN) of $O(nkL)$ where $k$ and $L$ denote the number of selected low/high eigenvalues and classes, respectively. 

\subsection{Analysis}
\label{subsec:analysis}
We first give a simple theoretical justification for using multiple polynomials. We upper-bound the approximation error achieved by using multiple polynomials by the error that the single polynomial parameterization achieves. We relegate the proofs of all the theorems of this section to the appendix.

\begin{theorem}
\label{thm:better_approximation}
For any frequency response $h^*$, and an integer $K\in\mathbb{N}$, let $\Tilde{h}:=h+h_f$, with $h_f$ having a continuous support over a subset of the spectrum, $\sigma_f$. Assume that $h$ and $h_f$ are parameterized by independent $K$ and $K'$-order polynomials, $p$ and $p_f$, respectively, with $K'\leq K$. Then there exists $\Tilde{h}$, such that $\min\|\Tilde{h} - h^*\|_2\leq \min\|h-h^*\|_2$, where the minimum is taken over the polynomial parameterizations. Moreover, for multiple polynomial adaptive filters $h_{f_1},h_{f_2},...,h_{f_m}$ parameterized by independent $K'$-degree polynomials with $K'\leq K$ but having disjoint, contiguous supports, the same inequality holds for $\Tilde{h} = h + \sum_{i=1}^m h_{f_i}$.
\end{theorem}

%The proof naturally arises from simple algebraic constructions. One can now think of the adaptive filters as providing better local control over the polynomial fit, adding more degrees of freedom on its support, and hence resulting in a better fit. But since the spectrum of the reference matrix is $[-1,1]$, controlling the lower order terms is more important that fitting the higher order terms, which can be achieved by using adaptive filters parameterized by a lower degree polynomial. One can show by a simple construction that the optimal approximation error by using such filters is still lower than the one achievable by a globally defined polynomial.

%\begin{corollary}
%\label{thm:lower_than_k}
%If the adaptive filters $h_{f_1},h_{f_2},...,h_{f_m}$ are parameterized by independent polynomials having degree $K'\leq K$, and let $h$ be parameterized by a K-degree polynomial, then $\|\Tilde{h} - h^*\|_2\leq \min\|h-h^*\|_2$.
%\end{corollary}

For a detailed proof please refer to \ref{thm:better_approximation_appendix}. We constructed waveforms of arbitrary complexity, approximated by first fitting a single globally-defined polynomial and then adding locally defined polynomials on top of it.  We assess the performance by varying the degrees of the local polynomials. The corresponding plots (See Figure~\ref{fig:fictitious}) indicate that use of lower-order filters achieves a fit comparable to one by a relatively higher-degree polynomial. Since an actual waveform is not observed in practice and instead, we estimate it by optimizing over the observed labels via learning a graph filter, we theoretically show that the family of filters that we learn is a strict superset of the polynomial filter family. The same result holds for the families of the resulting adapted graphs. 

\begin{theorem}
\label{thm:space_of_filters}
Define $\mathbb{H}:=\{h(\mathbf{\cdot})\;|\;\forall\text{ possible K-degree polynomial parameterizations of $h$}\}$ to be the set of all K-degree polynomial filters, whose arguments are $n\times n$ diagonal matrices, such that a filter response over some $\mathbf{\Lambda}$ is given by $h(\mathbf{\Lambda})$ for $h(\cdot)\in\mathbb{H}$. Similarly $\mathbb{H}':=\{ \Tilde{h}(\cdot)\;|\;\forall\text{ possible polynomial parameterizations of }\Tilde{h}\}$ is set of all filters learn-able via \ourmodel~, with $\Tilde{h} = h + h_{f_1} + h_{f_2}$, where $h$ is parameterized by a K-degree polynomial supported over entire spectrum, $h_{f_1}$ and $h_{f_2}$ are adaptive filters parameterized by independent $K'$-degree polynomials which only act on top and bottom $t$ diagonal elements respectively, with $t<n/2$ and $K'\leq K$; then $\mathbb{H}$ and $\mathbb{H}'$ form a vector space, with $\mathbb{H}\subset \mathbb{H}'$. Also, $\frac{\text{dim}(\mathbb{H}')}{\text{dim}(\mathbb{H})} = \frac{K+2K'+3}{K+1}$.
\end{theorem}

\begin{corollary}
\label{thm:space_of_graphs}
The corresponding adapted graph families $\mathbb{G}:=\{\mathbf{U}^T h(\mathbf{\cdot})\mathbf{U}^T\;|\;\forall h(\cdot)\in\mathbb{H}\}$ and $\mathbb{G'}:=\{\mathbf{U}^T \Tilde{h}(\cdot)\mathbf{U}^T\;|\;\forall \Tilde{h}(\cdot)\in\mathbb{H}'\}$ for any unitary matrix $\mathbf{U}$ form a vector space, with $\mathbb{G}\subset \mathbb{G}'$ and $\frac{\text{dim}(\mathbb{G}')}{\text{dim}(\mathbb{G})} = \frac{K+2K'+3}{K+1}$.
\end{corollary}

This implies that our model is learning from a more diverse space of filters and the corresponding adapted graphs. Moreover, the dimension of the space increases significantly by using just two adaptive filters. Note that learning from such a diverse region is feasible. This observation is possible from the proofs of Theorem 4.2 (\ref{thm:space_of_filters_appendix}) and Corollary 4.2.1 (\ref{thm:space_of_graphs_appendix}). Using the adaptive filters without any filter with the entire spectrum as support results in learning a set of adapted graphs, $\hat{\mathbb{G}}$. This set is disjoint from $\mathbb{G}$, with $\mathbb{G'}=\mathbb{G}\oplus\hat{\mathbb{G}}$. We conduct various ablative studies where we demonstrate the effectiveness of learning from $\hat{\mathbb{G}}$ and $\mathbb{G'}$.


==> sections/approach_old.tex <==
\section{Proposed Approach}

In this section, we present an alternate interpretation of the \gprgnn~and present our proposed approach that utilizes multiple adaptive filters, each acting on different subsets of the eigen spectrum. 

% . Talk about how we account for left over eigen values by adding in the GPR term. Also, formally describe the model.

\subsection{Untitled Model}

We start by observing closely the GPR component output given by: 
\begin{equation}
    {\mathbf G} = \eigenU h_K(\adjS) \eigenU^T {\mathbf Z}^{(0)}.
\label{eqn:GPRGNN2}    
\end{equation}
Our first observation is that learning filter coefficients is equivalent to learning a \textit{new} graph, ${\tilde \adj(\eigenU, \adjS;\alpha})$ which is dependent on the fixed set of eigenvectors and eigenvalues, but, parameterised using $\alpha$. Therefore, the \gprgnn~model may be interpreted as adapting the original adjacency matrix $\adj$. Next, as noted in the previous section, using the structures present in eigendecomposition and polynomial function, we can expand (\ref{eqn:GPRGNN2}) by unrolling over eigenvalues and interchanging the summation as:
\begin{equation}
    {\mathbf G} = \sum_{j=1}^n \eigenUc_j h_K(\lambda_j;\alpha) \eigenUc^T_j {\mathbf Z}^{(0)}.
\label{eqn:GPRGNN3}    
\end{equation}
% Basis our analysis in Section (Motivation section), we replace the single polynomial filter $h_K(.)$ in equation~(\ref{eqn:GPRGNN3}) with multiple polynomials as defined below:

% \begin{equation}
%     {\mathbf G_{m}} = \sum_{j=1}^n  \eigenUc_i h_K(\lambda_j;\alpha_{(j)}) \eigenUc^T_j {\mathbf Z}^{(0)},
% \label{eqn:multiPolyGPRGNN}    
% \end{equation}

% Equation~(\ref{eqn:multiPolyGPRGNN}) requires explicit decomposition of all eigenvalues. This would be intractable for large graphs. However, it would be feasible to compute and adapt a few eigen components.~\cite{gprgnn} and \cite{fagcn} have shown the importance of high frequency and low frequency components for the node classification task. Taking this into account, we could reformulate equation~(\ref{eqn:multiPolyGPRGNN}) as follows:

% \begin{equation}
%     {\mathbf GL} = \sum_{l=1}^L h_K(\lambda_l; \alpha_{(l)}) u_l u_l^T {\mathbf Z}^{(0)} + \sum_h^H h_K(\lambda_h; \alpha_{(h)}) u_h u_h^T {\mathbf Z}^{(0)}
% \label{eqn:GL}    
% \end{equation}

% where L refers to bottom-L eigen components and H refers to top-H eigen components. Equation~(\ref{eqn:GL}) can be interpreted as multiple polynomial filters acting on L-bottom and H-top eigen components. We can observe that depending on the number of top/bottom eigen components being adapted, several eigen components would be missed out. A simple fix to account for these lost signals would be to add ${\mathbf G}$ to the ${\mathbf GL}$ term, leading to our proposed approach as depicted below:

% \begin{equation}
%     {\mathbf G} + {\mathbf GL} = (1 - \beta)(\eigenU h_K(\adjS) \eigenU^T {\mathbf Z}^{(0)}) + \beta (\sum_{l=1}^L h(\lambda_l; \alpha_{(l)}) u_l u_l^T {\mathbf Z}^{(0)} + \sum_h^H h(\lambda_h; \alpha_{(h)}) u_h u_h^T {\mathbf Z}^{(0)})
% \label{eqn:GGL}    
% \end{equation}

% Since polynomial filters are used across the terms in the above equation, the above polynomials can be added together. The last two terms in equation~(\ref{eqn:GGL}) can be interpreted as correction terms that are working to reduce the residual error discussed in Section~(MOTIVATION). By appropriately setting the value of $\beta$, we can recover the original~\gprgnn~from equation~(\ref{eqn:GGL}). Since all the signals in the eigenspectrum are accounted for in this formulation, one can reduce the computation burden by limiting the explicit adaptation of eigen values (last two terms) depending on the compute available.

% In the following sections, we comprehensively compare our proposed approach against several baselines on benchmark datasets. We also provide several ablative studies and empirical analysis to show the usefulness of our approach.


The output graph of \gprgnn~can be written as:
\begin{equation}
    {\mathbf G} = \sum_k a_k A^k 
\label{eqn:G}    
\end{equation}
where $a_k$ are the learned polynomial coefficients. 

Basis our analysis in Section~\ref{motivation}, we replace the single polynomial filter $h_K(.)$ in equation~(\ref{eqn:GPRGNN3}) with multiple polynomial filters. The new output graph can be written as follows:

\begin{equation}
\mathbf{G_m} = \sum_{j=1}^n {h_K}^{(j)}(\lambda_j) u_j u_j^T
\end{equation}

However, we can observe that this computation would require an explicit decomposition, which would be intractable for large graphs. Let m be the feasible number of eigen components that can be adapted. We write this output graph with explicit adaptation, but missing signals as follows:

\begin{equation}
{\mathbf{GL}} = \sum_m g(\lambda_m) u_m u_m^T
\label{eqn:GL}
\end{equation}

We do the following to compensate for the missing signals in equation~\ref{eqn:GL}. We breakdown the eigenvalues into three disjoint partitions as follows:

\begin{equation}
\mathbf{G} = \eigenU (h_K(\adjS_{E - (E_l + Eh)}) + h_{K_1}(\adjS_{E_l}) + h_{K_2}(\adjS_{E_h}) ) \eigenU^T
\end{equation}

Let ${E_l}$ and ${E_h}$ denote l low-end eigenvalues and h high-end eigenvalues. These components can be captured and adapted by the $\mathbf{GL}$ term. We can see that the first partition term can be viewed as the $\mathbf{G}$ term.

Therefore, the final output graph with multiple polynomial adaptive filters acted on can be written as:

\begin{equation}
\mathbf{G_{eff}} = \sum_k \sum_m a_k \lambda^k u_m u_m^T  + \sum_m g(\lambda_m) u_m u_m^T
\end{equation}





==> sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
Several proposed models attempt to be robust to the correlations between graph and node labels. We build on the filter-based approach of \gprgnn~\citep{gprgnn}. This work proposed an effective polynomial filter design. We combine \gprgnn~with additional polynomials that adapt specifically to low and high-frequency components. Our experiments demonstrate that such an approach can learn filter functions that improve performance on the node classification task. Our plots of these filter functions suggest that they are of high order on several datasets. It would be interesting to analyze these filter plots and identify some common characteristics. These will enable us to a] characterize the correlation of graphs and labels, b] further improve the performance and c] build robust graph privacy models. We plan to do this as our future work.

==> sections/experiments_V1.tex <==
\section{Experiments}
\renewcommand{\arraystretch}{1.3}
\label{sec:experiments}
We conduct comprehensive experiments to demonstrate the effectiveness and competitiveness of the proposed PP-GNN model over state-of-the-art (SOTA)  models/methods and answer the following research questions. 
\begin{enumerate}
    \item \textbf{[RQ1]} Does the PP-GNN model outperform SOTA models/methods over a broad range of datasets (homophilic/heterophilic)?
\item \textbf{[RQ2]} Does the proposed model learn better and complex frequency responses that improve performance [Frequency response plots]?
\item \textbf{[RQ3]} With the PP-GNN model comprising of multiple filters, how does each filter contribute to achieving improved performance? 
\item \textbf{[RQ4 and RQ5]} Does the model learn better embedding, and do we need a large number of eigenvalues/vectors and polynomials to get improved performance?
\item \textbf{[RQ6]} How does the training time of the PP-GNN and GPR-GNN models compare?
\end{enumerate}

\textbf{Datasets and Setup.} We evaluate our model on several real-world heterophilic and homophilic datasets including a few large graphs for the node classification task. Detailed statistics of the benchmark datasets are provided in the appendix (\ref{app:dataset_stats}). The heterophilic datasets include \textbf{Texas}\footnote{\label{fn:webkb}http://www.cs.cmu.edu/afs/cs.cmu.edu/project/theo-11/www/wwkb}, \textbf{Cornell}\footnotemark[\value{footnote}], \textbf{Wisconsin}\footnotemark[\value{footnote}], \textbf{Chameleon}, \textbf{Squirrel}, \citep{chameleondataset} and \textbf{Flickr}. We use the 10 random splits (48\%/32\%/20\% of nodes for train/validation/test set) from~\cite{geomgcn}. For \textbf{Flickr}, \textbf{Ogbn-Arxiv}, and \textbf{Wiki-CS}, we use the data splits from~\cite{supergat}. We also evaluate on 8 homophilic datasets: \textbf{Cora-Full}, \textbf{Ogbn-Arxiv}, \textbf{Wiki-CS}, \textbf{Citeseer}, \textbf{Pubmed}, \textbf{Cora}, \textbf{Computer}, and \textbf{Photos} borrowed from \cite{supergat}. For the remaining homophilic datasets, we create 10 random splits for each dataset following~\cite{supergat}. We use PCA node features (\cite{supergat}) for the \textbf{Chameleon} and \textbf{Cora-Full} datasets. We report mean and standard deviation of test accuracy over splits to compare model performance. 

\textbf{Baselines.} We compare our model against (a) filtering based approaches, \gprgnn, ~\fagcn, ~\appnp, and~\lingcn, (b) other state-of-the-art models include ~\supergat, ~\tdgnn,~\hhgcn, and~\geomgcn, and (c) standard baselines, namely, \textsc{LR} (Logistic Regression), \textsc{MLP} (Multi Layer Perceptron), ~\gcn, and~\sgcn. Detailed descriptions for all the baselines, hardware and software specifications are in the appendix (\ref{app:baselines} and \ref{app:implimentation})

\textbf{Hyperparameter Tuning.} For the PP-GNN model, we separately partition the low-end and high-end eigenvalues into several contiguous partitions and use shared filter parameters for frequencies of each partition. The number of partitions, which can be interpreted as the number of filters, is swept in the range [2,3,4,5,10,20]. The polynomial filter order is swept in the range [1,10] in steps of size 1. The number of eigenvalues/vectors are swept in the range [32, 64, 128, 256, 512, 1024]. In our experiments, we set $\eta_l = \eta_h$ and we vary them in range (0, 1) and set $\eta_{gpr} = 1 - \eta_l$. We did hyperparameter tuning for other models as suggested in respective references and public repositories. More details are in the appendix (\ref{app:implimentation}).

%%%%%%%%%%%% RQ1
%\textbf{[RQ1]}
\begin{table}[H]
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccc}
\hline
\multicolumn{1}{c|}{\textbf{Test Acc}}                      & \textbf{Texas}         & \textbf{Wisconsin}     & \textbf{Squirrel}     & \textbf{Chameleon}    & \textbf{Cornell}      & \cellcolor[HTML]{FFFFFF}\textbf{Flickr} \\ \hline
\multicolumn{1}{c|}{\textbf{LR}}                            & 81.35 (6.33)           & 84.12 (4.25)           & 34.73 (1.39)          & 45.68 (2.52)          & \underline{83.24 (5.64)} & 46.51                                   \\
\multicolumn{1}{c|}{\textbf{MLP}}                           & 81.24 (6.35)           & 84.43 (5.36)           & 35.38 (1.38)          & 51.64 (1.89)          & \underline{83.78 (5.80)} & 46.93                                   \\
\multicolumn{1}{c|}{\textbf{SGCN}}                          & 62.43 (4.43)           & 55.69 (3.53)           & 45.72 (1.55)          & 60.77 (2.11)          & 62.43 (4.90)          & 50.75                                   \\
\multicolumn{1}{c|}{\textbf{GCN}}                           & 61.62 (6.14)           & 58.82 (4.89)           & 47.78 (2.13)          & 62.83 (1.52)          & 62.97 (5.41)          & 53.4                                    \\
\multicolumn{1}{c|}{\textbf{SuperGAT}}                      & 61.08 (4.97)           & 56.47 (3.90)           & 31.84 (1.26)          & 43.22 (1.71)          & 57.30 (8.53)          & \underline{53.47}                          \\
\multicolumn{1}{c|}{\textbf{Geom-GCN}}                      & 67.57*                 & 64.12*                 & 38.14*                & 60.90*                & 60.81*                & NA                                      \\
\multicolumn{1}{c|}{\textbf{H2GCN}}                         & \underline{84.86 (6.77)*} & \underline{86.67 (4.69)*} & 37.90 (2.02)*         & 58.40 (2.77)          & 82.16 (4.80)*         & OOM                                     \\
\multicolumn{1}{c|}{\textbf{FAGCN}}                         & 82.43 (6.89)           & 82.94 (7.95)           & 42.59 (0.79)          & 55.22 (3.19)          & 79.19 (9.79)          & OOM                                     \\
\multicolumn{1}{c|}{\textbf{APPNP}}                         & 81.89 (5.85)           & 85.49 (4.45)           & 39.15 (1.88)          & 47.79 (2.35)          & 81.89 (6.25)          & 50.33                                   \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{LGC}}   & 80.20 (4.28)           & 81.89 (5.98)           & 44.26 (1.49)          & 61.14 (2.07)          & 74.59 (3.42)          & 51.67                                   \\
\multicolumn{1}{c|}{\textbf{GPR-GNN}}                       & 81.35 (5.32)           & 82.55 (6.23)           & \underline{46.31 (2.46)} & \underline{62.59 (2.04)} & 78.11 (6.55)          & 52.74                                   \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{TDGNN}} & 83.00 (4.50)*          & 85.57 (3.78)*          & 43.84 (2.16)          & 55.20 (2.30)          & 82.92 (6.61)*         & OOM                                     \\\hline
% \multicolumn{1}{c|}{\textbf{UFG}}                           & 66.22 (7.46)           & 68.63 (4.98)           & 42.09 (1.70)          & 55.78 (1.29)          & 69.19 (6.40)          & OOM                                     \\ \hline
% \multicolumn{7}{c}{\textbf{Our Model}}                                                                                                                                                                                          \\ \hline
\multicolumn{1}{c|}{\textbf{\ourmodel}}                  & \textbf{89.73 (4.90)}  & \textbf{88.24 (3.33)}  & \textbf{56.86 (1.20)} & \textbf{67.74 (2.31)} & \textbf{82.43 (4.27)} & \textbf{55.17}                          \\ \hline
\end{tabular}
}
\caption{Results on Heterophilic Datasets. We underline the results for the best performing baseline model. `*' indicates that the results were borrowed from the corresponding papers.}
\label{tab:result_table_heterophily}
\end{table}


\begin{table}[H]
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccc}
\hline
\multicolumn{1}{c|}{\textbf{Test Acc}}                    & \textbf{Cora-Full}    & \cellcolor[HTML]{FFFFFF}\textbf{OGBN-ArXiv} & \textbf{Wiki-CS}      & \textbf{Citeseer}      & \textbf{Pubmed}       & \textbf{Cora}         & \textbf{Computer}                   & \textbf{Photos}       \\ \hline
\multicolumn{1}{c|}{\textbf{LR}}                          & 39.10 (0.43)          & 52.53                                       & 72.28 (0.59)          & 72.22 (1.54)           & 87.00 (0.40)          & 73.94 (2.47)          & 64.92 (2.59)                        & 77.57 (2.29)          \\
\multicolumn{1}{c|}{\textbf{MLP}}                         & 43.03 (0.82)          & 54.96                                       & 73.74 (0.71)          & 73.83 (1.73)           & 87.77 (0.27)          & 77.06 (2.16)          & 64.96 (3.57)                        & 76.96 (2.46)          \\
\multicolumn{1}{c|}{\textbf{SGCN}}                        & 61.31 (0.78)          & 68.51                                       & 78.30 (0.75           & 76.77 (1.52)           & 88.48 (0.45)          & 86.96 (0.78)          & 80.65 (2.78)                        & 89.99 (0.69)          \\
\multicolumn{1}{c|}{\textbf{GCN}}                         & 59.63 (0.86)           & 69.37                                       & 77.64 (0.49)          & 76.47 (1.33)           & 88.41 (0.46)          & 87.36 (0.91)          & 82.50 (1.23)                        & 90.67 (0.68)          \\
\multicolumn{1}{c|}{\textbf{SuperGAT}}                    & 57.75 (0.97)          & 55.1*                                       & 77.92 (0.82)          & 76.58 (1.59)           & 87.19 (0.50)          & 86.75 (1.24)          & 83.04 (1.02)                        & 90.31 (1.22)          \\
\multicolumn{1}{c|}{\textbf{Geom-GCN}}                    & NA                    & NA                                          & NA                    & \underline{77.99*}                 & \underline{90.05*}       & 85.27*                & NA                                  & NA                    \\
\multicolumn{1}{c|}{\textbf{H2GCN}}                       & 57.83 (1.47)          & OOM                                         & OOM                   & 77.07 (1.64)* & 89.59 (0.33)*         & 87.81 (1.35)*         & OOM                                 & 91.17 (0.89)          \\
\multicolumn{1}{c|}{\textbf{FAGCN}}                       & 60.07 (1.43)          & OOM                                         & 79.23 (0.66)          & 76.80 (1.63)           & 89.04 (0.50)          & \underline{88.21 (1.37)} & 82.16 (1.48)                        & 90.91 (1.11)          \\
\multicolumn{1}{c|}{\textbf{APPNP}}                       & 60.83 (0.55)          & 69.2                               & 79.13 (0.50)          & 76.86 (1.51)           & 89.57 (0.53)          & 88.13 (1.53)          & 82.03 (2.04)                        & 91.68 (0.62)          \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{LGC}} & \underline{61.84 (0.90)} & \underline{69.64}                                       & \underline{79.82 (0.49)} & 76.96 (1.73)           & 88.78 (0.51)          & 88.02 (1.44)          & 83.44 (1.77)                        & 91.56 (0.74)          \\
\multicolumn{1}{c|}{\textbf{GPR-GNN}}                     & 61.37 (0.96)          & 68.44                                       & 79.68 (0.50)          & 76.84 (1.69)           & 89.08 (0.39)          & 87.77 (1.31)          & 82.38 (1.60)                        & 91.43 (0.89)          \\
\multicolumn{1}{c|}{\textbf{TDGNN}}                       & OOM                   & OOM                                         & 79.58 (0.51)          & 76.64 (1.54)*          & 89.22 (0.41)*         & \underline{88.26 (1.32)*}         & \underline{84.52 (0.92)}                        & \underline{92.54 (0.28)}          \\ \hline
% \multicolumn{1}{c|}{\textbf{UFG}}                         & 60.98 (0.82)          & OOM                                         & \textbf{78.56 (0.43)} & 76.74 (1.33)           & 85.68 (0.62)          & 87.97 (1.61)          & {\color[HTML]{000000} 80.01 (1.78)} & 90.03 (1.41)          \\ \hline
% \multicolumn{9}{c}{\textbf{Our Model}}                                                                                                                                                                                                                                                         \\ \hline
\multicolumn{1}{c|}{\textbf{\ourmodel}}                & \textbf{61.42 (0.79)} & \textbf{69.28}                              & \textbf{80.04 (0.43)} & \textbf{78.25 (1.76)}  & \textbf{89.71 (0.32)} & \textbf{89.52 (0.85)} & \textbf{85.23 (1.36)}               & \textbf{92.89 (0.37)} \\ \hline
\end{tabular}
}
\caption{Results on Homophilic Datasets.}
\label{tab:result_table_homophily}
\end{table}

\subsection{RQ1: PP-GNN versus SOTA Models} 
We present several important observations from Tables 1 and 2. We observe that the PP-GNN model consistently outperforms all models, including recent filtering approach based models on all datasets (both heterophilic and homophilic) except Pubmed and Cornell, where it achieves similar performance. This result demonstrates the effectiveness and robustness of our model across a wide variety of datasets. Furthermore, compared with the GPR-GNN model, learning piece-wise polynomial filters improves performance significantly over learning a single polynomial filter. In particular, PP-GNN achieves performance improvements of around 10\% and 5\% on the Chameleon and Squirrel datasets.
 %This suggests that complex frequency responses are indeed needed for certain datasets and such responses can be learned effectively using the PP-GNN model.  

\subsection{RQ2: Adaptable Frequency Responses}
We computed the frequency responses (i.e., $h(\lambda)$) of learned polynomials of the PP-GNN and GPR-GNN models on several datasets, including Squirrel and Citeseer datasets shown in Figure~\ref{fig:PPGNN_learned_poly}. We observe from Figure~\ref{fig:RQ2_squirrel}, though the \gprgnn~model can learn some variations at low/high frequencies, it is insufficient to achieve higher classification accuracy. On the other hand, the \ourmodel~model can capture complex shapes at the low and high ends of the spectrum, enabling it to achieve significantly improved test accuracy. We observed a similar phenomenon for the chameleon dataset as well. To illustrate another behaviour, we present the frequency responses for the Citeseer dataset in Figure~\ref{fig:RQ2_citeseer}, and the responses are similar except for some variations at the low-end of the spectrum. Note that the \gprgnn~model does well on several homophilic datasets. These observations suggest that the \ourmodel~model adapts very well in learning desired frequency responses, as dictated by the task at hand. We can observe such a behaviour for two other datasets in the appendix (\ref{app:adap_freq_response}).     

\begin{figure}[H]
    % \centering
    % \begin{subfigure}[t]{0.5\textwidth}
    %     \centering
    %     \includegraphics[height=1.5in, width=0.85\textwidth]{iclr2022/images/G_GL_polyPlots/chameleon_pca_boundaryReg.png}
    %     \caption{Chameleon}
    %     \label{RQ3_chameleon}
    % \end{subfigure}%
    % ~ 
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[height=1.5in, width=0.85\textwidth]{iclr2022/images/G_GL_polyPlots/squirrel_boundaryReg.png}
        \caption{Squirrel}
        \label{fig:RQ2_squirrel}
    \end{subfigure}
    % \\
    % \vspace{2mm}
    % \begin{subfigure}[t]{0.5\textwidth}
    %     \centering
    %     \includegraphics[height=1.5in, width=0.85\textwidth]{iclr2022/images/G_GL_polyPlots/amazon_electronics_computers_boundaryReg.png}
    %     \caption{Computers}
    %     \label{RQ3_computers}
    % \end{subfigure}%
    % ~ 
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[height=1.5in, width=0.85\textwidth]{iclr2022/images/G_GL_polyPlots/citeseer_boundaryReg.png}
        \caption{Citeseer}
        \label{fig:RQ2_citeseer}
    \end{subfigure}
    
    \caption{Visualization of adapted eigenspectrum by our proposed model and~\gprgnn}
    \label{fig:PPGNN_learned_poly}
\end{figure}

%%%%%%%%%%%%%%%%%% RQ3

%\textbf{[RQ3]}


%\begin{table}[H]
%\resizebox{\textwidth}{!}{%
%\begin{tabular}{c|ccccccccccc}
%\hline
%{\color[HTML]{000000} \textbf{Test Acc}} & \textbf{Texas}                                 & \textbf{Wisconsin}                             & \textbf{Squirrel}                              & \textbf{Chameleon}                    & \textbf{Cornell}                      & \textbf{Cora-Full}                             & \textbf{Citeseer}                              & \textbf{Pubmed}                                & \textbf{Cora}                                  & \textbf{Computer}                              & \textbf{Photos}                                \\ \hline
%\textbf{GPR-GNN}                & 81.35   (5.32)                                 & 82.55   (6.23)                                 & 46.31   (2.46)                                 & 62.59   (2.04)                        & 78.11   (6.55)                        & 61.37   (0.96)                                 & 76.84   (1.69)                                 & 89.08   (0.39)                                 & 87.77   (1.31)                                 & 82.38   (1.60)                                 & 91.43   (0.89)                                 \\
%\textbf{GL Term}                & 85.68   (3.83)                                 & 85.10   (3.09)                                 & 55.63   (1.44)                                 & \textbf{68.51 (1.64)}                 & \textbf{82.70 (5.13)}                 & 55.93   (0.77)                                 & {\color[HTML]{330001} \textbf{78.41   (1.58)}} & 83.65   (0.53)                                 & 89.50   (0.78)                                 & 82.55   (1.93)                                 & 89.87   (0.49)                                 \\
%\textbf{\ourmodel}            & {\color[HTML]{000000} \textbf{89.73   (4.90)}} & {\color[HTML]{000000} \textbf{88.24   (3.33)}} & {\color[HTML]{000000} \textbf{56.86   (1.20)}} & {\color[HTML]{000000} 67.74   (2.31)} & {\color[HTML]{000000} 82.43   (4.27)} & {\color[HTML]{000000} \textbf{61.42   (0.79)}} & {\color[HTML]{000000} 78.25   (1.76)}          & {\color[HTML]{000000} \textbf{89.71   (0.32)}} & {\color[HTML]{000000} \textbf{89.52   (0.85)}} & {\color[HTML]{000000} \textbf{85.23   (1.36)}} & {\color[HTML]{000000} \textbf{92.89   (0.37)}} \\ \hline
%\end{tabular}
%}
%\caption{\ourmodel~v/s \gprgnn}
%\label{tab:result_ppgnnVSgprgnn}
%\end{table}

%%%%%%%%%%%%%%%%%% RQ4

%\textbf{[RQ4]}

%\begin{figure}[H]
%    \centering
%        \includegraphics[height=1.2in, width=\textwidth]{iclr2022/images/G_GL_tuning_lowHigh_comps/TuningEVDcollage_GPRGNN_tuningLowHighEVD.png}
%    \label{fig:AdaptingEVDTopBottom}
%    \caption{Adapting increasing number of top or bottom EVD components}
%\end{figure}

\subsection{RQ3: Performance comparison of Different Filters} 
Recall that the \ourmodel~model is a sum of polynomials model comprising of polynomial filters operating at different parts of the spectrum. Here, we study the importance and effect of using a combination of filters operating on different regions. For reference, we also compare the performance of \gprgnn~model that operates on the entire spectrum using a single filter. Several interesting observations are in order. From Table~\ref{tab:result_ppgnnVSgprgnn}, we see that the best performance is achievable using high-frequency signals alone for the heterophilic datasets (Squirrel and Chameleon), suggesting that significant discriminatory information is available at high frequencies compared to low-frequency signals. In contrast, homophilic datasets (Cora and Citeseer) exhibit a reverse trend. On comparing the first (second) and third (fourth) row results, we see that having the \gprgnn~filter as part of the \ourmodel~filter helps to get improved performance over individual filters (\ourmodel(Low) or \ourmodel~(High)). Finally, the \ourmodel~model can adapt well, capture contrasting information bands across datasets, and outperform the \gprgnn~model.     

\begin{table}[H]
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|llll}
\hline
\textbf{Test Acc}      & \multicolumn{1}{c}{\textbf{Squirrel}} & \multicolumn{1}{c}{\textbf{Chameleon}} & \multicolumn{1}{c}{\textbf{Citeseer}}                     & \multicolumn{1}{c}{\textbf{Cora}}   \\ \hline
\textbf{PP-GNN (Low)}      & 45.75 (1.69)                          & 56.73 (4.03)                           & 76.23 (1.54)                                              & 88.03 (0.79)                        \\
\textbf{PP-GNN (High)}     & 58.70 (1.60)                          & \textbf{69.19 (1.88)}                           & 55.50 (6.38)                                              & 73.76 (2.03)                        \\
\textbf{PP-GNN (GPR-GNN+Low)}  & 50.96 (1.26)                          & 63.71 (2.69)                           & 78.07 (1.71)                                              & \textbf{89.56 (0.93)}                        \\
\textbf{PP-GNN (GPR-GNN + High)} & 60.39 (0.91)                          & 67.83 (2.30)                           & \textbf{78.30 (1.60)}                                              & 89.42 (0.97)                        \\
\textbf{GPR-GNN}       & \multicolumn{1}{c}{42.06   (1.55)}    & \multicolumn{1}{c}{56.29 (1.58)}       & 76.74   (1.33)                                            & \multicolumn{1}{c}{87.93 (1.52)}    \\ \hline
\textbf{PP-GNN}        & \textbf{56.21 (1.79)}                          & 68.93 (1.95)                           & \multicolumn{1}{c}{{\color[HTML]{000000} 78.25   (1.76)}} & {\color[HTML]{000000} 89.52 (0.85)} \\ \hline
\end{tabular}
}
\caption{Performance of different filters}
\label{tab:result_ppgnnVSgprgnn}
\end{table}

\subsection{RQ4 - RQ6: Varying No. of EVs, Learned embedding and Timing Comparison}
We conducted ablative studies to see the effect of varying different hyperparameters of the PP-GNN model. From Figure~\ref{acc_ppgnn_vary_evd}, we see that as small as $32$ eigen components are sufficient to achieve near-best performance on the homophilic datasets (Cora, Citeseer). On the other hand, peak performance is achieved for some intermediate ($\approx$250-500) number of eigen components for the Squirrel and Chameleon datasets. Also, we note that we can achieve comparable performance to state of the art models on large datasets (Flickr and OGBN-Arxiv) using only $1024$ components (See Tables 1 and 2). This study suggests that the \ourmodel~model is scalable at least for medium sized graphs (~100K nodes). More evaluation and investigation are needed to study performance versus computation cost trade-off for very large graphs (millions of nodes). 

To assess the quality of learned embedding, we also created t-SNE plots and made a visual inspection. From Figure~\ref{PPGNN_TSNE_squirrel} and \ref{GPRGNN_TSNE_squirrel}, we see that the clusters belonging to different classes of the Squirrel dataset are better separated for the \ourmodel~ model compared to the \gprgnn~ model. We also measured the time taken by the \gprgnn~and \ourmodel~models. We observed that the \gprgnn~model is only $(1.2-2)\times$ faster than the \ourmodel~model (using $1024$ eigencomponents) on many datasets. Thus, the extra training cost incurred by the \ourmodel~model is not significantly different for practical purposes. More details are in the appendix (\ref{app:timing_analysis}). 

\begin{figure}
\centering
\begin{minipage}[c]{0.33\textwidth}
        \centering
        \includegraphics[height=1.5in, width=0.97\textwidth]{iclr2022/images/G_GL_tuning_lowHigh_comps/PPGNN_Varying_EVD.png}
        \subcaption{Varying No. of EVs}
        \label{acc_ppgnn_vary_evd}
\end{minipage}
\begin{minipage}[c]{0.3\textwidth}
        \centering
        \includegraphics[height=1.5in, width=0.97\textwidth]{iclr2022/images/TSNE/PPGNN_squirrel.png}
        \subcaption{PP-GNN on Squirrel}
        \label{PPGNN_TSNE_squirrel}
\end{minipage}
\begin{minipage}[c]{0.3\textwidth}
        \centering
        \includegraphics[height=1.5in, width=0.97\textwidth]{iclr2022/images/TSNE/gprgnn_squirrel.png}
        \subcaption{GPR-GNN on Squirrel}
        \label{GPRGNN_TSNE_squirrel}
\end{minipage}
\caption{Analyzing varying number of eigenvalues and the learned embeddings}
\end{figure}

==> sections/experiments_old.tex <==
\section{Experiments}
\renewcommand{\arraystretch}{1.3}

\label{sec:experiments}
We design several experiments to investigate the effectiveness of our proposed approach. Through these experiments, we would like to answer the following questions: \\
\textbf{[RQ1]} In Theorem~\ref{thm:better_approximation}, we claim that using multiple polynomial filters can approximate the latent frequency response better than using a single polynomial filter. How does this translate to classification performance? \textbf{[RQ2]} How does the proposed approach compare against existing state-of-the-art models? 
% \textbf{[RQ3]} We expect our model to work better when the latent optimal filter is of a higher order. How does the learnt filter look in practice? 
\textbf{[RQ3]} Theorem~\ref{thm:space_of_filters} shows that \ourmodel~can learn from a larger set of filters. Does the learnt filter response differ from that of \gprgnn? \textbf{[RQ4]} In Section~\ref{sec:proposedapproach}, we based our model on the observation that low-pass and high-pass frequency components are critical for performance. Do they really contain useful information? \textbf{[RQ5]} Does increasing the number of components and the number of polynomials improve our approximation of latent filter and give better performance? Or are there trade-offs involved? \textbf{[RQ6]} How expensive is it to compute top and bottom eigenpairs in practice?

%In the following subsections, we briefly describe the datasets used in our experiments, and provide responses to the above questions.\\

\textbf{Datasets.} We evaluate our model on several real-world Heterophilic and Homophilic datasets including a few large graphs for the node classification task. Detailed statistics of the benchmark datasets are provided in the Appendix. Our Heterophilic graphs include \textbf{Texas}\footnote{\label{fn:webkb}http://www.cs.cmu.edu/afs/cs.cmu.edu/project/theo-11/www/wwkb}, \textbf{Cornell}\footnotemark[\value{footnote}], \textbf{Wisconsin}\footnotemark[\value{footnote}], \textbf{Chameleon}, \textbf{Squirrel}, \citep{chameleondataset} and \textbf{Flickr}. We evaluate on 8 Homophilic graphs: \textbf{Cora-Full}, \textbf{Obgn-Arxiv}, \textbf{Wiki-CS}, \textbf{Citeseer}, \textbf{Pubmed}, \textbf{Cora}, \textbf{Computer}, and \textbf{Photos} borrowed from \cite{supergat}. We follow the experimental setup described in~\cite{supergat}. For Heterophilic datasets, we use the 10 random splits (48\%/32\%/20\% of nodes for train/validation/test set) from~\cite{geomgcn}. For \textbf{Flickr}, \textbf{Ogbn-Arxiv}, and \textbf{Wiki-CS}, we use the data splits from~\cite{supergat}. For the remaining Homophilic datasets, we create 10 random splits for each dataset following~\cite{supergat}. \textbf{Note:} for \textbf{Chameleon} and \textbf{Cora-Full} datasets, we resort to PCA node features as described in~\cite{supergat}.

% For datasets in \{Texas, Wisconsin, Cornell, Chameleon, Squirrel, Actor\}, we use 10 random splits (48\%/32\%/20\% of nodes for train/validation/test set) from~\cite{geomgcn}. For Crocodile, we create 10 random splits following~\cite{supergat}. We borrowed \textbf{Cora}, \textbf{Citeseer}, and \textbf{Pubmed} datasets and the corresponding train/val/test set splits from \cite{geomgcn}. The remaining datasets were borrowed from \cite{supergat}. We follow the same dataset setup mentioned in \cite{supergat} to create 10 random splits for each of these datasets.


\begin{table}[H]
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccc}
\hline
\multicolumn{1}{c|}{\textbf{Test Acc}}                      & \textbf{Texas}         & \textbf{Wisconsin}     & \textbf{Squirrel}     & \textbf{Chameleon}    & \textbf{Cornell}      & \cellcolor[HTML]{FFFFFF}\textbf{Flickr} \\ \hline
\multicolumn{1}{c|}{\textbf{LR}}                            & 81.35 (6.33)           & 84.12 (4.25)           & 34.73 (1.39)          & 45.68 (2.52)          & \textbf{83.24 (5.64)} & 46.51                                   \\
\multicolumn{1}{c|}{\textbf{MLP}}                           & 81.24 (6.35)           & 84.43 (5.36)           & 35.38 (1.38)          & 51.64 (1.89)          & \textbf{83.78 (5.80)} & 46.93                                   \\
\multicolumn{1}{c|}{\textbf{SGCN}}                          & 62.43 (4.43)           & 55.69 (3.53)           & 45.72 (1.55)          & 60.77 (2.11)          & 62.43 (4.90)          & 50.75                                   \\
\multicolumn{1}{c|}{\textbf{GCN}}                           & 61.62 (6.14)           & 53.53 (4.73)           & 46.04 (1.61)          & 61.43 (2.70)          & 62.97 (5.41)          & 53.4                                    \\
\multicolumn{1}{c|}{\textbf{SuperGAT}}                      & 61.08 (4.97)           & 56.47 (3.90)           & 31.84 (1.26)          & 43.22 (1.71)          & 57.30 (8.53)          & \textbf{53.47}                          \\
\multicolumn{1}{c|}{\textbf{Geom-GCN}}                      & 67.57*                 & 64.12*                 & 38.14*                & 60.90*                & 60.81*                & NA                                      \\
\multicolumn{1}{c|}{\textbf{H2GCN}}                         & \textbf{84.86 (6.77)*} & \textbf{86.67 (4.69)*} & 37.90 (2.02)*         & 58.40 (2.77)          & 82.16 (4.80)*         & OOM                                     \\
\multicolumn{1}{c|}{\textbf{FAGCN}}                         & 82.43 (6.89)           & 82.94 (7.95)           & 42.59 (0.79)          & 55.22 (3.19)          & 79.19 (9.79)          & OOM                                     \\
\multicolumn{1}{c|}{\textbf{APPNP}}                         & 81.89 (5.85)           & 85.49 (4.45)           & 39.15 (1.88)          & 47.79 (2.35)          & 81.89 (6.25)          & 50.33                                   \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{LGC}}   & 80.20 (4.28)           & 81.89 (5.98)           & 44.26 (1.49)          & 61.14 (2.07)          & 74.59 (3.42)          & 51.67                                   \\
\multicolumn{1}{c|}{\textbf{GPR-GNN}}                       & 81.35 (5.32)           & 82.55 (6.23)           & \textbf{46.31 (2.46)} & \textbf{62.59 (2.04)} & 78.11 (6.55)          & 52.74                                   \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{TDGNN}} & 83.00 (4.50)*          & 85.57 (3.78)*          & 43.84 (2.16)          & 55.20 (2.30)          & 82.92 (6.61)*         & OOM                                     \\\hline
% \multicolumn{1}{c|}{\textbf{UFG}}                           & 66.22 (7.46)           & 68.63 (4.98)           & 42.09 (1.70)          & 55.78 (1.29)          & 69.19 (6.40)          & OOM                                     \\ \hline
\multicolumn{7}{c}{\textbf{Our Model}}                                                                                                                                                                                          \\ \hline
\multicolumn{1}{c|}{\textbf{\ourmodel}}                  & \textbf{89.73 (4.90)}  & \textbf{88.24 (3.33)}  & \textbf{56.86 (1.20)} & \textbf{67.74 (2.31)} & \textbf{82.43 (4.27)} & \textbf{54.44}                          \\ \hline
\end{tabular}
}
\caption{Results on Heterophilic Datasets. We bold the results of the models that come close to achieving the performance of our proposed model, as well as the results of the models that perform better than our proposed approach. `*' indicates that the results were borrowed from corresponding papers. For computing the final average rank, we ignore the entries that contain `OOM' or `NA'.}
\label{tab:result_table_heterophily}
\end{table}


\begin{table}[H]
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccc}
\hline
\multicolumn{1}{c|}{\textbf{Test Acc}}                    & \textbf{Cora-Full}    & \cellcolor[HTML]{FFFFFF}\textbf{OGBN-ArXiv} & \textbf{Wiki-CS}      & \textbf{Citeseer}      & \textbf{Pubmed}       & \textbf{Cora}         & \textbf{Computer}                   & \textbf{Photos}       \\ \hline
\multicolumn{1}{c|}{\textbf{LR}}                          & 39.10 (0.43)          & 52.53                                       & 72.28 (0.59)          & 72.22 (1.54)           & 87.00 (0.40)          & 73.94 (2.47)          & 64.92 (2.59)                        & 77.57 (2.29)          \\
\multicolumn{1}{c|}{\textbf{MLP}}                         & 43.03 (0.82)          & 54.96                                       & 73.74 (0.71)          & 73.83 (1.73)           & 87.77 (0.27)          & 77.06 (2.16)          & 64.96 (3.57)                        & 76.96 (2.46)          \\
\multicolumn{1}{c|}{\textbf{SGCN}}                        & 61.31 (0.78)          & 68.51                                       & 78.30 (0.75           & 76.77 (1.52)           & 88.48 (0.45)          & 86.96 (0.78)          & 80.65 (2.78)                        & 89.99 (0.69)          \\
\multicolumn{1}{c|}{\textbf{GCN}}                         & 45.44 (1.01)          & 63.48                                       & 77.64 (0.49)          & 76.47 (1.33)           & 87.86 (0.47)          & 86.27 (1.34)          & 78.16 (1.85)                        & 86.38 (1.71)          \\
\multicolumn{1}{c|}{\textbf{SuperGAT}}                    & 57.75 (0.97)          & 55.1*                                       & 77.92 (0.82)          & 76.58 (1.59)           & 87.19 (0.50)          & 86.75 (1.24)          & 83.04 (1.02)                        & 90.31 (1.22)          \\
\multicolumn{1}{c|}{\textbf{Geom-GCN}}                    & NA                    & NA                                          & NA                    & 77.99*                 & \textbf{90.05*}       & 85.27*                & NA                                  & NA                    \\
\multicolumn{1}{c|}{\textbf{H2GCN}}                       & 57.83 (1.47)          & OOM                                         & OOM                   & \textbf{77.07 (1.64)*} & 89.59 (0.33)*         & 87.81 (1.35)*         & OOM                                 & 91.17 (0.89)          \\
\multicolumn{1}{c|}{\textbf{FAGCN}}                       & 60.07 (1.43)          & OOM                                         & 79.23 (0.66)          & 76.80 (1.63)           & 89.04 (0.50)          & \textbf{88.21 (1.37)} & 82.16 (1.48)                        & 90.91 (1.11)          \\
\multicolumn{1}{c|}{\textbf{APPNP}}                       & 60.83 (0.55)          & \textbf{69.2}                               & 79.13 (0.50)          & 76.86 (1.51)           & 89.57 (0.53)          & 88.13 (1.53)          & 82.03 (2.04)                        & 91.68 (0.62)          \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{LGC}} & \textbf{61.84 (0.90)} & 69.64                                       & \textbf{79.82 (0.49)} & 76.96 (1.73)           & 88.78 (0.51)          & 88.02 (1.44)          & 83.44 (1.77)                        & 91.56 (0.74)          \\
\multicolumn{1}{c|}{\textbf{GPR-GNN}}                     & 61.37 (0.96)          & 68.44                                       & 79.68 (0.50)          & 76.84 (1.69)           & 89.08 (0.39)          & 87.77 (1.31)          & 82.38 (1.60)                        & 91.43 (0.89)          \\
\multicolumn{1}{c|}{\textbf{TDGNN}}                       & OOM                   & OOM                                         & 79.58 (0.51)          & 76.64 (1.54)*          & 89.22 (0.41)*         & 88.26 (1.32)*         & 84.52 (0.92)                        & 92.54 (0.28)          \\ \hline
% \multicolumn{1}{c|}{\textbf{UFG}}                         & 60.98 (0.82)          & OOM                                         & \textbf{78.56 (0.43)} & 76.74 (1.33)           & 85.68 (0.62)          & 87.97 (1.61)          & {\color[HTML]{000000} 80.01 (1.78)} & 90.03 (1.41)          \\ \hline
\multicolumn{9}{c}{\textbf{Our Model}}                                                                                                                                                                                                                                                         \\ \hline
\multicolumn{1}{c|}{\textbf{\ourmodel}}                & \textbf{61.42 (0.79)} & \textbf{69.28}                              & \textbf{80.04 (0.43)} & \textbf{78.25 (1.76)}  & \textbf{89.71 (0.32)} & \textbf{89.52 (0.85)} & \textbf{85.23 (1.36)}               & \textbf{92.89 (0.37)} \\ \hline
\end{tabular}
}
\caption{Results on Homophilic Datasets.}
\label{tab:result_table_homophily}
\end{table}

% \textbf{Importance of ${\mathbf GL}$ Term:} We perform an ablative study in Table~\ref{tab:ablative_table} to understand the importance of GL term. We observe that using  ${\mathbf GL}$ Term alone gives improvements in performance of up to $\sim 10\%$ compared to \gprgnn. However, there is a drop in performance on a Homophilic datasets including Pubmed and Photos. We believe this gap in performance is because of the missing signals that the  ${\mathbf GL}$ Term is not compensating for. By combining \gprgnn with the ${\mathbf GL}$ Term, we can observe performance gains across datasets.


% \begin{table}[h]
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
%                      & \multicolumn{1}{c|}{Texas} & \multicolumn{1}{c|}{Wisconsin} & \multicolumn{1}{c|}{Squirrel} & \multicolumn{1}{c|}{Chameleon} & \multicolumn{1}{c|}{Cornell} & \multicolumn{1}{c|}{Flickr} & \multicolumn{1}{c|}{Cora-Full} & \multicolumn{1}{c|}{Ogbn-arxiv} & \multicolumn{1}{c|}{Wiki-CS} & \multicolumn{1}{c|}{Citeseer} & \multicolumn{1}{c|}{Pubmed} & \multicolumn{1}{c|}{Cora} & \multicolumn{1}{c|}{Computer} & \multicolumn{1}{c|}{Photos} \\ \hline
% \textbf{GPR-GNN}     & 81.35 (5.32)               & 82.55 (6.23)                   & 46.31 (2.46)                  & 62.59 (2.04)                   & 78.11 (6.55)                 & 52.74                       & 61.37 (0.96)                   & 68.44                           & 79.68 (0.50)                 & 76.84 (1.69)                  & 89.08 (0.39)                & 87.77 (1.31)              & 82.38 (1.60)                  & 91.43 (0.89)                \\ \hline
% \textbf{GL Term}     & 85.68 (3.83)               & 85.10 (3.09)                   & 55.63 (1.44)                  & 68.51 (1.64)                   & 82.70 (5.13)                 &                             & 55.93 (0.77)                   &                                 &                              & \textbf{78.41 (1.58)}         & 83.65 (0.53)                & 89.50 (0.78)              & 82.55 (1.93)                  & 89.87 (0.49)                \\ \hline
% \textbf{G + GL Term} & \textbf{89.73 (4.90)}      & \textbf{88.24 (3.33)}          & \textbf{56.86 (1.20)}         & 67.74 (2.31)                   & 82.43 (4.27)                 &                             & \textbf{61.42 (0.79)}          &                                 &                              & 78.25 (1.76)                  & \textbf{89.71 (0.32)}       & \textbf{89.52 (0.85)}     & \textbf{85.23 (1.36)}         & \textbf{92.89 (0.37)}       \\ \hline
% \end{tabular}
% }
% \caption{Importance of GL Term.}
% \label{tab:ablative_table}
% \end{table}


% \textbf{Effect of Varying number of adapted EVD components in ${\mathbf GL}$ Term:} We vary the number of adapted eigenvalues in our proposed approach for four benchmark datasets and plot them in Figure~\ref{fig:EVDablative}. We observe that as we keep increasing the number of adapted eigen components until a certain point, the test accuracy increases in general for graphs with low homophily scores. This phenomenon can be observed in the Chameleon and Squirrel dataset as shown in Figures XXXChameleon, XXXSquirrel. On the contrary, adapting a few eigen components in graphs with higher homophily levels seems sufficient as can be seen in Figures XXXCora, XXXCiteseer. The test accuracy stabilizes even though more eigen components are adapted. We conjecture that a smooth polynomial filter is sufficient for homophilic graphs, while a complicated polynomial might be required for graphs with lower homophilic scores. 

% \begin{figure}[t!]
%     \centering
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.95\textwidth]{images/G_GL_EVDPlots/chameleon_pca.jpg}
%         \caption{Chameleon}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.95\textwidth]{images/G_GL_EVDPlots/squirrel.jpg}
%         \caption{Squirrel}
%     \end{subfigure} 
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.95\textwidth]{images/G_GL_EVDPlots/cora.jpg}
%         \caption{Cora}
%     \end{subfigure}%
%     ~
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.95\textwidth]{images/G_GL_EVDPlots/citeseer.jpg}
%         \caption{Citeseer}
%     \end{subfigure}
%     \caption{Effect of Varying EVD components}
%     \label{fig:EVDablative}
% \end{figure}


% \textbf{Comparing Polynomials learned by our model against that of \gprgnn's:} To pictorially analyse the effect of adaptation in \gprgnn and our model, we plot the learned polynomials in Figure~\ref{fig:polyPlots}. We observe that the polynomials learned by our model starkly differs from \gprgnn's polynomial on Heterophilic datasets like Texas and Squirrel. Also, these are the datasets, where our approach outperforms \gprgnn's classification performance by a significant margin. Conversely, the polynomials learned by both these approaches are very similar in Homophilic datasets like Cora and Citeseer. We believe that adapting the eigen spectrum using multiple filters has more significant effect in terms on performance on Heterophilic datasets than on Homophilic datasets. 


% \begin{figure}[H]
%     \centering
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.95\textwidth]{images/G_GL_polyPlots/texas_split5.png}
%         \caption{Texas}
%         \label{fig:texas}
%     \end{subfigure}%
%     ~
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.95\textwidth]{images/G_GL_polyPlots/squirrel_split3.png}
%         \caption{Squirrel}
%         \label{fig:squirrel}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.95\textwidth]{images/G_GL_polyPlots/cora_split2.png}
%         \caption{Cora}
%         \label{fig:Cora}
%     \end{subfigure}%
%     ~
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.95\textwidth]{images/G_GL_polyPlots/citeseer_split8.png}
%         \caption{Citeseer}
%         \label{fig:citeseer}
%     \end{subfigure}
%     \caption{Learned Polynomial Plots. Red curves correspond to the learned polynomial from our model. Blue curve corresponds to \gprgnn's learned polynomial.}
%     \label{fig:polyPlots}
% \end{figure}


% \textbf{RQ1.} How does adapting low and high frequency components simultaneously affect task performance? \textit{GL Term is important, Varying EVD comps in G+GL} \todo{\textbf{Add Ablative Table, Discuss which plots to add}}

\textbf{[RQ1] \ourmodel~vs. \gprgnn~\ms{Need to fix the title}}

% We conduct an extensive set of experiments that compare~\ourmodel~against \gprgnn~and report the results in Tables~(\ref{tab:result_table_heterophily},~\ref{tab:result_table_homophily}). \ourmodel~outperforms \gprgnn~on all our benchmark datasets with significant gains of up to~10\% on heterophilic datasets and considerable gains of up to~2\% on homophilic datasets. Our studies at an individual split level for benchmark datasets show performance gains ranging from 0.15\% to 18.92\%. \ms{Refer to Appendix} \ms{T-SNE plots for qualitative analysis}

\textbf{Points to convey:} \\
1) Using multiple polynomial filters over single filter can give superior performance. This is evident in Tables~(\ref{tab:result_table_heterophily},~\ref{tab:result_table_homophily}). \\
2)On performing an individual split level analysis, we observe gains with our model over \gprgnn~on almost all of the splits [on 93.6\% splits, we have better results]. \\
3) t-SNE plots of learned embedding



\textbf{[RQ2] Comparison against other state-of-the-art models?}

% \textbf{Baselines.} We compare our model against filtering based approaches, which includes~\gprgnn, ~\fagcn, ~\ufg, and~\lingcn. Other state-of-the-art baseline models include~\tdgnn,~\mixhop,~\hhgcn, and~\geomgcn. In addition, we compare against standard baselines namely, \textsc{LR} (Logistic Regression), \textsc{MLP} (Multi Layer Perceptron), ~\gcn, and~\sgcn. Detailed baselines descriptions, hardware and software specifications including hyper-parameter tuning are provided in the Appendix.

% \textbf{Performance on Benchmark Datasets:} The test performance of the various baselines and our approach is reported in Table~\ref{tab:result_table_heterophily} and~\ref{tab:result_table_homophily}. We observe that on both homophilic and heterophilic datasets, \ourmodel~outperforms or performs competitively to the baselines in comparison. We compute the average rank for all the models in comparison across datasets and observe that \ourmodel~ achieves a rank of XXX.

\textbf{Points to Convey:} [Can combine with (RQ1)] \\ 
1) We observe that our model outperforms all the baselines in comparison on majority on the datasest. On the remaining datasets, we perform competitively. We observe significant lifts of up to 10\% over previous SOTA models.
2) Average rank of our model.

% \textbf{[RQ3]} We expect our model to work better when the latent optimal filter is of a higher order. How does the learnt filter look in practice? What about the optimal filter?


\textbf{[RQ3] \ourmodel's learnt frequency response.}
\textbf{Use Figure ~\ref{fig:PPGNN_learned_poly} for this RQ. The important points are conveyed in the below para. Additional point: Significant improvement in classification performance on heterophilic graphs, where we also observe a stark difference in learnt frequency responses of models in comparison.} 
Figure ~\ref{fig:PPGNN_learned_poly} indicates that \ourmodel~learns a more complicated frequency response compared to \gprgnn~for heterophilic datasets, while both the models learn a simple and similar frequency response for homophilic datasets. This indicates that the latter possibly requires a simple frequency response to achieve a better task performance with a single polynomial filter. This is in stark contrast to heterophilic datasets, where multiple polynomial filters significantly improve the task performance. Even though the learned frequency response is marginally different from \gprgnn's response, we observe considerable gains in homophilic datasets. For instance, we observe gains of up to 1.18\% in Citeseer and up to 2.19\% on Computers dataset. Our observations align with Theorem~\ref{thm:space_of_filters}, which shows that \gprgnn~is incapable of constructing the complicated frequency response that \ourmodel~ is learning. 

\begin{figure}[H]
    % \centering
    % \begin{subfigure}[t]{0.5\textwidth}
    %     \centering
    %     \includegraphics[height=1.5in, width=0.85\textwidth]{iclr2022/images/G_GL_polyPlots/chameleon_pca_boundaryReg.png}
    %     \caption{Chameleon}
    %     \label{RQ3_chameleon}
    % \end{subfigure}%
    % ~ 
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[height=1.5in, width=0.85\textwidth]{iclr2022/images/G_GL_polyPlots/squirrel_boundaryReg.png}
        \caption{Squirrel}
        \label{RQ3_squirrel}
    \end{subfigure}
    % \\
    % \vspace{2mm}
    % \begin{subfigure}[t]{0.5\textwidth}
    %     \centering
    %     \includegraphics[height=1.5in, width=0.85\textwidth]{iclr2022/images/G_GL_polyPlots/amazon_electronics_computers_boundaryReg.png}
    %     \caption{Computers}
    %     \label{RQ3_computers}
    % \end{subfigure}%
    % ~ 
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[height=1.5in, width=0.85\textwidth]{iclr2022/images/G_GL_polyPlots/citeseer_boundaryReg.png}
        \caption{Citeseer}
        \label{RQ3_citeseer}
    \end{subfigure}
    
    \caption{Visualization of adapted eigenspectrum by our proposed model and~\gprgnn}
    \label{fig:PPGNN_learned_poly}
\end{figure}

% The next question that we would like to address is that does such a complicated polynomial exist in practice? 

% Since we don't have access to this underlying optimal frequency response, we try to construct this `optimal' frequency response by solving a regression task. The details of this regression are left to the appendix. On plotting the moving average of this constructed frequency response, we observe that our learned polynomial filters are structurally similar to this constructed frequency response, thereby learning. \textbf{I am not sure whether we should include this question/points at all. This is like opening a can of worms as these are the questions a reviewer can ask: 1. Does a complicated polynomial exist in practise? If we use the constructed optimal polynomial, now all the claims about not needed a complicated polynomial for homophilic datasets don't work anymore. If we do decide to add this, lets just remove the question on the optimal polynomial. Lets take a call on this.} 

\textbf{[RQ4] In Section~\ref{sec:proposedapproach}, we based our model on the observation that low-pass and high-pass frequency components are critical for task performance. Do they really contain useful information?}

\textbf{Using Table~\ref{tab:result_ppgnnVSgprgnn}, Figure~\ref{fig:AdaptingEVDTopBottom}}

\textbf{Points to convey:}

1) Adapting the lower and higher ends of the spectrum for heterophilic datasets can already lead to a graph that performs well for the node classification task. However, adapting the entire spectrum for homophilic datasets leads to a better node classification performance, as compared to adapting only the ends of the spectrum. This seems to show that the lower and higher ends of the spectrum contain lot more information about the graph for heterophilic datasets, while the information seems to be more diffused throughout the entire spectrum for homophilic datasets. On adapting both the lower and higher ends of the spectrum in conjunction with adapting the entire spectrum does lead to better classification performance for homophilic datasets, further strengthening the argument that adapting the entire spectrum is indeed required for homophilic graphs.   
From this analysis, we conjecture that for heterophilic datasets, the lower and higher ends of the spectrum contain a lot more information about the graph (for the task at hand). We also conjecture that for homophilic datasets, the information regarding the graph is diffused throughout the spectrum thereby needing adaption on the entire spectrum. Evidence from Table~\ref{tab:result_ppgnnVSgprgnn}. For instance, GL Term outperforms GPR-GNN on all heterophilic datasets. However, GL term is lacking in performance on Homophilic datasets. In PP-GNN, where the missing middle eigen spectrum is also accounted for, we see it performing well across the datasets. This reiterates it is important to account for the entire spectrum in homophilic graphs. 

We plot the results for the described studies in Figure~\ref{fig:AdaptingEVDTopBottom} and make the following observations: 1) For Homophilic datasets, adapting an increasing number of components in the lower ends of the spectrum exhibits better classification accuracy compared to adapting the higher end counterparts. Also, adapting only the lower or higher frequencies in conjunction with a global filter shows similar performance. Basis these observations, we extrapolate that important signals in the input graph are diffused throughout the spectrum, thereby requiring an adaption on the entire spectrum. 2) On the contrary, Heterophilic datasets display significant improvements in performance by adapting the higher ends of the spectrum. We also observe that adapting the lower ends of the spectrum in conjunction with adapting the entire spectrum performs worse than adapting only higher ends of the spectrum. This seems to show that for Heterophilic datasets, useful signals for the task at hand are concentrated in the higher end of the spectrum. 




\begin{table}[H]
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|ccccccccccc}
\hline
{\color[HTML]{000000} \textbf{Test Acc}} & \textbf{Texas}                                 & \textbf{Wisconsin}                             & \textbf{Squirrel}                              & \textbf{Chameleon}                    & \textbf{Cornell}                      & \textbf{Cora-Full}                             & \textbf{Citeseer}                              & \textbf{Pubmed}                                & \textbf{Cora}                                  & \textbf{Computer}                              & \textbf{Photos}                                \\ \hline
\textbf{GPR-GNN}                & 81.35   (5.32)                                 & 82.55   (6.23)                                 & 46.31   (2.46)                                 & 62.59   (2.04)                        & 78.11   (6.55)                        & 61.37   (0.96)                                 & 76.84   (1.69)                                 & 89.08   (0.39)                                 & 87.77   (1.31)                                 & 82.38   (1.60)                                 & 91.43   (0.89)                                 \\
\textbf{GL Term}                & 85.68   (3.83)                                 & 85.10   (3.09)                                 & 55.63   (1.44)                                 & \textbf{68.51 (1.64)}                 & \textbf{82.70 (5.13)}                 & 55.93   (0.77)                                 & {\color[HTML]{330001} \textbf{78.41   (1.58)}} & 83.65   (0.53)                                 & 89.50   (0.78)                                 & 82.55   (1.93)                                 & 89.87   (0.49)                                 \\
\textbf{\ourmodel}            & {\color[HTML]{000000} \textbf{89.73   (4.90)}} & {\color[HTML]{000000} \textbf{88.24   (3.33)}} & {\color[HTML]{000000} \textbf{56.86   (1.20)}} & {\color[HTML]{000000} 67.74   (2.31)} & {\color[HTML]{000000} 82.43   (4.27)} & {\color[HTML]{000000} \textbf{61.42   (0.79)}} & {\color[HTML]{000000} 78.25   (1.76)}          & {\color[HTML]{000000} \textbf{89.71   (0.32)}} & {\color[HTML]{000000} \textbf{89.52   (0.85)}} & {\color[HTML]{000000} \textbf{85.23   (1.36)}} & {\color[HTML]{000000} \textbf{92.89   (0.37)}} \\ \hline
\end{tabular}
}
\caption{\ourmodel~v/s \gprgnn}
\label{tab:result_ppgnnVSgprgnn}
\end{table}

\begin{figure}[H]
    \centering
        \includegraphics[height=1.2in, width=\textwidth]{iclr2022/images/G_GL_tuning_lowHigh_comps/TuningEVDcollage_GPRGNN_tuningLowHighEVD.png}
    \label{fig:AdaptingEVDTopBottom}
    \caption{Adapting increasing number of top or bottom EVD components}
\end{figure}


% \textbf{[RQ4] Importance of low/high frequency components.}
%The improvement over the classification performance can be explained from two perspectives: (a) from the filter response, and (b) the adapted graph being learnt. All the experiments done till now indicate that we need more control over the frequency response towards the extremal subsets of the spectrum for the graphs having lower homophily score as compared to ones having a higher score, which work upon a shared polynomial response. 
% Theorem`\ref{thm:space_of_filters} showed that the basis corresponding to the adaptive filters (with supports on spectrum's extrema) spans a different space, a point of which represents the corresponding low/high frequency response. We term these points to be having a 'locally focused response'. Following \textbf{[RQ3]}, we know that homophilic graphs are relatively apathetic towards the locally-focused responses. To understand the role of adapting low and high frequency components in \ourmodel~for homophilic datasets, we perform the following ablative studies. \textbf{1)} We assess the test performance for our \ourmodel~with only the $G_L$ term. This forces to learn from a locally-focused family. The results are present in Figure~\ref{fig:AdaptingEVD}, where learning with only the GL term (plot corresponding to 'GL EVD') results in a marginal drop of performance as comapred to the global model. \textbf{2)} To study this lack of sensitivity, we conduct another experiment, where we vary the parameters of the adaptive filters, namely support-size and the number of polynomials. We plot these results as  Figure~\ref{RQ4_cora}. We can observe that the homophilic graphs' performance is seemingly unaffected by these parameters. \textbf{3)} To compare the relative importance of top and bottom ends of the spectrum, we conduct experiments, where we adapt only one of these ends at a time, on two models: a model with global polynomial present (we call it '\ourmodel-Top/Bottom EVD') and a model without it (referred to as 'GL-Top/Bottom EVD'). The corresponding results are plotted in Figure~\ref{fig:AdaptingEVD}. As expected, the first model is insensitive to the adaptation of any of the ends, whereas in the second model, we observe that adapting the bottom end of the spectrum gives significant performance lifts as compared to adapting the top end. This seems to suggest that a lot more information that is present at the lower ends of the spectrum as compared to the top ends. It also seems to show that information is diffused throughout the spectrum, for homophilic graphs.

% We perform similar sets of experiments for heterophilic datasets: \textbf{1)} When we force the model to learn from a global family, which is what \gprgnn~does, there's a significant drop in the performance, as evident in Table 1, which is in line with our claims. \textbf{2)} We modify this experiment, where now we run two models: \ourmodel~which adapts to both ends of spectrum (referred to as '\ourmodel~EVD') and the same model without the global polynomial (referrred to as 'GL EVD'), with results plotted in Figure~\ref{fig:AdaptingEVD}. We observe that the presence of a global polynomial doesn't affects the performance much. We then plot the learnt frequency response of only the GL term \ms{we also comment on beta here. If these look favourable, we add a line here}. \textbf{3)} For experiments where we adapt only one of these ends at a time, the results are plotted in Figure~\ref{fig:AdaptingEVD}. In contrast to our observations for homophilic datasets, adapting only the top ends of the spectrum gave significant performance gains compared to adapting only the lower end. We can observe that adapting the bottom ends of the spectrum in conjunction with adapting the entire spectrum still performs worse than adapting only the higher ends of the spectrum, on increasing the number of adapted eigenpairs. This seems indicate that useful signals, for the task at hand, are concentrated at the higher ends of the spectrum.   
%Experiment description%
% \ms{We plan an experiment where we run one $G_L$ only model in parallel with $G+G_L$ model of \gprgnn~for the heterophilic datasets and then observe the waveform learnt by the $G_L$ filters of both the $G_L$ only model and $G+G_L$ only model. If they seem to coincide/be very similar, we can make a strong statement: heterophilic Graphs are apathetic to the global polynomial family in presence of a locally-focused family, whereas homophilic datasets are apathetic to any locally focused family in presence of a global family. We have evidence for latter half, but we would need the $G_L$ responses for the first}.

\textbf{[RQ5] Does increasing the number of components and the number of polynomials improve our approximation of the underlying latent filter and give better performance?}\\

\textbf{Using Figure~\ref{fig:AdaptingSupportSize}}

\textbf{Points to convey:} \\
1) The variation in performance when increasing the number of polynomial filters is minimal. This same trend is observed across both homophilic and heterophilic graphs. 
[For fixed polynomial order]
2) For heterophilic graphs, varying the support size (number of evd components adapted) has a significant effect on the task performance. For instance, in Chameleon dataset (Figure~\ref{fig:AdaptingSupportSize} a) the task performance reaches it's peak when the support size increases to 256 and then we observe a dip in performance as we increase the support size. However, in Squirrel dataset, the task performance sharply increases as we increase the support size. As emphasized before, important signals for task are concentrated in extremes of the eigenspectrum for heterophilic graphs. This phenomenon is reflected in our plots.
3) For homophilic graphs, the task performance is agnostic to any increment in the support size. [Not sure why this is happening. Analysing the beta values might give us some insights.]
4) We also repeat the same analysis for a different polynomial order and observe similar behavior. This also suggests we can get good performance using our model with even a lower order polynomial.


\begin{figure}[H]
    \centering
        \includegraphics[height=1.2in, width=\textwidth]{iclr2022/images/2D_Plots/2D_plot_all_5_degree.png}
    \label{fig:AdaptingSupportSize5}
    \caption{Effect of varying the number of polynomial filters and the support size for a 5textsuperscript{th} polynomial}
\end{figure}


\begin{figure}[H]
    \centering
        \includegraphics[height=1.2in, width=\textwidth]{iclr2022/images/2D_Plots/2D_plot_all_10_degree.png}
    \label{fig:AdaptingSupportSize10}
    \caption{Effect of varying the number of polynomial filters and the support size for a 5textsuperscript{th} polynomial}
\end{figure}


\begin{table}[H]
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|llll}
\hline
\textbf{Test Acc}      & \multicolumn{1}{c}{\textbf{Squirrel}} & \multicolumn{1}{c}{\textbf{Chameleon}} & \multicolumn{1}{c}{\textbf{Citeseer}}                     & \multicolumn{1}{c}{\textbf{Cora}}   \\ \hline
\textbf{GL (Low)}      & 45.75 (1.69)                          & 56.73 (4.03)                           & 76.23 (1.54)                                              & 88.03 (0.79)                        \\
\textbf{GL (High)}     & 58.70 (1.60)                          & 69.19 (1.88)                           & 55.50 (6.38)                                              & 73.76 (2.03)                        \\
\textbf{G + GL (Low)}  & 50.96 (1.26)                          & 63.71 (2.69)                           & 78.07 (1.71)                                              & 89.56 (0.93)                        \\
\textbf{G + GL (High)} & 60.39 (0.91)                          & 67.83 (2.30)                           & 78.30 (1.60)                                              & 89.42 (0.97)                        \\ \hline
\textbf{PP-GNN}        & 56.21 (1.79)                          & 68.93 (1.95)                           & \multicolumn{1}{c}{{\color[HTML]{000000} 78.25   (1.76)}} & {\color[HTML]{000000} 89.52 (0.85)}
\end{tabular}
}
\caption{}
\label{tab:result_ppgnnVSgprgnn}
\end{table}

\begin{figure}[H]
    \centering
        \includegraphics[height=1.2in, width=\textwidth]{iclr2022/images/G_GL_tuning_lowHigh_comps/TuningEVDcollage_GPRGNN_tuningLowHighEVD.png}
    \label{fig:AdaptingEVDTopBottom}
    \caption{Adapting increasing number of top or bottom EVD components}
\end{figure}


% For heterophilic datasets, increasing the number of filters with fixed supports at spectrum's extremes can give the desired local control and allows us to search for models in an even higher dimensional subspace. However, this control comes at a cost of increased model complexity, thus increasing the generalization error. Due to this bias-variance trade off, we do not expect to see any monotonous trend in performance while increasing the number of filters. This is also reflected in Table X. One possible way to mitigate this trade off is to increase the support size without changing the number of filters. This does not reduces the bias as the model complexity and the search space dimension remain the same. Thus, we can adapt to more regions of the spectrum's extremas without running into bias-variance pulls. But since we have observed that model is relatively apathetic to global adaptation for heterophilic datasets, this indicates that the central parts of the spectrum adds a diffused signal to the response. This is further indicated by experiments of table XXX, where we see a significant increase in performance for initial increase of the support, but the performance drops after increasing it more than a certain number, which we hypothesize is where the diffusive response starts accumulating.

%To understand the role of adapting low and high frequency components in our proposed model, we perform the following ablative study. Our model can be viewed as learning a global filter (G, refer to equation) that acts on the entire eigenspectrum, which is refined by multiple adaptive polynomial filters (GL) acting on a few disjoint subsets of this spectrum. We decouple G and GL and study them in isolation. We report the test performance for these individual components in Table XXX and make the following observations: % We first learn a graph filter (G / GPR-GNN) that acts on the entire spectrum. Next, we learn a graph filter (GL) that adapts only the lower and higher ends of the eigenspectrum. Finally, we combine both the filters (G + GL/ PP-GNN) to understand the effect of such a combination.1) The graph filter (GL) performs better than the graph filter (G) (\gprgnn) on Heterophilic datasets. However, on most Homophilic datasets, G performs better than GL. We conjecture that for Heterophilic graphs, adapting both lower and higher ends of the spectrum can already lead to a graph that performs well for the node classification task. However, reaching such a graph for Homophilic datasets might require adapting the entire spectrum as useful signals could be scattered throughout. 
%1) Adapting the lower and higher ends of the spectrum for heterophilic datasets can already lead to a graph that performs well for the node classification task. However, adapting the entire spectrum for homophilic datasets leads to a better node classification performance, as compared to adapting only the ends of the spectrum. This seems to show that the lower and higher ends of the spectrum contain lot more information about the graph for heterophilic datasets, while the information seems to be more diffused throughout the entire spectrum for homophilic datasets. On adapting both the lower and higher ends of the spectrum in conjunction with adapting the entire spectrum does lead to better classification performance for homophilic datasets, further strenthening the arguement that adapting the entire spectrum is indeed required for homophilic graphs.   
% From this analysis, we conjecture that for heterophilic datasets, the lower and higher ends of the spectrum contain a lot more information about the graph (for the task at hand). We also conjecture that for homophilic datasets, the information regarding the graph is diffused throughout the spectrum thereby needing adaption on the entire spectrum. 
% 2) Following the previous conjecture, we then combine both G and GL and observe a performance boost across all the homophilic datasets, while retaining or improving performance across heterophilic datasets as well. 
% 2) Combining G with GL adapts the eigenspectrum that is not accounted in the GL graph filter. This effect is also reflected in Table XXX. G + GL model achieves significant improvements on Heterophilic datasets, while also giving considerable lifts on Homophilic datasets. This study reaffirms our conjecture that adapting the entire spectrum does indeed help increase the performance on Homophilic datasets.   


% \begin{figure}[H]
%     \centering
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.85\textwidth]{iclr2022/images/TA_Varying_EVD_Components/chameleon_pca_TA_Varying_EVD_Components.png}
%         \caption{Chameleon}
%         \label{RQ1_chameleon}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.85\textwidth]{iclr2022/images/TA_Varying_EVD_Components/citeseer_TA_Varying_EVD_Components.png}
%         \caption{Citeseer}
%         \label{RQ1_citeseer}
%     \end{subfigure}
%     ~
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.85\textwidth]{iclr2022/images/TA_Varying_EVD_Components/cora_TA_Varying_EVD_Components.png}
%         \caption{Cora}
%         \label{RQ1_cora}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.85\textwidth]{iclr2022/images/TA_Varying_EVD_Components/squirrel_TA_Varying_EVD_Components.png}
%         \caption{Squirrel}
%         \label{RQ1_squirrel}
%     \end{subfigure}
    
%     \label{fig:RQ1}
%     \caption{Impact of number of EVD components adapted on Test Accuracy in proposed model}
% \end{figure}


% Need to reformulate RQ2. THis is what we would have to add: How does adapting only low (GL-Low) and only high frequency (GL-High) components in conjunction with G affect task performance? Is it sufficient to create such a filter?
% \textbf{RQ2. How does adapting only low and high frequency components in isolation affect task performance? Is it sufficient to adapt only high or only low frequency components?} \textit{It is better to adapt both ends of the spectrum following experiments}

%\textbf{Our previous studies highlight the importance of adapting both low and high frequency components. How does adapting only low and high frequency components in isolation affect task performance? Is it sufficient to adapt only high or only low frequency components?}

%To understand this phenomenon, we perform two ablative studies: i) The first study adapts increasing number of eigenvalues in the lower ends of the frequency spectrum. ii) The second study explores a similar setting in the higher ends of the frequency spectrum. We further extend these studies by appending another filter in conjunction to adapt the entire frequency spectrum. We finally compare these settings with our proposed approach, which adapts eigenvalues in both ends of the spectrum in conjunction with a global filter.
% We finally adapt both the higher and lower ends of the spectrum while having another filter in conjunction that adapts the entire spectrum. 
%We plot the results for the described studies in Figure XXX and make the following observations: 1) For Homophilic datasets (Figures X, Y), adapting increasing number of components in the lower ends of the spectrum exhibits better classification accuracy compared to adapting the higher end counterparts. Also, adapting only the lower or higher frequencies in conjunction with a global filter shows similar performance. Basis these observations, we extrapolate that important signals in the input graph are diffused throughout the spectrum, thereby requiring an adaption on the entire spectrum. 2) On the contrary, Heterophilic datasets display significant improvements in performance by adapting the higher ends of the spectrum. We also observe that adapting the lower ends of the spectrum in conjunction with adapting the entire spectrum performs worse than adapting only higher ends of the spectrum. This seems to show that for Heterophilic datasets, useful signals for the task at hand are concentrated in the higher end of the spectrum. 
% \todo{1. Add Performance Plots. 2. Finish and add the polynomial plots, refine RQ2 once we have the polynomial plots.}



% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.85\textwidth]{iclr2022/images/G_GL_tuning_lowHigh_comps/chameleon_pca_GPRGNN_tuningLowHighEVD.png}
%         \caption{Chameleon}
%         \label{RQ2_chameleon}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.85\textwidth]{iclr2022/images/G_GL_tuning_lowHigh_comps/citeseer_GPRGNN_tuningLowHighEVD.png}
%         \caption{Citeseer}
%         \label{RQ2_citeseer}
%     \end{subfigure}

    % \begin{subfigure}[t]{0.5\textwidth}
    %     \centering
    %     \includegraphics[height=1.5in, width=0.85\textwidth]{iclr2022/images/G_GL_tuning_lowHigh_comps/cora_GPRGNN_tuningLowHighEVD.png}
    %     \caption{Cora}
    %     \label{RQ2_cora}
    % \end{subfigure}%
    % ~ 
    % \begin{subfigure}[t]{0.5\textwidth}
    %     \centering
    %     \includegraphics[height=1.5in, width=0.85\textwidth]{iclr2022/images/G_GL_tuning_lowHigh_comps/squirrel_GPRGNN_tuningLowHighEVD.png}
    %     \caption{Squirrel}
    %     \label{RQ2_squirrel}
    % \end{subfigure}
    
%     \label{fig:AdaptingEVD}
%     \caption{Adapting increasing number of top or bottom EVD components}
% \end{figure}


\textbf{RQ6. [Manan] How expensive is it to compute top/bottom EVD components in practice? (Can move it to motivation section as well)}\\
Since we only deal with the extremal eigenpairs, we use \MATLAB implementation of the Arnoldi-Lanczos' Iterative Algorithm, provided via ARPACK, which proceeds by first tridiagonalizing the input matrix, and then performs a series of non-trivial steps to obtain the required eigenpairs. It benefits immensely from the sparsity and symmetry of the input matrix, making it a suitable choice for. Complexity analysis of Lanczos seems to be hard to find in the literature. Analysis of the probabilistic relative failure of the algorithm, by Kuczyński and Woźniakowski indicates that the bounds for the Lanczos algorithm depend on the ratio between the difference of the two largest eigenvalues and the difference of the largest and the smallest eigenvalues.



%\textbf{RQ3 [Manan]  What is the effect of using multiple adaptive filters on classification performance? How \ourmodel's filter response varies from GPRGNN's. Can we connect this difference to improvements in accuracy? \ms{A possible reframe: "How can we attribute use of high/low pass filters to the performance gains, and when are they useful? Also what effects does the number of polynomials and the support sizes have on the performance?"; the difference in response then serves to answer the second question}}\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.85\textwidth]{images/2D_Plots/chameleon_pca_2D_plot_10_order}
%         \caption{Chameleon}
%         \label{RQ4_chameleon}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.5in, width=0.85\textwidth]{images/2D_Plots/cora_2D_plot_10_order}
%         \caption{Cora}
%         \label{RQ4_cora}
%     \end{subfigure}
%     % \\
%     % \vspace{2mm}
%     % \begin{subfigure}[t]{0.5\textwidth}
%     %     \centering
%     %     \includegraphics[height=1.5in, width=0.85\textwidth]{images/2D_Plots/squirrel_2D_plot_10_order}
%     %     \caption{Squirrel}
%     %     \label{RQ4_squirrel}
%     % \end{subfigure}%
%     % ~ 
%     % \begin{subfigure}[t]{0.5\textwidth}
%     %     \centering
%     %     \includegraphics[height=1.5in,width=0.85\textwidth]{images/2D_Plots/computers_2D_plot_10_order}
%     %     \caption{Computers}
%     %     \label{RQ4_computers}
%     % \end{subfigure}
    
%     \caption{Effect of varying the number of polynomial filters and the support size}
%     \label{fig:RQ4}
% \end{figure}

%\textbf{RQ4.} In Theorem X, we claimed that multiple polynomial adaptive filters can give lesser classification error compared to using a single polynomial filter. Does this actually happen in practice? What happens to the task performance as we vary the degree of the polynomial, the number of eigenvalues adapted and the number of adaptive filters?
% vary the number of adaptive filters
%5To understand 

%\todo{1. Update plot for all the intermediate values [2, 4, 8, 16,.., 1024], 2. Add plots. 3. Refine RQ4. once thats done}







%\textbf{RQ5.} Theorem Y shows that our proposed model can explore a larger space of graphs than~\gprgnn, thereby possibly leading to obtain a better graph for the task at hand. Can we quantify the quality of these graphs? \textbf{TBD: Experiment has to be done}


==> sections/introduction.tex <==
\section{Introduction}
In this work, we are interested in the problem of classifying nodes in a graph. In this problem, a graph and features for all the nodes in the graph are made available. We are also given labels for a subset of the nodes in the graph. The learning model utilizes this information to predict labels for the remaining nodes. Graph Neural Networks (GNNs) perform well on such problems~\citep{gcn}. GNNs predict a node's label by aggregating information from its neighbours. Thus, the performance of GNN is dependent on how well the given graph correlates with the node labels. Characterizing the correlation between the graph and node labels is an active area of research. Several metrics have been proposed including edge homophily~\citep{mixhop, h2gcn}, node homophily~\citep{geomgcn}, class homophily~\citep{newbenchmark}. All these metrics show that GNNs perform well when the graphs and node labels are positively correlated. For example, in the simplest case, GNNs work well when the node and its neighbours share similar labels. However, the performance can be poor if this criterion is not satisfied.

Several proposed GNN models attempt to be robust to the underlying correlation between graphs and labels. Some approaches modify the aggregation mechanism~\citep{geomgcn, h2gcn, supergat}, while other approaches propose to estimate and leverage the label-label compatibility matrix as a prior~\citep{cpgnn}. More recent approaches have tackled this problem from a filter learning perspective~\citep{fagcn,gprgnn}. These methods learn a filter function that operates on the eigenvalues of the graph. With eigenvalues having frequency interpretations~\citep{shumangsp}, the filter function selectively accentuates and suppresses various frequencies as required by the task. This process enables the model to learn better embeddings, which translates to improved performance. Our interest lies in the area of modelling GNNs that can learn an effective filter.

\citet{gprgnn} proposed to learn a polynomial filter. This model achieves good performance gains on several datasets with varying correlations between graphs and labels. However, we observe that learning a polynomial of a degree lower than the number of nodes can be seen as solving an over-determined system of equations. Our observation suggests needing a higher-order polynomial to model richer or more complex frequency responses for certain datasets. The design of the model proposed in~\cite{gprgnn} makes it ineffective in learning a higher-order polynomial. It happens because the model attempts to overcome over-smoothing by giving smaller coefficient values to larger powers. In this paper, we address this issue and make the following contributions:
\begin{itemize}
    \setlength\itemsep{0.1cm}
    \item Inspired by \citet{gprgnn}, we propose to learn a polynomial filter; however, we do so by learning a sum of polynomials over different subsets of eigenvalues. Such modelling enables learning higher-order polynomials with several low order polynomials acting over the different subsets.
    \item Such modelling, however, requires an eigendecomposition of the graph, which can be expensive. We leverage the model in~\citet{gprgnn} and the fact that there exist efficient algorithms for computing top and bottom eigen components to propose a practically efficient model.
    \item We present theoretical analysis that suggests that our sum of polynomials approach can approximate a latent optimal filter better than a single polynomial. We also show that the space of learnable filters and graphs using our approach is larger than what is possible with~\citet{gprgnn}.
    \item Our experimental results show that our model performs better than state-of-the-art methods on several datasets, giving up to 10\% gains. These gains indicate that modelling the filter as a sum of polynomials is needed to approximate the latent filter better. We also answer other research questions through ablative studies, including the importance of the top and bottom eigenvalues, the number of top and bottom eigenvalues needed, the number of polynomials needed, and the trade-offs involved.
\end{itemize}

The rest of the paper is organized as follows: We present related work in Section~\ref{sec:relatedwork}, problem setup and motivation for the approach in Section~\ref{sec:preliminaries}, details of the proposed approach with complexity and theoretical analysis in Section~\ref{sec:proposedapproach} and finally experimental results and empirical analysis in Section~\ref{sec:experiments}.

==> sections/preliminaries_V1.tex <==
\section{Problem Setup and Motivation}
\label{sec:preliminaries}
We focus on the problem of semi-supervised node classification on a simple graph $\graph = (\verts, \edges)$, where $\verts$ is the set of vertices and $\edges$ is the set of edges. Let $\adj \in \{0, 1\}^{n \times n}$ be the adjacency matrix associated with $\graph$, where $n = |\verts|$ is the number of nodes. Let $\mathcal{Y}$ be the set of all possible class labels. Let $\feat \in \real^{n \times d}$ be the $d$-dimensional feature matrix for all the nodes in the graph. Given a training set of nodes $\train \subset \verts$ whose labels are known, along with $\adj$ and $\feat$, our goal is to predict the labels of the remaining nodes. Let $\adji = \adj + \eye$ where $\eye$ is the identity matrix. Let $\dadji$ be the degree matrix of $\adji$ and $\tadj = \dadji^{-1/2}\adji\dadji^{-1/2}$. 

Let $\tadj = \boldsymbol{E}\adjS\boldsymbol{E}$ be the eigendecomposition of $\tadj$. Then, the spectral convolution of $\feat$ on the graph $\adj$ can be defined via the reference operator $\tadj$ and a filter function $h$ operating on the eigenvalues, in the Fourier domain~\citep{tremblay2017design} as,
\begin{gather}
    \label{eq:spec_conv}
    Z = \boldsymbol{E}H(\adjS)\boldsymbol{E}X
\end{gather}
where $H(\adjS) = \textrm{diag}(h(\adjS))$. This process can be seen as the filter function adapting the graph for the desired task at hand. To tackle the problem of heterophily,~\citet{gprgnn} proposed a polynomial filter design, $H(\adjSv) = \sum_{i=1}^k \alpha_i \adjSv^i$ where $\alpha_i$'s are coefficients of the polynomial, $k$ is the order of the polynomial and $\adjSv$ is any eigenvalue from $\adjS$. Thus, $H(\adjS) = \textrm{diag}(V\boldsymbol{\alpha})$ where $V \in \real^{n \times k}$ is a Vandermonde matrix constructed using eigenvalues from $\adjS$ and $\boldsymbol{\alpha} \in \real^{k \times 1}$ is the vector consisting of $\alpha_j$'s. Thereby, we can write Equation~\ref{eq:spec_conv} as,
\begin{gather}
    \label{eq:spec_conv_poly_direct}
    Z = \boldsymbol{E}\textrm{diag}(V\boldsymbol{\alpha})\boldsymbol{E}X
\end{gather}
To avoid full eigendecomposition, Equation~\ref{eq:spec_conv_poly_direct} with the polynomial filter can be written as,
\begin{gather}
    \label{eq:spec_conv_poly}
    Z = \sum_{j=1}^k \alpha_j \tadj^j X
\end{gather}

 It is well-known that polynomial filters can approximate any graph filter \citep{shumangsp, tremblay2017design}. However, the inherent design of this model makes it less effective at learning a good polynomial filter. Let $h^*$ be the optimal filter for some given task, then comparing Equation~\ref{eq:spec_conv} and~\ref{eq:spec_conv_poly_direct}, we can see that for a fixed polynomial order $k$, the solutions for $\boldsymbol{\alpha}$ in Equation~\ref{eq:spec_conv_poly_direct} will be a superset of the solutions for the following linear system of equations,
\begin{gather}
    \label{eq:overdeterminedsystem}
    h^* = V\boldsymbol{\alpha}
\end{gather}
 Notice that, Equation~\ref{eq:overdeterminedsystem} is an overdetermined system of equations since the number of unknowns ($k$, the size of $\boldsymbol{\alpha}$) is less than the number of equations ($n$, the number of nodes). To obtain a consistent solution, we may have to work with higher-order polynomials. At higher powers, node features computed via $\tadj^jX$ becomes indistinguishable (see Figure~\ref{fig:indistinguishable}). Since the node features are indistinguishable, the importance of the coefficient associated with $\tadj^jX$ for the task at hand reduces significantly. We performed experiments by increasing the order of the polynomial. In Figure~\ref{fig:vary_order_cora} and~\ref{fig:vary_order_chameleon}, we plot the final task's accuracy for various polynomial orders. We observe that test accuracies do not improve significantly with an increase in the order of the polynomial. These observations are inline with Theorem 4.2 in~\citet{gprgnn}. It is noted in that Theorem that as the node features become indistinguishable (or over-smoothing happens), the corresponding coefficients of the polynomial go to zero. Now, one can avoid this issue with $\tadj^jX$ by directly working with Equation~\ref{eq:spec_conv_poly_direct}. However, this will incur the cost of doing full eigendecomposition, prohibitively expensive for large graphs. Even if we were to do this, $\adjSv_i$'s are in the range of $[-1, 1]$ and thus $\adjSv_i^j$ will diminish with higher powers. Thus, it will continue to be less effective in learning coefficients of a higher power. 
 
 To address the above problem, we propose to learn the polynomial filter as a sum of polynomials operating on different eigenvalue intervals. The next section is organized in the following way: 1] We gives detailed information about the model and the filter design, taking into account practical considerations of such an implementation. 2] We go ahead and show some of the properties of this filter design. We first show that our proposed filter design can approximate the latent optimal graph filter better than a single polynomial. As discussed earlier, the filter function adapts the graph for the desired task. We show that the possible learnable graphs via a single polynomial filter are a smaller subset of the learnable graphs via our proposed filter design. 3] Finally, we discuss the training and computational complexity of the proposed model.
 \begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[height=1.5in, width=0.95\textwidth]{iclr2022/images/Oversmoothening/cora_oversmoothening.png}
        \caption{}
        \label{fig:indistinguishable}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[height=1.5in, width=0.95\textwidth]{iclr2022/images/TA_Varying_K_GPRGNN/cora_TA_Varying_K_GPRGNN.png}
        \caption{}
        \label{fig:vary_order_cora}
    \end{subfigure}
    %\label{fig:fictitious}
    ~ 
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[height=1.5in, width=0.95\textwidth]{iclr2022/images/TA_Varying_K_GPRGNN/chameleon_pca_TA_Varying_K_GPRGNN.png}
        \caption{}
        \label{fig:vary_order_chameleon}
    \end{subfigure}
    \caption{In (a), we plot the average of pairwise distances between node features for the Cora dataset, after computing $\tadj^jX$ for increasing $j$ values. X-axis represents the various powers $j$ and the Y-axis represents the average of pairwise distances between node features. In (b) and (c), we plot the test accuracies of the model in \citet{gprgnn} for increasing order of polynomials for Cora and Chameleon dataset respectively. X-axis represents the order of the polynomial and Y-axis represents the test accuracy achieved for that order.}
\end{figure}


==> sections/preliminaries_V2.tex <==
\section{Problem Setup and Motivation}
\label{sec:preliminaries}
We focus on the problem of semi-supervised node classification on a simple graph $\graph = (\verts, \edges)$, where $\verts$ is the set of vertices and $\edges$ is the set of edges. Let $\adj \in \{0, 1\}^{n \times n}$ be the adjacency matrix associated with $\graph$, where $n = |\verts|$ is the number of nodes. Let $\mathcal{Y}$ be the set of all possible class labels. Let $\feat \in \mathbb{R}^{n \times d}$ be the $d$-dimensional feature matrix for all the nodes in the graph. Given a training set of nodes $\train \subset \verts$ whose labels are known, along with $\adj$ and $\feat$, our goal is to predict the labels of the remaining nodes. Let $\adji = \adj + \eye$ where $\eye$ is the identity matrix. Let $\dadji$ be the degree matrix of $\adji$ and $\tadj = \dadji^{-1/2}\adji\dadji^{-1/2}$. Let $\tadj = \eigenU\adjS\eigenU^T$ be the eigendecomposition of $\tadj$. Then, the spectral convolution of $\feat$ on the graph $\adj$ can be defined via the reference operator $\tadj$ and a filter function $h$ operating on the eigenvalues, in the Fourier domain~\citep{tremblay2017design, gprgnn} as,
\begin{gather}
    \label{eq:spec_conv}
    Z = \eigenU H(\adjS)\eigenU^T X = \eigenU\textrm{diag}(V\boldsymbol{\alpha})\eigenU^T X =  \sum_{j=1}^k \alpha_j \tadj^j X
\end{gather}
where $H(\adjS) = \textrm{diag}(h(\adjS))$. In this process, the filter function is essentially adapting the graph for the desired task at hand. The second equality follows from using a polynomial filter, $H(\adjSv) = \sum_{i=1}^k \alpha_i \adjSv^i$ where $\alpha_i$'s are coefficients of the polynomial, $k$ is the order of the polynomial and $\adjSv$ is any eigenvalue from $\adjS$. Note that $H(\adjS) = \textrm{diag}(V\boldsymbol{\alpha})$ where $V \in \mathbb{R}^{n \times k}$ is a Vandermonde matrix constructed using eigenvalues from $\adjS$ and $\boldsymbol{\alpha} \in \mathbb{R}^{k \times 1}$ is the vector consisting of $\alpha_j$'s. The last equality follows from the eigendecomposition properties, enabling avoidance of eigendecomposition. It is well-known that polynomial filters can approximate any graph filter \citep{shumangsp, tremblay2017design}. However, several practical challenges arise in learning a good polynomial filter. We briefly discuss them below.  %However, the inherent design of this model makes it less effective at learning a good polynomial filter.
%Thereby, we can write Equation~\ref{eq:spec_conv} as,
%\begin{gather}
%    \label{eq:spec_conv_poly_direct}
%    Z = \boldsymbol{E}\textrm{diag}(V\boldsymbol{\alpha})\boldsymbol{E}X
%\end{gather}
%To avoid full eigendecomposition, Equation~\ref{eq:spec_conv_poly_direct} with the polynomial filter can be written as,
%\begin{gather}
%    \label{eq:spec_conv_poly}
%    Z = \sum_{j=1}^k \alpha_j \tadj^j X
%\end{gather}

Let $h^*$ be the optimal filter for some given task. Learning a polynomial filter involves the approximation: $h^* \approx  V\boldsymbol{\alpha}$. Notice that this system is over-determined since the number of unknowns ($k$, the size of $\boldsymbol{\alpha}$) is less than the number of equations ($n$, the number of nodes). To obtain a consistent solution, we may have to work with higher-order polynomials. Working with higher powers poses several practical challenges, and the following observations are in order. First, node features computed via $\tadj^jX$ becomes indistinguishable (see Figure~\ref{fig:indistinguishable} and \ref{subsec:node_feature_indistin}). Since the node features are indistinguishable, the importance of the coefficient associated with $\tadj^jX$ for the task at hand reduces significantly. These observations are in line with Theorem 4.2 in~\citet{gprgnn}, where it states that as over-smoothing happens, the corresponding coefficients of the polynomial go to zero. We observe that with insignificant contributions from higher-order terms, the performance (aka test accuracy) does not improve with the increase in the order of the polynomial (See Figure~\ref{fig:vary_order_cora}, ~\ref{fig:vary_order_chameleon} and \ref{app:vary_order_gprgnn}).   
%We performed experiments by increasing the order of the polynomial. In Figure~\ref{fig:vary_order_cora} and~\ref{fig:vary_order_chameleon}, we plot the final task's accuracy for various polynomial orders. We observe that test accuracies do not improve significantly with an increase in the order of the polynomial. 
Next, one can think of addressing this issue with $\tadj^jX$ by directly working with full eigendecomposition. However, this approach is prohibitively expensive for large graphs. Even if we were to do this, $\adjSv_i$'s are in the range of $[-1, 1]$ and thus $\adjSv_i^j$ will diminish with higher powers. Therefore, it will continue to be less effective in learning coefficients of a higher power. Motivated by the above observations, we propose a novel piece-wise polynomial filter learning approach.  
 
 %To address the above problem, we propose to learn the polynomial filter as a sum of polynomials operating on different eigenvalue intervals. The next section is organized in the following way: 1] We gives detailed information about the model and the filter design, taking into account practical considerations of such an implementation. 2] We go ahead and show some of the properties of this filter design. We first show that our proposed filter design can approximate the latent optimal graph filter better than a single polynomial. As discussed earlier, the filter function adapts the graph for the desired task. We show that the possible learnable graphs via a single polynomial filter are a smaller subset of the learnable graphs via our proposed filter design. 3] Finally, we discuss the training and computational complexity of the proposed model.
 
 \begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[height=1.5in, width=0.95\textwidth]{iclr2022/images/Oversmoothening/cora_oversmoothening.png}
        \caption{}
        \label{fig:indistinguishable}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[height=1.5in, width=0.95\textwidth]{iclr2022/images/TA_Varying_K_GPRGNN/cora_TA_Varying_K_GPRGNN.png}
        \caption{}
        \label{fig:vary_order_cora}
    \end{subfigure}
    %\label{fig:fictitious}
    ~ 
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[height=1.5in, width=0.95\textwidth]{iclr2022/images/TA_Varying_K_GPRGNN/chameleon_pca_TA_Varying_K_GPRGNN.png}
        \caption{}
        \label{fig:vary_order_chameleon}
    \end{subfigure}
    \caption{In (a), we plot the average of pairwise distances between node features for the Cora dataset, after computing $\tadj^jX$ for increasing $j$ values. X-axis represents the various powers $j$ and the Y-axis represents the average of pairwise distances between node features. In (b) and (c), we plot the test accuracies of the model in \citet{gprgnn} for increasing order of polynomials for Cora and Chameleon dataset respectively. X-axis represents the order of the polynomial and Y-axis represents the test accuracy achieved for that order.}
\end{figure}

==> sections/preliminaries_old.tex <==
\section{Problem Setup and Motivation}

We focus on the problem of semi-supervised node classification on a simple graph $\graph = (\verts, \edges)$, where $\verts$ is the set of vertices and $\edges$ is the set of edges. Let $\adj \in \{0, 1\}^{n \times n}$ be the adjacency matrix associated with $\graph$, where $n = |\verts|$ is the number of nodes. Let $\mathcal{Y}$ be the set of all possible class labels. Let $\feat \in \real^{n \times d}$ be the $d$-dimensional feature matrix for all the nodes in the graph. Given a training set of nodes $\train \subset \verts$ whose labels are known, along with $\adj$ and $\feat$, our goal is to predict the labels of the remaining nodes. The proportion of edges that connect two nodes with the same labels in a graph is called the homophily score of the graph. In our problem, we are particularly concerned with graphs that exhibit low homophily scores. In the next sub-section, we provide background material on the GPR-GNN modelling method and its approach to graph adaptation.

\subsection{\gprgnn~Model}  
The \gprgnn~\citep{gprgnn} model consists of two core components: (a) a non-linear network that transforms raw feature input $\feat$: ${\bf Z}^{(0)} = f(\feat;{\mathbf W})$ and (b) a generalized page ranking (GPR) component, ${\mathbf G}$, that essentially aggregates  the transformed output ${\mathbf Z}$ recursively as: ${\bf Z}^{(k)} = \adj{\bf Z}^{(k-1)}, k = 1, \ldots, K$. Notice that there is no nonlinear operation involved after each aggregation step over $k$. Therefore, the functionality of the GPR component can be written using an operator ${\mathbf G}$ defined as: ${\mathbf G} = \sum_{k=0}^K \alpha_k {\mathbf A}^k$
and we obtain aggregated node embedding by applying ${\mathbf G}$ on the nonlinear network output:  ${\mathbf S} = {\mathbf G} {\mathbf Z}^{(0)}$. 
Using eigendecomposition, ${\adj} = \eigenU \adjS \eigenU^T$, \citet{gprgnn} presented an interpretation that the GPR component essentially performs a graph filtering operation: ${\mathbf G} = \eigenU h_K(\adjS) \eigenU^T$ where $h_K(\adjS)$ is a polynomial graph filter applied element-wise and $h_K(\adjSv_i) = \sum_{k=0}^K \alpha_k \adjSv^k_i$ where $\adjSv_i$ is the $i^{th}$ eigen value. As explained in~\citet{gprgnn}, learning filter coefficients (i.e.,$\alpha$) help to get improved performance. Since the coefficients can take negative values the \gprgnn~model is able to capture high-frequency components of the graph signals, enabling the model to achieve improved performance on heterophilic graphs. In the following subsection, we identify the inadequacies of \gprgnn.

\subsection{Motivation}  
\label{motivation}

\noindent\fbox{%
    \parbox{\textwidth}{%
    We plan to add the inadequacies of \gprgnn~in this section itself.
        \begin{enumerate}
            \item Now, for a fixed output $\bf Z_0$, \gprgnn~ tries to obtain the optimal value of the parameters of the filter $h_K$, which try to approximate the underlying waveform $h^*$ corresponding to the graph $\bf{A}$ and transformed features $\bf Z_0$. If we assume that the noise-less $h^*$ is fully observed on the interval [-1,1] and assuming it can be arbitrarily complex, then it can approximated it with using a very high degree polynomial, so it fits almost perfectly in [-1,1] (since this interval of interest is fully observed, any polynomial with appropriately high order can be made to fit the waveform with arbitrary accuracy (that depends on the choice of degree of the polynomial).
            \item But we observe that increasing the degree of polynomial in \gprgnn~does not generally leads to an increase in its performance. The reason behind this is the phenomenon of oversmoothing, that is observed for orders greater than some $K'$, such that for $K>K'$, the rows of matrix $\mathbf{A}^K\mathbf{X}$ approach a single vector with arbitrary proximity governed by $K$.
            \item We take a different way to approximate the waveform. (Need to cite those spline interpolation literature here), where it can be shown that, error bound in fitting a single spline to the waveform is more that the error achieved in fitting multiple independent splines defined on disjoint, mutually exclusive domains. The plots in Figure 1 demonstrate the idea where a single 10-degree polynomial fails to fit a fictitious waveform as compared to multiple 10-degree polynomials. We observe that even using multiple 5-degree polynomials performs much better than a single 1-degree polynomial as evident in figure 1(c).
            \item After this we define \textbf{Polynomial Adaptive Filters} like in Definition 3.1 whose definition naturally arises from the last point.
            \item We prove that least achievable approximation error by using one polynomial is higher than the least achievable approximation error obtained by using multiple adaptive filters. This is Theorem 3.1
            \item We theoretically show that a model with adaptive filters learns a more diverse set of graphs than \gprgnn, which includes \gprgnn's graphs as well. This is Theorem 3.2 and increasing the hypothesis space is reducing bias. To show that the extra graphs reachable by our model perform well, we add the plots/numbers of those experiments where only the $GL$ term is present. The graph family learnt by only $GL$ model is disjoint with the family learnt by \gprgnn, and yet the numbers/performance is competitive with our model and superior with \gprgnn~on heterophilic datasets and comparable on homophilic ones.
            \item $\left[\text{IN PROGRESS}\right]$ We show that our model's generalization error bound that grows slowly when we increase adaptive filters, as compared to when we increase $K$.

        \end{enumerate}
    }%
}

\cite{fagcn} and \cite{gprgnn} have shown the importance of low/high frequency components for the node classification task on graphs with varying levels of homophily. The polynomial graph filter described in \gprgnn~can, in theory, approximate any function given a high degree polynomial, but computing higher order terms is computationally intensive. Instead, we show that having polynomial adaptive filters on top of \gprgnn~help us to get a reduced error bound for the same degree polynomial as compared with \gprgnn.

\begin{definition}[Polynomial Adaptive Filter] A \textbf{polynomial adaptive filter}, denoted by $h_f(\adjS)$, is a polynomial filter (parameterized by polynomial $p$) whose frequency response acts only on a subset of the spectrum of the reference matrix. Given a support, $\mathbf\sigma_f\subset\mathbf\sigma(\mathbf A)$; $h_f(\adjSv) = \mathbbm{1}_{\adjSv\in\sigma_f}p(\adjSv)$.
\end{definition}

The following theorem shows that having an polynomial adaptive filter with a polynomial filter approximate any frequency response over the graph better than just the polynomial filter.

\begin{theorem}
For any frequency response $h^*$, and an integer $K\in\mathbb{N}/{\infty}$, let $\Tilde{h}:=h+h_f$, with $h_f$ having any random eigenvalue support $\sigma_f$, and let $\Hat{h}:=h$. Assuming $h$ and $h_f$ to be parameterized by $K$-order polynomials $p$ and $p_f$ respectively, then $\min\left\Vert\Tilde{h} - h^*\right\Vert_2\leq\min\norm{\Hat{h}-h^*}_2$. Moreover, for multiple polynomial adaptive filters $h_{f_1},h_{f_2},...,h_{f_m}$ with disjoint supports, the same inequality holds for $\Tilde{h} = h + \sum_{i=1}^m h_{f_i}$. The inequality can be made tighter by appropriate selection of support sizes.
\end{theorem}
\begin{proof}
For simplicity, we show the above bound for the case where the size of supports of all $h_{f_i}$ are equal, though following can be easily extended to unequal supports as well. We make the following assumptions:
\begin{enumerate}
    \item $\abs{\sigma_{f_i}}>K,\;\; \forall i\in[m]$
    \item All eigenvalues of the reference matrix are distinct
\end{enumerate}

For methods that use a single polynomial filter, the polynomial graph filter, $h_K(\adjS) = diag(\mathbf V\mathbf \gamma)$ where $\mathbf{\gamma}$ is a vector of coefficients, with sorted in descending order in components, and $\mathbf V$ is a Vandermonde matrix:
\begin{equation*}
\begin{aligned}
    \mathbf V = 
    \begin{bmatrix} 
    1&\lambda_1&\lambda_1^2&\cdots&\lambda_1^K\\ 
    1&\lambda_2&\lambda_2^2&\cdots&\lambda_2^K\\
    \vdots&\vdots&\vdots&\ddots&\vdots\\
    1&\lambda_n&\lambda_n^2&\cdots&\lambda_n^K\\\end{bmatrix}\\
\end{aligned}
\end{equation*}

And to approximate a frequency response $h^*$, we have the following objective:
\[
\min_{\gamma}\norm{diag(h^*) - diag(\mathbf V\gamma)}^2_F = \min_{\gamma}\norm{h^* - \mathbf V\gamma}^2_2
 \]
Where $\norm{}_F$ and $\norm{}_2$ are the Frobenius and $L_2$ norms respectively. Due to assumption 2, the system of equations $h^* = \mathbf V\gamma$ is well-defined and has a unique minimizer, say $\gamma^*$. Next we break the error vector as:
\begin{equation*}
\begin{aligned}
    \mathbf e_p &:= h^* - \mathbf V\gamma^* \\ 
    &= \sum_{i=1}^m (h^*_i - \mathbf V_i\gamma^*) + (h^*_L - \mathbf V_L\gamma^*)\\ 
    &= \sum_{i=1}^m \mathbf e_{p_i} + \mathbf e_{p_L}
\end{aligned}
\end{equation*}
Where $h^*_i$ is a vector whose value at components corresponding to the set $\sigma(h_{f_i})$ is same as that of $h^*$ and rest are zero. Similarly, $\mathbf V^*_i$ is a matrix whose rows corresponding to the set $\sigma(h_{f_i})$ are same as that of $\mathbf V$ with other rows being zero. Also, $\mathbf V_L = \mathbf V - \sum_{i=0}^m \mathbf V_i$ and $h^*_L = h^* - \sum_{i=0}^m h^*_i$. Note that by this construction, the vectors $\mathbf e_i$ form a linearly independent set.
Now, we analyze the case where we have polynomial adaptive filters added, where the objective is:
\[
\min_{\gamma,[\gamma_i]}\norm{diag(h^*) - diag\left(\mathbf V\gamma + \sum_{i=0}^m \mathbf V_i\gamma_i\right)}^2_F = \min_{\gamma, [\gamma_i]}\norm{h^* - \mathbf V\gamma - \sum_{i=0}^m \mathbf V_i\gamma_i}^2_2
\]
Before characterizing the above system, we break a general error vector as:
\begin{equation*}
\begin{aligned}
    \mathbf e_g &:= h^* - \mathbf V\gamma - \sum_{i=0}^m \mathbf V_i\gamma_i\\ 
    &= \sum_{i=1}^m (h^*_i - \mathbf V_i(\gamma + \gamma_i)) - (h^*_L - \mathbf V_L\gamma) \\ 
    &= \sum_{i=1}^m \mathbf e_{g_i} + \mathbf e_{g_L}
\end{aligned}
\end{equation*}
Clearly, the systems of equations, $\mathbf e_{g_i} = 0,\;\;\forall i$ and $\mathbf e_{g_L} = 0$ are well-defined. Since all the systems of equations have independent argument, unlike in the polynomial filter case where the optimization is constrained over a single variable; one can now resort to individual minimization of squared norms of $\mathbf e_{g_i}$ which results in a minimum squared norm of $\mathbf e_g$. Thus, we can set:
\[
\gamma = \mathbf V_L^{\dagger}h^*_L;\;\;\;\;\;\gamma_i = \mathbf V_i^{\dagger}h^*_i - \mathbf V_L^{\dagger}h^*_L,\;\;\forall i\in[m] 
\]
to minimize squared norms of $\mathbf e_{g_i}$ and $\mathbf e_{g_L}$. Since these form an orthogonal set, we have $\norm{\mathbf e_{g}}^2 = \sum_{i=1}^m\norm{\mathbf e_{g_i}}^2 + \norm{\mathbf e_{g_L}}^2$, and hence the above assignment leads to minimizing $\mathbf e_g$.

Clearly, $\norm{\mathbf e_{p_i}}^2\leq \norm{\mathbf e_{g_i}}^2$ and $\norm{\mathbf e_{p_L}}^2\leq \norm{\mathbf e_{g_L}}^2$ since the LHS in these inequalities is a solution of a constrained minimization problem, whereas the RHS comes from an unconstrained one.
Hence,
\[
\begin{aligned}
\sum_{i=1}^m\norm{\mathbf e_{p_i}}^2 + \norm{\mathbf e_{p_L}}^2 &\leq \sum_{i=1}^m\norm{\mathbf e_{g_i}}^2 + \norm{\mathbf e_{p_L}}^2 \\
\min\left\Vert\Tilde{h} - h^*\right\Vert &\leq \min\norm{\Hat{h}-h^*}
\end{aligned}
\]
\end{proof}

\begin{theorem}
Let $\mathbb{G}$ be the family of graphs learned by \gprgnn~, such that $\mathbb{G}:=\{\mathbf{U}^T h(\mathbf{\Lambda})\mathbf{U}\;|\;\forall\text{ possible K-degree polynomial parameterizations of }h\}$ for any unitary matrix $\mathbf{U}$. If $\mathbb{G}':=\{\mathbf{U}^T \Tilde{h}(\mathbf{\Lambda})\mathbf{U}\;|\;\forall\text{ possible K-degree polynomial parameterizations of }\Tilde{h}\}$ is the family of graphs learned by \ourmodel~, with $\Tilde{h} = h + h_{f_1} + h_{f_2}$, where $h$ is parameterized by a K-degree polynomial supported over entire spectrum, $h_{f_1}$ and $h_{f_2}$ are adaptive filters parameterized by independent K-degree polynomials supported over top and bottom $t$ eigenvalues respectively, with $t<n/2$; then $\mathbb{G}$ and $\mathbb{G}'$ form a subspace in $\mathbb{M}_{n\times n}[\mathbb{R}]$, with $\mathbb{G}\subset \mathbb{G}'$. Also, $\frac{\text{dim}(\mathbb{G}')}{\text{dim}(\mathbb{G})} = 3$.
\end{theorem}
\begin{proof}
Consider the set of all the univariate polynomials having degree at most $K$ in the vector space over the ring $\mathbb{K}[x_1,\ldots,x_n]$ where $\mathbb{K}$ is the field of real numbers. Partition this set into $n$ subsets, say $V_1,\ldots,V_n$, such that for $i\in[n]$,  $V_i$ contains all polynomials of degree up to $K$ in $x_i$. It is easy to see that $V_1,\ldots,V_n$ are subspaces of $\mathbb{K}[x_1,\ldots,x_n]$. Define $V = V_1 \oplus V_2 \oplus \cdots \oplus V_n$. Define the matrix $D_{i}[c]$ whose $(i,i)^{\text{th}}$ entry is $c$ and all the other entries are zero. For $i\in[n]$, define a linear map $\phi_i:V_i \rightarrow \mathbb{M}_{n\times n}\left(\mathbb{R}\right)$ by $f(x_i)\mapsto D_{i}[f(\lambda_i)]$. Im($\phi_i$) forms a vector space of all diagonal matrices, whose $(i,i)$ entry is the evaluation of an element of $V_i$ at $\lambda_i$.
Generate a linear map $\phi:V\rightarrow \mathbb{M}_{n\times n}(\mathbb{R})$ by mapping $\phi(f(x_i))$ to $ \phi_i(f(x_i))$ for all $i\in[n]$. Note that $\phi_i$ for $i\in[n]$ are injective maps, making $\phi$ an injective map. Observe that $h(\mathbf{\Lambda})\subset \text{Im}(\phi)$ is a subspace with basis $\mathcal{B}_h:=$ $\{\phi(1+\cdots+1), \phi(x_1+\cdots+x_n), \ldots, \phi(x_1^K+\cdots+x_n^K)\}$, making $\text{dim}(h(\mathbf{\Lambda})) = K+1$. Similarly we have, $h'(\mathbf{\Lambda})\subset \text{Im}(\phi)$, a subspace with basis $\mathcal{B}_{h'}:=\mathcal{B}_h \bigcup\;\{\phi(1+\cdots+1+0+\cdots+0), \phi(x_1+\cdots+x_t+0+\cdots+0), \ldots, \phi(x_1^K+\cdots+x_t^K+0+\cdots+0)\}\bigcup\;\{\phi(0+\cdots+0+1+\cdots+1), \phi(0+\cdots+0+x_{n-t+1}+\cdots+x_n), \ldots, \phi(0+\cdots+0+x_{n-t+1}^K+\cdots+x_n^K)\}$, implying $h(\mathbf{\Lambda})\subset h'(\mathbf{\Lambda})$ and $\text{dim}(h'(\mathbf{\Lambda})) = 3(K+1)$. Consider the injective linear maps $f_1,f_2:\mathbb{M}_{n\times n}(\mathbb{R})\rightarrow \mathbb{M}_{n\times n}(\mathbb{R})$ as $f_1(\mathbf{A})=\mathbf{U}^T\mathbf{A}$ and $f_2(\mathbf{A})=\mathbf{AU}$. Define $f_3: \text{Im}(\phi) \rightarrow \mathbb{M}_{n\times n}(\mathbb{R})$ as $f_3(\mathbf A) = (f_1\circ f_2)(\mathbf A)$. Since $f_3$ is a monomorphism, we have $\mathbb{G}\subset \mathbb{G}'$.
\end{proof}

\begin{corollary}
For a frequency response $h^*$ belonging to a set of absolute minimizers of the downstream task objective corresponding to the optimal error corresponding to any $\Theta$, use of polynomial adaptive filters achieve a lower error in approximating $h^*$ than \gprgnn~and Linear Graph Convolution (LGC) methods. Specificially for node classification, $\Tilde{h}\in \argmin_h[\min_{\Theta} \norm{\mathbf{Y} - softmax(\eigenU h(\adjS)\eigenU^Tf_{\Theta}(\mathbf X)}_F^2]$, where $f_{\Theta}$ is a (non) linear down-scaling function. Minimizing the cross-entropy error is approximately equivalent to approximating the response $\Tilde{h}$ above.
\end{corollary}
\begin{proof}
We start by bounding the cross-entropy loss similar to \cite{errorcomp}. Let $q(\cdot|x_i):=softmax(\eigenU h(\adjS)\eigenU^Tf_{\Theta}(\mathbf X)$ where the softmax is applied along the rows of its argument. Denote the true label of node $i$ as $y_i$ We define the cross-entropy and MSE loss as:
\[
\begin{aligned}
\mathcal{L}_{xent} &= -\sum_{i=1}^n [\ln q(y_i|x_i)]\\
\mathcal{L}_{MSE} &= \sum_{i=1}^n\sum_{y=1}^c [\delta(y,y_i) - q(y|x_i)]^2
\end{aligned}
\]
While cross-entropy is only defined over the model's score for the correct label, MSE is defined over model's score for all the labels, making it difficult to directly compare it with the cross-entropy. We instead try to get the upper and lower bounds for the MSE. For any node $i$, the cost term for MSE is 
\[
\mathcal{L}_{MSE,i} = \sum_{y=1}^c [\delta(y,y_i) - q(y|x_i)]^2 = (1-q(y_i|x_i))^2 + \sum_{y\neq y_i} q(y|x_i)^2
\]
Now by definition, every component of $q(\cdot|x_i)$ is positive. Hence, we have: 
\[
\sum_{y\neq y_i} q(y|x_i)^2 \leq \left(\sum_{y\neq y_i} q(y|x_i)\right)^2 = \left(1-q(y_i|x_i)\right)^2
\]
Thus,
\[
\mathcal{L}_{MSE,i} \leq 2\left(1-q(y_i|x_i)\right)^2 < -\ln q(y_i|x_i) = \mathcal{L}_{xent, i} \\
\]
The second inequality holds since $q(y_i|x_i) \in (0,1)$. Above result implies that the upper bound of MSE is strictly bounded above by the cross-entropy loss. Thus by minimizing the cross-entropy, one also minimizes the MSE, and it is easy to see that:

\begin{equation*}
\begin{split}
\mathcal{L}_{MSE} & = \norm{\mathbf{Y} - softmax(\eigenU h(\adjS)\eigenU^Tf_{\Theta}(\mathbf X))}_F^2 \\
&= \norm{\mathbf{Y} - softmax(\eigenU h^*(\adjS)\eigenU^Tf_{\Theta}(\mathbf X) + softmax(\eigenU h^*(\adjS)\eigenU^Tf_{\Theta}(\mathbf X) - softmax(\eigenU h(\adjS)\eigenU^Tf_{\Theta}(\mathbf X)}_F^2 \\
&\leq \norm{\mathbf{Y} - softmax(\eigenU h^*(\adjS)\eigenU^Tf_{\Theta}(\mathbf X)}_F^2  + \norm{softmax(\eigenU h^*(\adjS)\eigenU^Tf_{\Theta}(\mathbf X) - softmax(\eigenU h(\adjS)\eigenU^Tf_{\Theta}(\mathbf X)}_F^2 \\
&\leq \norm{softmax(\eigenU h^*(\adjS)\eigenU^Tf_{\Theta}(\mathbf X) - softmax(\eigenU h(\adjS)\eigenU^Tf_{\Theta}(\mathbf X)}_F^2 \\
&\leq \norm{\eigenU h^*(\adjS)\eigenU^Tf_{\Theta}(\mathbf X - \eigenU h(\adjS)\eigenU^Tf_{\Theta}(\mathbf X}_F^2\\
&=\norm{\eigenU (h^*(\adjS) - h(\adjS))\eigenU^Tf_{\Theta}(\mathbf X)}
\end{split}
\end{equation*}

The second inequality results from the term $\norm{\mathbf{Y} - softmax(\eigenU h^*(\adjS)\eigenU^Tf_{\Theta}(\mathbf X)}_F^2$ being independent of $h$. The third inequality results from the standard softmax being an 1-Lipschitz function. Thus, when we minimize the classification objective, we also end up minimizing the MSE. Since $\Tilde{h},\Tilde{\Theta}=\argmin_{h.\Theta}\mathcal{L}_{MSE}$ define the best performing model for the observed graph data in the \ourmodel~family, this defines the lower bound on the achievable MSE across all models in the \ourmodel~family. Now, it follows from Theorem 3.1 that the frequency response corresponding to this lower bound achievable by any model in \ourmodel~family is closer to the observed frequency response than the family of models relying on a polynomial filter.
\end{proof}

Theorem 3.1 implies that polynomial adaptive filters better approximate the frequency response, since they provide flexibility to adapt to specific regions of the spectrum providing a local control over it, without any dependence on the other regions, unlike their single polynomial counterparts which try to adapt to all eigenvalues at once thereby limiting the model flexibility. Thus adaptive filters eliminate the need of increasing the polynomial order while simultaneously achieving the better approximation. Since we do not have access to $h^*$ in order to correctly approximate $\Tilde{h}$, we do so approximately via minimizing a downstream objective like the cross-entropy objective for the node classification. This comes from the intuition that the observed labels are the function of the optimal frequency response.

% To support the argument that GPR-GNN as well our proposed approach reduces to solving a system of equations as shown in theorem 3.1, given a fixed input functional transformation, we can construct the following thought experiment.\\
% ----------------------------------------------------------------------

% \textbf{Possible argument for adding MLP} (Appendix):

% The questions that we still have to answer are the following:

% 1. How do we connect solving a system of equations to GPR-GNN\\
% 2. We then have to show how our approach ends up performing better. I think this is well known. 1 is not very well understood. I will try to use some intuition to connect 1 with GPR-GNN and then we can discuss that.

% Lets consider that we have a fixed functional transformation (instead of a learnable one) given by $f$. Then solution that GPR-GNN is trying to find out reduces to the following:

% \begin{equation}
%     \gamma^* = min_{\gamma} \sum_{i=1}^{N}H(y_i, softmax(\hat{y}_i))
% \end{equation}

% Where $H$ is the cross entropy, $N$ is the number of nodes, and $\hat{y}$ is defined as follows:

% %\begin{equation}
% %    \hat{y} = \sum_{k=1}^{M}\gamma_{k} A^{k} f(X)
% %\end{equation}

% %\begin{equation}
% %    \hat{y} = \sum_{k=1}^{M} \gamma_{k}U  \Lambda^k U^T f(X)
% %\end{equation}

% \begin{equation}
%     \hat{y} =  U  diag(V \gamma) U^T f(X)
% \end{equation}

% Let $y^*$ be the $\hat{y}$ that corresponds to the optimal solution. Let the filter response that corresponds to $y^*$ be h. Therefore:

% \begin{equation}
%     y^* =  U  diag(h) U^T f(X)
% \end{equation}

% Now from equation 2 and 3 we can observe that for GPR-GNN to approach the optimal solution, we need $\hat{y} \approx y^*$ when then implies $diag(V\gamma) \approx diag(h) \implies V\gamma \approx h$. Hence we can conjecture that given a fixed functional transformation, all GPR-GNN is learning is an optimal $\gamma$ that satisfies $V \gamma \approx h$ which can be obtained by solving a system of linear equations: $h = V\gamma$. Hence we can reduce the entire GPR-GNN model to solving a linear system of equations. \\
% ----------------------------------------------------------------------

% End to end error analysis:

% Let the output filtered graph signal that gives the best classification accuracy be defined as follows:

% \begin{equation*}
%     x^* = Udiag(h)U^Tf_{*}(X)    
% \end{equation*}

% Note that $h$ and $f_*$ are the ideal filter response and the ideal functional transformation of the input graph signal respectively. There can be multiple such $h$ and $f_*$ that would give a good classification accuracy. We pick one amongst the solution set.

% Let the output of the GPR-GNN model be defined as follows:

% \begin{equation*}
%     \tilde{x} = Udiag(V\gamma)U^Tf_{\theta}(X)    
% \end{equation*}

% The error due to GPR-GNN not being an exact solution can be seen as follows:

% \begin{equation*}
% \begin{aligned}
%     e = Udiag(h)U^Tf_{*}(X) - Udiag(V\gamma)U^Tf_{\theta}(X) \\
    
% \end{aligned}
% \end{equation*}


--------------------------------

Next, to empirically validate the results, we performed experiments on a complex, fictitious waveform where we demonstrate that a single polynomial performs poorly in approximating the waveform as compared to polynomial with polynomial adaptive filters applied. The corresponding plots are shown in Figure 1. Clearly, due to local flexibility of the adaptive filters, we can better approximate for the waveform without increasing the polynomial degree. We refer the reader to Appendix X, where we demonstrate that fits of comparable approximation error can be achieved by even a much lower degree polynomial, an observation that we exploit to achieve comparable performance on the downstream task using a scaled-down model.

\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[height=1.5in, width=0.95\textwidth]{figs/gprgnn_order10.png}
        \caption{Fitting single 10-degree polynomial}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[height=1.5in, width=0.95\textwidth]{figs/adafilt_order10.png}
        \caption{Fitting 10-degree polynomial with adaptive filters}
    \end{subfigure}
    %\label{fig:fictitious}
    \caption{To demonstrate the adaptability of adaptive polynomial filter, we try to approximate a complex waveform (blue dashed line) via (a) a single 10 degree polynomial, and (b) a 10-degree polynomial with 10 adaptive filters. The waveform learnt via the filter is shown in a solid dashed line. The corresponding RMSE are: (a) 3.9011, (b) 0.1824}
\end{figure}

\todo{For the proof:\\
    i) [\textbf{DONE}] From DSP, how frequency response of graph filter leads to solving system of equations: \\
    ii) [\textbf{DONE}] How h($\Lambda$), in \gprgnn, can be written as Vandermonde matrix \\
    iii) [\textbf{DONE}] Overdetermined/Underdetermined system based on how we partition these system of equations and solve the coefficients \\
    iv) [\textbf{DONE}] Talk about residual error for each case: 1) using single polynomial, 2) using multiple polynomials, and 3) a polynomial for every eigen component\\
    v) [\textbf{DONE}] Empirically show what happens to residual error as we increase number of polynomials (Fictitious waveform experiment)\\
    vi) [\textbf{DONE}] We also need to consider the effect of $f(X)$. We can probably write the alternative interpretation as a loose theorem or at the worst case a conjecture. However such a similar process would have to be done for our G+GL model as well.\\
    vii) Reframe theorem 3.1 and Corollary 3.1.1 into a) Lemma 1: Cross entropy minimization leads to MSE minimization; b) Solving h=V$\gamma$ leads to MSE minimization c) Theorem: multiple polynomials approximate $h^*$ better than single polynomial and d) a corollary that connects end-to-end: cross-entropy minimization gives better results for \ourmodel~than \gprgnn. Now to cover up the loose connection b/w lemma 1 and 2, we'll use the word 'approximately' in corollary.

\vspace{0.12in}

For the writing part for the motivation: \\   
1) [\textbf{DONE}] Introduce what having multiple adaptive filters upon GPRGNN mean \\
2) [\textbf{DONE}] State the theorem that having different adaptive filters can approximate any frequency response better than GPRGNN\\
3) [\textbf{DONE}] Then we can show empirical results on fictitious waveforms.\\
4) [\textbf{DONE}] Talk about scalability issues as well\\
5) Talk about oversmoothing as another possible drawback when increasing the polynomial order.
}
%Previous Motivation%
% We conduct the following empirical experiment to infer if a higher order polynomial is required for heterophilic datasets. We consider the eigendecomposition of given graph as ${\adj} = \eigenU \adjS \eigenU^T$ and we assign the node features as $\eigenU \adjS^{\frac{1}{2}}$. The columns in this feature matrix are essentially the eigenvectors. We construct new training data with these features using the known labels from training set~$\train$. We train a Logistic Regression model with this data. We perform max pooling on the per-class weights learned by the model and depict this in Figure~\ref{fig:polyAnalysis}. Max pooling reveals the highest weight required by the corresponding class for a given node. We also plot a closest fit polynomial on these weighted eigenvalues. We observe that in both Chameleon and Squirrel datasets, a polynomial with order as high as 70 is required to capture finer subtleties. 

% We conjecture that a sophisticated  adaptation function, or a high degree polynomial might be required for further improvement in performance. A simple fix to achieve this would be to increase the order of polynomial learned in \gprgnn. However, as reflected in Table XXX, we observe that increasing the polynomial order does not translate to improvement in performance and in some cases leads to degradation. Computing higher powers of the input graph leads to the oversmoothing problem (CITE XXX). Also, from a practical view, it is infeasible to compute powers of a large graph. Computationally this can also lead to numerical instabilities. In the next section, we present our proposed approach that addresses these inadequacies. 

==> sections/related.tex <==
\section{Related Works}
\label{sec:relatedwork}
In the recent times, Graph Neural Networks (GNNs) have become an increasingly popular method for semi-supervised classification with graphs. \citet{spectralnetwork} set the stage for early GNN models, which was then followed by various modifications~\citep{chebgnn, gcn, graphsage, gat}. Incorporating random walk information~\citep{ngcn, mixhop, deeperinsights} gave further improvements in these models, but they still suffer from over smoothing. Several proposed models attempt to overcome this problem~\citep{appnp, breadthwisebackprop, grand, itergnn}.

Another line of research explored the question of which graphs worked well with GNNs. The critical understanding was that the performance of GNN was dependent on the correlation of the graphs with the node labels. Several approaches \citep{mixhop, h2gcn, tdgnn} considered edge homophily and proposed a robust GNN model by aggregating information from several higher-order hops. \citet{supergat} also considered edge homophily and mitigated the issue by learning robust attention models. \citet{geomgcn} talks about node homophily and proposes to aggregate information from neighbours in the graph and neighbours inferred from the latent space. \citet{cpgnn} proposes to estimate label-label compatibility matrix and uses it as a prior to update posterior belief on the labels. However, these approaches still rely on the given graphs for information like the hop neighbours etc., which might be poor approximations of the desired neighbours with similar labels.

Some of the recent approaches focused on learning filter functions that operate on the eigenvalues of the graph. Learning these filter functions can be viewed as directly adapting the graph for the desired task. \citet{fagcn} models the filter function as an attention mechanism on the edges, which learns the difference in the proportion of low-pass and high-pass frequency signals. \citet{gprgnn} proposes a polynomial filter on the eigenvalues that directly adapts the graph for the desired task. \citet{ufgconv} decompose the graph into low-pass and high-pass frequencies, and define a framelet based convolutional model. Our work is closely related to these lines of exploration. In this work, we propose to learn a filter function as a sum of polynomials over different subsets of the eigenvalues, enabling design of effective filters to model task-specific complex frequency responses with compute trade-offs.  
%We provide theoretical analysis and insights into the model, including showing that the sum of polynomials can approximate the latent optimal filter better than learning a single polynomial.

%The following section gives a brief overview of the problem setting and motivates our proposed approach.

==> sections/statements.tex <==
\section{Reproducibility Statement}
\label{sec:reprostatement}
We have taken several steps to ensure the reproducibility of our work. First, we provide a detailed description of our model in Section~\ref{sec:proposedapproach}. Section~\ref{sec:experiments} provides a brief description of the datasets utilized in our experiments. A detailed description of the datasets, including their sources, statistics are given in the appendix (\ref{app:dataset_stats}). We also provide details on the number of splits and the method used to generate them. We also list out all the baselines utilized in the experiments in Section~\ref{sec:experiments}. A detailed description of these baselines and the parameter sweep ranges are given in the appendix (\ref{app:baselines}). We also provide implementation detail of our model in the appendix (\ref{app:implimentation}). 

%Additionally, we share an anonymized URL of the code for our model, and the data splits in the appendix (\ref{app:codeanddata}).

\section{Ethics Statement}
\label{sec:ethicstatement}
Social network graphs form the most exciting application for GNNs. GNNs can be used to reveal user information that the user otherwise would have preferred to keep private. Privacy-preserving methods might rely on obfuscating the graph by adding spurious edges, and these edges will, in turn, reduce the graph's correlation with the node labels. Earlier GNNs would likely not have predicted the target label with reasonable accuracy under this setting. Thereby, such obfuscation methods would give some level of privacy for the users. However, our model exhibits good performance even in the presence of a lower correlation. Such methods can make simple obfuscation based privacy approaches obsolete while still revealing important information about the users. On the other hand, our model can also give insights into what makes graphs reveal certain information and develop a more robust privacy model for graphs.
